Multilingual Reasoning Cascades Need More Context

Translation cascades for reasoning translate the query from another language to English, reason in English, and translate the answer back to the original language. This is a competitive approach to multilingual reasoning, but structurally lossy, since each stage discards information later stages may need, including cues for cultural grounding, register, and disambiguation. We examine the benefits of a simple and training-free intervention: a context-aware translation cascade, which additionally provides the original question, the English translated question, and the reasoning trace to the context of the final translation module. We evaluate gains across nine multilingual benchmarks including various task types, three backbone models, and 285 high-, mid-, and low-resource languages, and demonstrate strong gains for open-ended generation across models and resource regimes. We show that the original language question carries most of the beneficial context. Our study emphasizes the need to better design information flow in machine translation cascades for mitigating error propagation, and provides a simple and actionable default strategy: preserve the original user question until the end of the pipeline.

==> latex/main_text/1-intro.tex <==
\begin{itemize}
    \item Given that multilingual reasoning with LLMs is often of poorer quality than reasoning in high-resource languages like English, translation cascades are a critical alternative approach to reasoning in these settings \NB{cite}. Not only do they match or exceed SOTA end-to-end approaches, they are a strong practical option for leveraging powerful English LLMs without multilingual adaptation. Given this, improving the translation cascade is a critical way forwards in extending the powerful capabilities of LLMs to other languages.
    \item A typical cascaded approach involves translating different language input into English (\mtone module), performing reasoning in English (\reasoning module), and translating final answers back into the original language (\mttwo module) \NB{cite}.
    \item Cascaded systems notoriously suffer from error propagation \NB{cite}. In the LLM-MT cascade, \mttwo only has access to the final English answer but not the original language and English question. However, accurate and grounded translation of the final English answer may require informational cues present only in the original question, depending on the syntax of the target language, cultural context, or simply to recover from errors in intermediate stages. 
    \item This may be more relevant for some settings as compared to others: for example, for tasks requiring cultural context and grounding, given certain answer formats, or for certain target languages that diverge typologically or have poor translation support. However, in some settings it may even be damaging, when the additional context may be distracting or confusing. 
    \item In this work, we explore the following question: when does extra context benefit the machine translation cascade? 
    \item In order to do so, we first introduce \textbf{context-aware MT cascade} and compare it against the \textbf{standard cascade}. The former differs from the latter only in that the \mttwo module now has access to the original input and intermediate outputs, as depicted in \NB{@Dengjia, Stella: Figure 1. Showing both the standard MT cascade and the context-aware cascade. Preferably with a short and clear example motivating the latter.} This is intended as a simple and targeted mitigation strategy against the fallibility of cascaded systems to error propagation.
    \item We analyse the usefulness of a context-aware cascade given various factors, specifically, the task, required output format, the resource regime of the target language, and the typology of the target language.
    \item We find that (1) the context-aware cascade shows broad improvements over the standard cascade on average, constituting a simple but effective improvement for this paradigm (2) this effect is especially observed for open-ended generation as opposed to classification-style tasks, and across resource regimes and target language typologies. \NB{@Arnav reframe based on actual conclusions}
\end{itemize}


% \subsection{Motivation}
% \begin{itemize}
%     \item Multilingual cascades are a natural way to combine strong English reasoning with target-language generation
%     \item A common idea is to improve the final translation stage by giving MT2 more context, such as the original target-language question, the English question, the English reasoning trace, and the English answer \NB{As stated above, this is not already done. You can introduce it as an intuitive idea.}
%     \item This modification is intuitively appealing, but it is not obvious whether it should help uniformly across multilingual settings
%     \item In particular, we are interested in \textbf{culturally grounded tasks}, where generating a good target-language answer may require more than literal back-translation
% \end{itemize}

% \subsection{Research question}
% \begin{itemize}
%     \item When does context-aware MT2 help relative to a standard cascade and an end-to-end baseline?
%     \item Is the advantage of context mainly a function of resource level, or does it depend more strongly on the type of task/output being generated?
%     \item Do culturally grounded multilingual tasks form a regime in which context is especially useful?
% \end{itemize}

% \subsection{Main contributions}
% \begin{itemize}
%     \item We identify \textbf{culturally grounded multilingual tasks} as a regime where context-aware MT2 is especially effective
%     \item We show that this advantage is \textbf{not just a high-resource effect}: in the settings where context helps, it remains competitive or superior across resource levels
%     \item We show that the advantage is \textbf{regime-specific rather than universal}; non-cultural and exact-answer tasks provide an important contrast
%     \item We provide an interpretable explanation of when context helps: context appears most useful when MT2 must perform richer \textbf{semantic realization}, which is especially common in culturally grounded tasks
% \end{itemize}

% \subsection{Paper overview}
% \begin{itemize}
%     \item We compare three systems: a standard cascade, a context-aware cascade, and an end-to-end target-language baseline
%     \item We evaluate them on both culturally grounded and non-cultural datasets, using standard \textbf{chrF} and \textbf{accuracy} metrics, normalized so that results can be compared across tasks
%     \item We then perform simple analyses of task regime, resource level, and dataset type to understand when context helps and when it does not
% \end{itemize}




==> latex/main_text/2-related.tex <==
\NB{Look at the 12 related works I listed on the original google doc and look for new work if necessary, and summarize into one coherent paragraph with the following points.}
\begin{itemize}
    \item Several prior work presents a translation cascade approach as a strong competitor with end-to-end multilingual systems \NB{cite}.
    \item This has been shown for various tasks and settings in NLP, like retrieval \NB{cite}, natural language understanding \NB{cite},...
    \item A long line of work describes the vulnerability of various cascaded systems to error propagation \NB{look for a bunch of works, you should find things especially in ASR speech literature}. \NB{Is Translation All you need} show that the translate cascade is less useful on inputs requiring cultural content. \NB{double check if this is true, if not find the paper that does this.} 
    \item We are the first to introduce and study the benefits of context-aware cascade, which shows potential in countering the general problem of error propagation in cascaded systems.
\end{itemize}

==> latex/main_text/3-method.tex <==
a whole figure is needed for the method
\subsection{Cascade Variants}
We compare three systems that differ only in how information flows
between the translation and reasoning stages.

\paragraph{Standard cascade ($\mathrm{C}_{\text{std}}$).}
MT1 translates $q_t$ into English to obtain $q_e$. The reasoning model
then produces an English chain-of-thought $r_e$ and an English answer
$a_e$ conditioned only on $q_e$. Finally, MT2 translates $a_e$ back into
$t$, conditioned only on $a_e$:
\[
q_e = \mathrm{MT1}(q_t)
\]
\[
(r_e, a_e) = \mathrm{Reason}(q_e), \quad
\]
\[
a_t = \mathrm{MT2}(a_e).
\]
This represents the common practice of treating translation as a
self-contained pre- and post-processing step around an English-only
reasoner.

\paragraph{Context-aware cascade ($\mathrm{C}_{\text{ctx}}$).}
The first two stages are identical to $\mathrm{C}_{\text{std}}$. The
only change is that MT2 is conditioned on the full upstream context
rather than on $a_e$ alone:
\[
a_t = \mathrm{MT2}(q_t,\; q_e,\; r_e,\; a_e).
\]
The motivation is that $a_e$ is often a short span---a named entity, a
number with units, or a multiple-choice letter---whose correct surface
form in $t$ depends on information that has been discarded by the time
MT2 runs. Examples include the grammatical gender or register implied by
$q_t$, the unit conventions made explicit only in $r_e$, and the mapping
between option letters and their target-language phrasings. Exposing
MT2 to $(q_t, q_e, r_e, a_e)$ lets it resolve such ambiguities without
changing the reasoning model itself.

\paragraph{End-to-end baseline ($\mathrm{E2E}$).}
As a reference point we also evaluate direct target-language generation
without any explicit translation stage: the same Llama-3.1-8B-Instruct
model receives $q_t$ and is prompted to reason and answer in $t$. This
isolates the contribution of the cascade structure relative to letting
the model operate natively in the target language.

==> latex/main_text/4-exp.tex <==
\subsection{Models}
We use \textbf{Llama-3.1-8B-Instruct}~\NB{cite} adn \textbf{Qwen2.5-7B-Instruct} as the
backbone for every component of every system in this work. \nb{We have no other model results? This will be a problem for reviewers i.e. seeing just one model. It's okay to say even have some subset of main experiments on 2-3 other models even if main analysis on only 1.} The
same checkpoint plays three roles depending on the prompt it receives:
(i) a forward translator MT1 that maps $q_t \to q_e$, (ii) a reasoner
that produces $(r_e, a_e)$ from $q_e$, and (iii) a back-translator MT2
that produces $a_t$. Using one model across all roles is deliberate: it
isolates the effect of the \emph{pipeline structure} from confounds
introduced by mixing model families of different capabilities, and it
matches a realistic deployment in which a single multilingual LLM is
served behind one endpoint. All components use greedy decoding with
temperature $0$; the prompts used for translation, reasoning, and
end-to-end generation are listed in Appendix~\ref{app:prompts}.

\subsection{Datasets}
We evaluate on a range of multilingual benchmarks grouped here by output regime, requiring various types and levels of reasoning, translation precision, and cultural context.
\NB{For any dataset where you are doing anything nonstandard, like treating global piqa as longform/MCQ, explain. Use the normal name for the standard form.}
\begin{itemize}
    \item \textbf{Open-ended answer generation:}
    Aya Dataset, MKQA, BLEnD, and Global-PIQA~\NB{cite:
    {aya,mkqa,blend,globalpiqa}} require free-form target-language
    answers. \NB{so and so datasets include items that may require cultural grounding, ...}

    \item \textbf{Multiple-choice and constrained QA:}
    Global-MMLU, MCSQA, Belebele, and Global-PIQA-MC~\NB{cite:
    {globalmmlu,mcsqa,belebele,globalpiqamc}} require selecting or
    producing an answer from a constrained set of options.

    \item \textbf{Math and exact-answer reasoning:}
    MGSM and MMath~\NB{cite: {mgsm,mmath}} require numerical reasoning and
    exact final answers. 
\end{itemize}

See a short description of each dataset in \NB{@Dengjia appendix table with dataset, full name, number of languages, main relevant characteristics}.

\subsection{Languages}

We evaluate on all languages supported by each dataset, resulting in a total of \NB{todo} languages over all datasets.
\NB{We categorize them into high, mid, and low-resource languages by... say how you did this.}
We provide a full list of languages in \NB{@Dengjia list of languages with datasets as columns, with a tick if supported. you could also just have a list of languages per dataset.}

% We evaluate on three families of tasks that stress different
% capabilities of the pipeline.

% \begin{itemize}
% \item \textbf{Open-ended QA:} Global-PIQA, MKQA, and
% Aya~\NB{cite: {globalpiqa,mkqa,aya}}, which require generating
% free-form answers and are sensitive to surface-form fidelity in $t$.
% \item \textbf{Multiple choice:} Global-MMLU, MCSQA, and
% Belebele~\NB{cite: {globalmmlu,mcsqa,belebele}}, which test whether
% the cascade preserves the mapping between options and the chosen answer.
% \item \textbf{Math:} MMath and MGSM~\NB{cite: {mmath,mgsm}}, which
% stress the reasoning stage and depend on faithful translation of
% numerical quantities and units.
% \end{itemize}

% We evaluate on datasets spanning different \textbf{task types} and
% different degrees of \textbf{cultural grounding}.

% \begin{itemize}
% \item \textbf{Task types}
% \begin{itemize}
%     \item \textbf{Open-ended QA:} Global-PIQA, MKQA, Aya, and
%     BLEnD~\NB{cite: {globalpiqa,mkqa,aya,blend}}, which require generating
%     free-form answers and are sensitive to surface-form fidelity in $t$
%     \item \textbf{Multiple choice:} Global-PIQA-MC, Global-MMLU, MCSQA, and
%     Belebele~\NB{cite: {globalpiqamc,globalmmlu,mcsqa,belebele}}, which test whether
%     the cascade preserves the mapping between options and the chosen answer
%     \item \textbf{Math:} MMath and MGSM~\NB{cite: {mmath,mgsm}}, which
%     stress the reasoning stage and depend on faithful translation of
%     numerical quantities and units
% \end{itemize}

% \item \textbf{Cultural grounding}
% \begin{itemize}
%     \item \textbf{Culturally grounded:} Aya (our culturally grounded subset),
%     BLEnD, Global-PIQA, and Global-PIQA-MC
%     \item \textbf{Non-cultural contrasts:} MKQA, Global-MMLU, MCSQA,
%     Belebele, MMath, and MGSM
% \end{itemize}
% \end{itemize}

% This two-axis grouping lets us separate effects of \textit{task regime}
% from effects of \textit{cultural grounding}, which partially overlap in
% our benchmark set.

\subsection{Evaluation}
For multiple-choice tasks we report \textbf{accuracy} against the gold
option after extracting the predicted choice from $a_t$ with a
deterministic parser over option letters and their target-language
equivalents (details in Appendix~\ref{app:parsing}). For open-ended QA
we report \textbf{chrF} between $a_t$ and the reference answer in $t$, computed as a character $n$-gram F-score after Unicode NFKC normalization and lowercasing, which is better suited than token-level overlap metrics for multilingual generation because it is less sensitive to tokenization differences across languages~\NB{cite: {chrf}}. For
math tasks we report \textbf{exact-match accuracy} on the final
numerical answer extracted from $a_t$, treating answers as equal after
stripping units and normalizing decimal separators (e.g., ``1,5'' vs.\
``1.5''). All numbers are averaged over the full evaluation split of
each dataset.



==> latex/main_text/5-results.tex <==
\NB{@Dengjia: make the main results figure. try bar plot with averages per resource regime for each dataset. check out figure 5 in https://aclanthology.org/2025.ijcnlp-long.83.pdf for inspiration.}
We also provide more detailed results per language in \NB{@Dengjia appendix tables}

\paragraph{Overall winner}

Broadly,...

\paragraph{Cultural grounding}

We look at the group of datasets that need cultural grounding: specifically, ... , as opposed to... We find that...

\paragraph{Resourcedness and typology of target language}
\NB{@Arnav: 1-2 small figures making the targeted points you want, if need.}
\begin{itemize}
    \item We further test whether the advantage of Context is simply a high-resource effect
    \item Instead, in the regimes where Context helps, it remains competitive or superior across resource levels
    \item This suggests that resource alone does not explain the main pattern; the broader task regime is more important
\end{itemize}

% Placeholder: main table of dataset-level results
% \input{latex/tables/main_results_table}

% \subsection{Cultural versus non-cultural regimes}
% \begin{itemize}
%     \item When we group datasets by regime, the strongest gains for Context appear in the culturally grounded group
%     \item This supports the view that extra MT2 context is most useful when target-language generation requires richer semantic realization rather than literal answer transfer alone
%     \item The non-cultural datasets serve as a contrast set and help show that the effect is regime-specific rather than a general property of all multilingual tasks
% \end{itemize}

% Placeholder: grouped summary figure/table
% \input{latex/tables/cultural_vs_noncultural_summary}
% \includegraphics[width=\linewidth]{figures/cultural_vs_noncultural.png}



% Placeholder: resource-bucket figure
% \includegraphics[width=\linewidth]{figures/context_by_resource.png}


==> latex/main_text/6-analysis.tex <==

\subsection{Interpreting the advantage of context}
\begin{itemize}
    \item Our basic analyses are intended to explain \textit{when} context helps rather than to maximize predictive accuracy
    \item The main qualitative pattern is that context is most useful when MT2 must perform richer semantic realization, which is especially common in culturally grounded tasks
    \item In contrast, exact-answer tasks provide a natural failure case, suggesting that extra context can be less useful when the output must be tightly preserved
\end{itemize}

% Placeholder: interpretable model figure
% \includegraphics[width=\linewidth]{figures/context_interpretability.png}

\subsection{What this suggests about context-aware MT2}
\begin{itemize}
    \item We do not view context-aware MT2 as a universal upgrade to multilingual cascades
    \item Instead, our results suggest that it is a \textbf{regime-dependent technique}: it is strongest in culturally grounded settings, remains robust across resource levels in those settings, and weakens in non-cultural or exact-answer regimes
\end{itemize}

==> latex/main_text/7-conclusion.tex <==
\begin{itemize}
    \item Context-aware MT2 is not a universal improvement to multilingual cascades
    \item Its strongest gains appear in culturally grounded multilingual tasks, where richer context appears to help target-language semantic realization
    \item This advantage is not confined to high-resource settings; in the regimes where Context helps, it remains competitive or superior across resource levels
    \item At the same time, non-cultural and exact-answer tasks show that the benefit is regime-specific rather than universal
    \item More broadly, our results suggest that multilingual cascade design should be evaluated with attention to \textbf{task regime}, not only aggregate score improvements
\end{itemize}

==> latex/main_text/81-results.tex <==
\onecolumn

\input{latex/tables/llama/global_mmlu}
\input{latex/tables/llama/MCSQA}
\input{latex/tables/llama/belebele}
\input{latex/tables/llama/piqa}   
\input{latex/tables/llama/mgsm}
\input{latex/tables/llama/mmath}

\input{latex/tables/qwen/global_mmlu}
\input{latex/tables/qwen/mcsqa}
\input{latex/tables/qwen/belebele}
\input{latex/tables/qwen/piqa}   
\input{latex/tables/qwen/mgsm}
\input{latex/tables/qwen/mmath}

\input{latex/tables/aya}
\input{latex/tables/blend}
\input{latex/tables/global_piqa_oe}
\input{latex/tables/mkqa}


==> latex/plots/1_correlation_plots.tex <==
\clearpage
\begin{figure}[p]
\centering
\includegraphics[width=\textwidth]{latex/plots/llama_corrs.pdf}
\caption{Llama Normalized scores, Context - Standard vs. Standard and End-to-End, colored by resource level. Context helps performance at lower Standard/End-to-End scores and resource levels}
\label{fig:ctxstd-resource}
\end{figure}



\begin{figure}[p]
\centering
\includegraphics[width=\textwidth]{latex/plots/qwen_corrs.pdf}
\caption{Qwen Normalized scores, Context - Standard vs. Standard and End-to-End, colored by resource level. Context helps performance at lower Standard/End-to-End scores and resource levels}
\label{fig:ctxstd-resource}
\end{figure}






\clearpage
% \begin{figure}[p]
% \centering
% \includegraphics[width=\textwidth]{latex/plots/llama_cultural_std_cxt_resource}
% \caption{Llama Context - Standard over language resource score.}
% \label{fig:ctxstd-resource}
% \end{figure}



% \begin{figure}[p]
% \centering
% \includegraphics[width=\textwidth]{latex/plots/llama_other_std_cxt_resource.pdf}
% \caption{Llama Context - Standard over language resource score.}
% \label{fig:ctxstd-resource}
% \end{figure}

% \clearpage


% \begin{figure}[p]
% \centering
% \includegraphics[width=\textwidth]{latex/plots/llama_cultural_e2e_cxt_resource}
% \caption{Llama Context - End-to-End over language resource score.}
% \label{fig:ctxstd-resource}
% \end{figure}



% \begin{figure}[p]
% \centering
% \includegraphics[width=\textwidth]{latex/plots/llama_other_e2e_cxt_resource.pdf}
% \caption{Llama Context - End-to-End over language resource score.}
% \label{fig:ctxstd-resource}
% \end{figure}

% \clearpage

% \begin{figure}[p]
% \centering
% \includegraphics[width=\textwidth]{latex/plots/qwen_cultural_std_cxt_resource.pdf}
% \caption{Qwen Context - Standard over language resource score.}
% \label{fig:ctxstd-resource}
% \end{figure}



% \begin{figure}[p]
% \centering
% \includegraphics[width=\textwidth]{latex/plots/qwen_other_std_cxt_resource.pdf}
% \caption{Qwen Context - Standard over language resource score.}
% \label{fig:ctxstd-resource}
% \end{figure}


% \clearpage


% \begin{figure}[p]
% \centering
% \includegraphics[width=\textwidth]{latex/plots/qwen_cultural_e2e_cxt_resource.pdf}
% \caption{Qwen Context - End-to-End over language resource score.}
% \label{fig:ctxstd-resource}
% \end{figure}



% \begin{figure}[p]
% \centering
% \includegraphics[width=\textwidth]{latex/plots/qwen_other_e2e_cxt_resource.pdf}
% \caption{Qwen Context - End-to-End over language resource score.}
% \label{fig:ctxstd-resource}
% \end{figure}


% \clearpage





==> latex/plots/2_decision_trees.tex <==
\clearpage
\begin{figure}[p]
\centering
\includegraphics[width=\textwidth]{latex/plots/llama_cxt_vs_std_tree.pdf}
\caption{Decision tree to predict Context - Standard scores for Llama using all available features.}
\label{fig:llama-ctxstd-tree}
\end{figure}



\begin{figure}[p]
\centering
\includegraphics[width=\textwidth]{latex/plots/llama_cxt_vs_std_tree_no_resource.pdf}
\caption{Decision tree to predict Context - Standard scores for Llama omitting resource score.}
\label{fig:llama-ctxstd-no-resource-tree}
\end{figure}

\clearpage


\begin{figure}[p]
\centering
\includegraphics[width=\textwidth]{latex/plots/llama_cxt_vs_e2e_tree.pdf}
\caption{Decision tree to predict Context - End-to-End scores for Llama using all available features.}
\label{fig:llama-ctxe2e-tree}
\end{figure}



\begin{figure}[p]
\centering
\includegraphics[width=\textwidth]{latex/plots/llama_cxt_vs_e2e_tree_no_resource.pdf}
\caption{Decision tree to predict Context - End-to-End scores for Llama omitting resource score.}
\label{fig:llama-ctxe2e-no-resource-tree}
\end{figure}

\clearpage







\begin{figure}[p]
\centering
\includegraphics[width=\textwidth]{latex/plots/qwen_cxt_vs_std_tree.pdf}
\caption{Decision tree to predict Context - Standard scores for Qwen using all available features.}
\label{fig:qwen-ctxstd-tree}
\end{figure}



\begin{figure}[p]
\centering
\includegraphics[width=\textwidth]{latex/plots/qwen_cxt_vs_std_tree_no_resource.pdf}
\caption{Decision tree to predict Context - Standard scores for Qwen omitting resource score.}
\label{fig:qwen-ctxstd-no-resource-tree}
\end{figure}

\clearpage


\begin{figure}[p]
\centering
\includegraphics[width=\textwidth]{latex/plots/qwen_cxt_vs_e2e_tree.pdf}
\caption{Decision tree to predict Context - End-to-End scores for Qwen using all available features.}
\label{fig:qwen-ctxe2e-tree}
\end{figure}



\begin{figure}[p]
\centering
\includegraphics[width=\textwidth]{latex/plots/qwen_cxt_vs_e2e_tree_no_resource.pdf}
\caption{Decision tree to predict Context - End-to-End scores for Qwen omitting resource score.}
\label{fig:qwen-ctxe2e-no-resource-tree}
\end{figure}

\clearpage

==> latex/plots/3_normalized_radars.tex <==
\clearpage
\begin{figure}[p]
\centering
\includegraphics[width=\textwidth]{latex/plots/llama_script_method_radar_top_coverage.pdf}
\caption{Llama, Mean normalized scores for top 3 most frequent language scripts among all benchmarks.}
\label{fig:ctxstd-resource}
\end{figure}



\begin{figure}[p]
\centering
\includegraphics[width=\textwidth]{latex/plots/llama_family_method_radar_top_coverage.pdf}
\caption{LLam, Mean normalized scores for top 6 most frequent language families among all benchmarks.}
\label{fig:ctxstd-resource}
\end{figure}

\clearpage


\begin{figure}[p]
\centering
\includegraphics[width=\textwidth]{latex/plots/llama_genus_method_radar_top_coverage.pdf}
\caption{LLama, Mean normalized scores for top 6 most frequent language genera among all benchmarks.}
\label{fig:ctxstd-resource}
\end{figure}



\begin{figure}[p]
\centering
\includegraphics[width=\textwidth]{latex/plots/llama_task_method_radar.pdf}
\caption{LLama, Mean normalized scores for each task among all benchmarks.}
\label{fig:ctxstd-resource}
\end{figure}

\clearpage



\begin{figure}[p]
\centering
\includegraphics[width=\textwidth]{latex/plots/qwen_script_method_radar_top_coverage.pdf}
\caption{Qwen, Mean normalized scores for top 3 most frequent language scripts among all benchmarks.}
\label{fig:ctxstd-resource}
\end{figure}



\begin{figure}[p]
\centering
\includegraphics[width=\textwidth]{latex/plots/qwen_family_method_radar_top_coverage.pdf}
\caption{Qwen, Mean normalized scores for top 6 most frequent language families among all benchmarks.}
\label{fig:ctxstd-resource}
\end{figure}


\clearpage

\begin{figure}[p]
\centering
\includegraphics[width=\textwidth]{latex/plots/qwen_genus_method_radar_top_coverage.pdf}
\caption{Qwen, Mean normalized scores for top 6 most frequent language genera among all benchmarks.}
\label{fig:ctxstd-resource}
\end{figure}


\begin{figure}[p]
\centering
\includegraphics[width=\textwidth]{latex/plots/qwen_task_method_radar.pdf}
\caption{Qwen, Mean normalized scores for each task among all benchmarks.}
\label{fig:ctxstd-resource}
\end{figure}

\clearpage




==> latex/tables/aya.tex <==
% \begin{table}[t]
% \centering
% \small
% \begin{tabular}{lccc}
% \toprule
% \textbf{Language} & \textbf{Standard} & \textbf{Context} & \textbf{End-to-end} \\
% \midrule
% Telugu & 3.36 & 5.09 & \textbf{8.19} \\
% Yoruba & 2.86 & 2.50 & \textbf{3.51} \\
% Arabic & 9.25 & \textbf{11.21} & 9.18 \\
% Turkish & 15.41 & \textbf{18.02} & 17.67 \\
% Portuguese & 22.52 & 26.79 & \textbf{26.96} \\
% Chinese & 4.87 & 8.35 & \textbf{10.12} \\
% \midrule
% \textbf{Avg} & 9.71 & 11.99 & \textbf{12.61} \\
% \bottomrule
% \end{tabular}
% \caption{chrF scores on Aya using Mistral across standard, context, and end-to-end.}
% \label{tab:aya-mistral-chrf}
% \end{table}



\begin{table}[t]
\centering
\small
\begin{tabular}{lccc}
\toprule
\textbf{Language} & \textbf{Standard} & \textbf{Context} & \textbf{End-to-end} \\
\midrule
Telugu & 12.67 & 14.15 & 10.95 \\
Yoruba & 3.54 & 4.05 & \textbf{6.13} \\
Arabic & 14.51 & 15.89 & \textbf{17.59} \\
Turkish & 18.86 & 20.00 & \textbf{22.84} \\
Portuguese & 25.17 & 25.97 & \textbf{26.08} \\
Chinese & \textbf{13.16} & 13.04 & 12.18 \\
\bottomrule
\end{tabular}
\caption{chrF scores on Aya using GPT across standard, context, and end-to-end.}
\label{tab:aya-gpt-chrf}
\end{table}





% \begin{table}[t]
% \centering
% \small
% \begin{tabular}{lccc}
% \toprule
% \textbf{Language} & \textbf{Standard} & \textbf{Context} & \textbf{End-to-end} \\
% \midrule
% Telugu & 7.93 & \textbf{11.09} & 11.01 \\
% Yoruba & 1.66 & 2.11 & \textbf{2.55} \\
% Arabic & 8.67 & \textbf{13.63} & 9.43 \\
% Turkish & 14.33 & \textbf{20.94} & 15.64 \\
% Portuguese & 19.72 & \textbf{27.29} & 22.54 \\
% Chinese & 5.02 & \textbf{10.49} & 6.46 \\
% \bottomrule
% \end{tabular}
% \caption{chrF scores on Aya using Llama across standard, context, and end-to-end.}
% \label{tab:aya-llama-chrf}
% \end{table}



% \begin{table}[t]
% \centering
% \small
% \begin{tabular}{lccc}
% \toprule
% \textbf{Language} & \textbf{Standard} & \textbf{Context} & \textbf{End-to-end} \\
% \midrule
% Telugu & 7.80 & 9.59 & \textbf{12.95} \\
% Yoruba & 1.71 & 2.78 & \textbf{3.06} \\
% Arabic & 10.05 & 12.79 & \textbf{13.88} \\
% Turkish & 15.74 & \textbf{19.70} & 16.27 \\
% Portuguese & 25.26 & \textbf{28.84} & 25.32 \\
% Chinese & 7.50 & 10.30 & \textbf{14.56} \\
% \bottomrule
% \end{tabular}
% \caption{chrF scores on Aya using Qwen across standard, context, and end-to-end.}
% \label{tab:aya-qwen-chrf}
% \end{table}






% \begin{table}[t]
% \centering
% \small
% \begin{tabular}{lccc}
% \toprule
% \textbf{Language} & \textbf{Standard} & \textbf{Context} & \textbf{End-to-end} \\
% \midrule
% Telugu & 7.93 & \textbf{11.10} & 11.01 \\
% Yoruba & 1.60 & 2.04 & \textbf{2.45} \\
% Arabic & 8.67 & \textbf{13.63} & 9.43 \\
% Turkish & 13.95 & \textbf{20.32} & 15.20 \\
% Portuguese & 19.25 & \textbf{26.68} & 21.98 \\
% Chinese & 5.01 & \textbf{10.48} & 6.45 \\
% \bottomrule
% \end{tabular}
% \caption{chrF scores on Aya using Llama across standard, context, and end-to-end.}
% \label{tab:aya-llama-chrf}
% \end{table}



% \begin{table}[t]
% \centering
% \small
% \begin{tabular}{lccc}
% \toprule
% \textbf{Language} & \textbf{Standard} & \textbf{Context} & \textbf{End-to-end} \\
% \midrule
% Telugu & 7.80 & 9.59 & \textbf{12.95} \\
% Yoruba & 1.66 & 2.69 & \textbf{2.96} \\
% Arabic & 10.05 & 12.79 & \textbf{13.87} \\
% Turkish & 15.29 & \textbf{19.15} & 15.77 \\
% Portuguese & 24.73 & \textbf{28.22} & 24.55 \\
% Chinese & 7.48 & 10.25 & \textbf{14.51} \\
% \bottomrule
% \end{tabular}
% \caption{chrF scores on Aya using Qwen across standard, context, and end-to-end.}
% \label{tab:aya-qwen-chrf}
% \end{table}


% \begin{table}[t]
% \centering
% \small
% \begin{tabular}{lccc}
% \toprule
% \textbf{Language} & \textbf{Standard} & \textbf{Context} & \textbf{End-to-end} \\
% \midrule
% Telugu & 11.31 & 24.99 & \textbf{25.55} \\
% Yoruba & 3.16 & 5.74 & \textbf{10.73} \\
% Arabic & 10.07 & \textbf{19.10} & 16.91 \\
% Turkish & 16.74 & 26.32 & \textbf{26.38} \\
% Portuguese & 23.86 & \textbf{33.94} & 32.58 \\
% Chinese & 6.47 & \textbf{12.94} & 12.82 \\
% \bottomrule
% \end{tabular}
% \caption{chrF scores on Aya using GPT across standard, context, and end-to-end.}
% \label{tab:aya-gpt-chrf}
% \end{table}

==> latex/tables/blend.tex <==
% \begin{table}[t]
% \centering
% \small
% \setlength{\tabcolsep}{5pt}
% \begin{tabular}{lccc}
% \toprule
% \textbf{Language} & \textbf{Standard} & \textbf{Context} & \textbf{End-to-end} \\
% \midrule
% Chinese (Simplified) & 6.03 & 7.53 & \textbf{8.37} \\
% Spanish (Spain) & 15.81 & 16.52 & \textbf{17.41} \\
% Spanish (Mexico) & 15.29 & \textbf{16.89} & 16.06 \\
% Indonesian & 13.16 & \textbf{13.18} & 13.09 \\
% Korean (South Korea) & 4.43 & \textbf{5.33} & 4.41 \\
% Korean (North Korea) & 1.85 & 3.64 & \textbf{4.34} \\
% Greek & 10.65 & \textbf{11.28} & 5.68 \\
% Persian & \textbf{9.16} & 9.15 & 5.52 \\
% Arabic (Algeria) & 10.47 & \textbf{10.80} & 5.23 \\
% Azerbaijani & 8.81 & \textbf{9.31} & 6.83 \\
% Javanese & 8.95 & \textbf{9.24} & 5.86 \\
% Assamese & 6.16 & \textbf{7.74} & 2.49 \\
% Hausa & 3.66 & 3.54 & \textbf{3.84} \\
% Amharic & 1.39 & \textbf{2.51} & 0.82 \\
% \midrule
% \textbf{Avg} & 8.27 & \textbf{9.05} & 7.14 \\
% \bottomrule
% \end{tabular}
% \caption{chrF scores on BLEnD using Mistral across standard, context, and end-to-end.}
% \label{tab:blend-mistral-chrf}
% \end{table}



\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{lccc}
\toprule
\textbf{Language} & \textbf{Standard} & \textbf{Context} & \textbf{End-to-end} \\
\midrule
Chinese (Simplified) & 12.02 & 9.76 & \textbf{25.09} \\
Spanish (Spain) & \textbf{29.85} & 27.00 & 23.59 \\
Spanish (Mexico) & 26.58 & \textbf{27.03} & 23.13 \\
Indonesian & 22.08 & 22.30 & \textbf{29.09} \\
Korean (South Korea) & 10.56 & 9.29 & \textbf{12.64} \\
Korean (North Korea) & 5.29 & \textbf{6.41} & 6.34 \\
Greek & 23.03 & 22.35 & \textbf{33.68} \\
Persian & 19.82 & 19.57 & \textbf{33.67} \\
Arabic (Algeria) & 18.47 & 19.93 & \textbf{28.70} \\
Azerbaijani & 21.03 & 20.64 & \textbf{25.89} \\
Javanese & 17.20 & 16.57 & \textbf{25.53} \\
Assamese & 13.93 & 13.78 & \textbf{21.22} \\
Hausa & 17.35 & \textbf{17.64} & 15.57 \\
Amharic & 4.38 & \textbf{9.38} & 5.31 \\
\bottomrule
\end{tabular}
\caption{chrF scores on BLEnD using GPT across standard, context, and end-to-end.}
\label{tab:blend-gpt-chrf}
\end{table}


% \begin{table}[t]
% \centering
% \small
% \begin{tabular}{lccc}
% \toprule
% \textbf{Language} & \textbf{Standard} & \textbf{Context} & \textbf{End-to-end} \\
% \midrule
% Chinese (Simplified) & 5.23 & 8.95 & \textbf{26.31} \\
% Spanish (Spain) & 14.97 & \textbf{18.01} & 13.79 \\
% Spanish (Mexico) & 14.94 & \textbf{16.66} & 14.70 \\
% Indonesian & 13.27 & \textbf{16.63} & 12.11 \\
% Korean (South Korea) & 6.42 & 8.43 & \textbf{11.29} \\
% Korean (North Korea) & 2.95 & \textbf{5.71} & 5.32 \\
% Greek & 11.50 & \textbf{14.23} & 13.32 \\
% Persian & 11.72 & \textbf{13.58} & 12.88 \\
% Arabic (Algeria) & 11.82 & \textbf{12.82} & 12.13 \\
% Azerbaijani & 10.20 & \textbf{15.07} & 13.04 \\
% Javanese & 9.74 & \textbf{13.45} & 9.93 \\
% Assamese & 9.08 & \textbf{11.79} & 11.17 \\
% Hausa & 6.20 & \textbf{9.04} & 6.77 \\
% Amharic & 4.59 & \textbf{5.65} & 4.05 \\
% \bottomrule
% \end{tabular}
% \caption{chrF scores on BLEnD using Llama across standard, context, and end-to-end.}
% \label{tab:blend-llama-chrf}
% \end{table}





% \begin{table}[t]
% \centering
% \small
% \begin{tabular}{lccc}
% \toprule
% \textbf{Language} & \textbf{Standard} & \textbf{Context} & \textbf{End-to-end} \\
% \midrule
% Chinese (Simplified) & 14.61 & 13.77 & \textbf{32.75} \\
% Spanish (Spain) & \textbf{24.10} & 23.90 & 18.78 \\
% Spanish (Mexico) & \textbf{25.62} & 24.07 & 17.50 \\
% Indonesian & 19.52 & 18.58 & \textbf{24.63} \\
% Korean (South Korea) & 12.23 & 12.52 & \textbf{16.36} \\
% Korean (North Korea) & 5.09 & 6.89 & \textbf{8.34} \\
% Greek & 15.51 & \textbf{16.28} & 7.22 \\
% Persian & 12.73 & \textbf{12.93} & 6.23 \\
% Arabic (Algeria) & 14.96 & 16.40 & \textbf{16.72} \\
% Azerbaijani & 11.36 & \textbf{11.61} & 6.82 \\
% Javanese & \textbf{12.94} & 10.89 & 10.68 \\
% Assamese & 9.68 & \textbf{11.77} & 7.23 \\
% Hausa & \textbf{7.93} & 5.44 & 5.37 \\
% Amharic & 2.24 & \textbf{4.10} & 2.44 \\
% \bottomrule
% \end{tabular}
% \caption{chrF scores on BLEnD using Qwen across standard, context, and end-to-end.}
% \label{tab:blend-qwen-chrf}
% \end{table}





% \begin{table}[t]
% \centering
% \small
% \begin{tabular}{lccc}
% \toprule
% \textbf{Language} & \textbf{Standard} & \textbf{Context} & \textbf{End-to-end} \\
% \midrule
% Chinese & 5.15 & 8.91 & \textbf{26.35} \\
% Spanish (Spain) & 13.93 & \textbf{16.91} & 13.13 \\
% Spanish (Mexico) & 13.77 & \textbf{15.74} & 13.82 \\
% Indonesian & 11.71 & \textbf{14.32} & 10.13 \\
% Korean (South Korea) & 6.40 & 8.35 & \textbf{11.20} \\
% Korean (North Korea) & 2.95 & \textbf{5.71} & 5.32 \\
% Greek & 10.98 & \textbf{13.74} & 12.84 \\
% Persian & 11.72 & \textbf{13.58} & 12.88 \\
% Arabic & 11.82 & \textbf{12.82} & 12.13 \\
% Azerbaijani & 9.26 & \textbf{13.70} & 11.24 \\
% Javanese & 9.00 & \textbf{11.98} & 8.32 \\
% Assamese & 8.80 & \textbf{11.42} & 10.85 \\
% Hausa & 5.88 & \textbf{8.48} & 6.05 \\
% Amharic & 4.59 & \textbf{5.65} & 4.05 \\
% \bottomrule
% \end{tabular}
% \caption{chrF scores on BLEnD using Llama across standard, context, and end-to-end.}
% \label{tab:blend-llama-chrf}
% \end{table}



% \begin{table}[t]
% \centering
% \small
% \begin{tabular}{lccc}
% \toprule
% \textbf{Language} & \textbf{Standard} & \textbf{Context} & \textbf{End-to-end} \\
% \midrule
% Chinese (Simplified) & 14.47 & 13.69 & \textbf{31.62} \\
% Spanish (Spain) & \textbf{22.23} & 21.87 & 18.00 \\
% Spanish (Mexico) & \textbf{22.96} & 21.74 & 16.44 \\
% Indonesian & 16.79 & 15.78 & \textbf{21.09} \\
% Korean (South Korea) & 12.25 & 12.52 & \textbf{16.19} \\
% Korean (North Korea) & 5.09 & 6.89 & \textbf{8.34} \\
% Greek & 14.86 & \textbf{15.78} & 7.00 \\
% Persian & 12.73 & \textbf{12.93} & 6.23 \\
% Arabic (Algeria) & 14.96 & 16.40 & \textbf{16.72} \\
% Azerbaijani & 10.57 & \textbf{10.69} & 6.39 \\
% Javanese & \textbf{11.64} & 9.73 & 9.33 \\
% Assamese & 9.32 & \textbf{11.30} & 7.01 \\
% Hausa & \textbf{7.40} & 5.10 & 5.18 \\
% Amharic & 2.24 & \textbf{4.10} & 2.44 \\
% \bottomrule
% \end{tabular}
% \caption{chrF scores on BLEnD using Qwen across standard cascade, context, and end-to-end.}
% \label{tab:blend-qwen-chrf}
% \end{table}

==> latex/tables/global_piqa_oe.tex <==

% \clearpage
% \begin{table}[p]
% \centering
% \scriptsize
% \setlength{\tabcolsep}{4pt}
% \begin{tabular}{p{0.50\textwidth}ccc}
% \toprule
% \textbf{Language} & \textbf{Standard} & \textbf{Context} & \textbf{End-to-end} \\
% \midrule
% Mesopotamian Arabic (Arabic script) & 12.67 & \textbf{14.31} & 5.13 \\
% Taizzi-Adeni Arabic (Arabic script) & 13.65 & \textbf{16.13} & 5.27 \\
% Tunisian Arabic (Arabic script) & 12.79 & \textbf{13.66} & 5.48 \\
% Gulf Arabic (Arabic script) & 11.47 & \textbf{12.41} & 5.65 \\
% Tosk Albanian (Latin script) & 13.28 & \textbf{14.24} & 12.54 \\
% Levantine Arabic (Jordan) & 15.56 & \textbf{17.53} & 10.06 \\
% Levantine Arabic (Lebanon) & 12.53 & \textbf{12.77} & 5.47 \\
% Levantine Arabic (Palestine) & 11.06 & \textbf{11.55} & 5.06 \\
% Levantine Arabic (Syria) & 11.82 & \textbf{12.83} & 6.02 \\
% Algerian Arabic (Arabic script) & \textbf{12.25} & 12.00 & 5.37 \\
% Najdi Arabic (Arabic script) & 15.86 & \textbf{17.24} & 7.73 \\
% Moroccan Arabic (Arabic script) & 12.14 & \textbf{12.48} & 5.77 \\
% Egyptian Arabic (Arabic script) & 14.01 & \textbf{15.06} & 5.79 \\
% Bambara (Latin script) & 5.91 & \textbf{9.91} & 9.78 \\
% Belarusian (Cyrillic script) & 12.64 & \textbf{18.36} & 15.78 \\
% Bengali (Bengali script) & 8.86 & \textbf{10.40} & 4.61 \\
% Bengali (Latin script) & 7.00 & 4.92 & \textbf{11.54} \\
% Bhojpuri (Devanagari script) & 8.57 & \textbf{10.07} & 5.98 \\
% Bosnian (Latin script) & \textbf{23.91} & 23.53 & 21.04 \\
% Burushaski (Arabic script) & 2.92 & \textbf{5.28} & 3.64 \\
% Bulgarian (Cyrillic script) & 23.91 & \textbf{24.04} & 20.38 \\
% Catalan (Latin script) & 20.56 & \textbf{21.41} & 17.68 \\
% Czech (Latin script) & 14.27 & \textbf{15.87} & 14.49 \\
% Central Kurdish (Arabic script) & 8.41 & \textbf{12.70} & 4.87 \\
% Chakma (Latin script) & 3.11 & 1.17 & \textbf{4.55} \\
% Mandarin Chinese (Traditional) & 2.87 & 7.00 & \textbf{9.21} \\
% German (Latin script) & 19.28 & \textbf{20.31} & 18.55 \\
% Dhundari (Devanagari script) & 7.45 & \textbf{10.25} & 4.92 \\
% Estonian (Latin script) & 14.14 & \textbf{14.62} & 9.94 \\
% \midrule
% \multicolumn{4}{r}{\emph{Continued in the next table.}} \\
% \bottomrule
% \end{tabular}
% \caption{chrF scores on Global-PIQA using Mistral across standard, context, and end-to-end.}
% \label{tab:global-piqa-mistral-chrf}
% \end{table}

% \begin{table}[p]
% \addtocounter{table}{-1}
% \centering
% \scriptsize
% \setlength{\tabcolsep}{4pt}
% \begin{tabular}{p{0.50\textwidth}ccc}
% \toprule
% \textbf{Language} & \textbf{Standard} & \textbf{Context} & \textbf{End-to-end} \\
% \midrule
% Ekpeye (Latin script) & 4.38 & 4.64 & \textbf{6.28} \\
% Greek (Greek script) & 10.08 & \textbf{11.00} & 10.36 \\
% English (Latin script) & 21.18 & 24.93 & \textbf{25.88} \\
% Faroese (Latin script) & 14.58 & \textbf{17.55} & 14.52 \\
% Finnish (Latin script) & 19.55 & \textbf{20.73} & 17.43 \\
% French (Canada) & 24.10 & \textbf{24.52} & 22.63 \\
% French (France) & 20.78 & \textbf{21.38} & 20.38 \\
% Galician (Latin script) & 18.64 & \textbf{22.22} & 20.07 \\
% Hausa (Latin script) & 9.90 & 9.48 & \textbf{10.45} \\
% Hawaiian (Latin script) & 11.99 & \textbf{16.53} & 12.62 \\
% Hebrew (Hebrew script) & 13.78 & \textbf{16.00} & 9.33 \\
% Hindi (Devanagari script) & 10.74 & \textbf{13.22} & 11.60 \\
% Croatian (Latin script) & \textbf{16.26} & 15.29 & 16.06 \\
% Hungarian (Latin script) & 21.76 & \textbf{21.96} & 17.07 \\
% Armenian (Armenian script) & 11.47 & 14.00 & \textbf{15.42} \\
% Igbo (Latin script) & 9.51 & \textbf{17.16} & 15.30 \\
% Idoma (Latin script) & 5.59 & 7.90 & \textbf{7.95} \\
% Indonesian (Latin script) & \textbf{22.96} & 22.88 & 21.92 \\
% Icelandic (Latin script) & 17.49 & \textbf{18.06} & 15.03 \\
% Isoko (Latin script) & 5.40 & \textbf{10.06} & 8.30 \\
% Italian (Latin script) & 18.80 & \textbf{22.88} & 21.24 \\
% Javanese (Latin script) & 15.19 & \textbf{15.59} & 11.69 \\
% Kannada (Kannada script) & 11.79 & 13.51 & \textbf{17.25} \\
% Georgian (Georgian script) & 10.30 & 11.56 & \textbf{11.52} \\
% Kazakh (Cyrillic script) & 11.74 & \textbf{13.33} & 11.81 \\
% Kinyarwanda (Latin script) & 9.55 & \textbf{12.44} & 11.07 \\
% Kyrgyz (Cyrillic script) & 11.23 & \textbf{10.99} & 9.47 \\
% Korean (Hangul script) & 3.34 & \textbf{5.02} & 3.83 \\
% Lingala (Latin script) & 9.86 & 11.56 & \textbf{11.97} \\
% \midrule
% \multicolumn{4}{r}{\emph{Continued in the next table.}} \\
% \bottomrule
% \end{tabular}
% \caption{chrF scores on Global-PIQA using Mistral across standard, context, and end-to-end. --- continued.}
% \end{table}

% \clearpage

% \begin{table}[p]
% \addtocounter{table}{-1}
% \centering
% \scriptsize
% \setlength{\tabcolsep}{4pt}
% \begin{tabular}{p{0.50\textwidth}ccc}
% \toprule
% \textbf{Language} & \textbf{Standard} & \textbf{Context} & \textbf{End-to-end} \\
% \midrule
% Lithuanian (Latin script) & 11.39 & \textbf{10.55} & 8.62 \\
% Luo (Latin script) & 9.01 & 10.18 & \textbf{11.71} \\
% Malayalam (Malayalam script) & 10.33 & 12.64 & \textbf{13.36} \\
% Meitei (Bengali script) & 2.65 & \textbf{2.88} & 1.89 \\
% Meitei (Meitei Mayek script) & 0.01 & \textbf{10.38} & 3.32 \\
% Naga Pidgin (Latin script) & 12.73 & \textbf{13.14} & 10.05 \\
% Dutch (Latin script) & \textbf{23.82} & 22.12 & 23.43 \\
% Norwegian Nynorsk (Latin script) & 18.70 & \textbf{19.92} & 17.78 \\
% Norwegian Bokmal (Latin script) & 20.31 & \textbf{20.62} & 19.91 \\
% Nepali (Devanagari script) & 11.13 & \textbf{14.98} & 11.11 \\
% Punjabi (Gurmukhi script) & 8.53 & \textbf{8.69} & 7.45 \\
% Persian (Arabic script) & 15.35 & \textbf{17.70} & 14.67 \\
% Polish (Latin script) & 19.63 & \textbf{20.28} & 17.51 \\
% Portuguese (Brazil) & \textbf{18.81} & 18.49 & 19.04 \\
% Portuguese (Portugal) & 18.98 & 20.28 & \textbf{20.91} \\
% Romanian (Latin script) & 19.73 & \textbf{20.20} & 18.21 \\
% Russian (Cyrillic script) & 20.71 & 21.98 & \textbf{22.50} \\
% Marwari (Devanagari script) & 9.21 & \textbf{11.17} & 7.15 \\
% Sinhala (Sinhala script) & 5.40 & \textbf{6.58} & 4.47 \\
% Slovak (Latin script) & 15.81 & 17.08 & \textbf{17.14} \\
% Slovak & 11.03 & \textbf{11.82} & 10.12 \\
% Slovenian (Latin script) & 17.23 & \textbf{18.29} & 17.44 \\
% Slovenian & 11.76 & 11.52 & \textbf{9.61} \\
% Sindhi (Arabic script) & 7.17 & \textbf{9.97} & 3.70 \\
% Sindhi (Devanagari script) & 3.91 & \textbf{7.68} & 4.61 \\
% Spanish (Mexico) & 25.11 & \textbf{26.49} & 25.92 \\
% Spanish (Peru) & 23.18 & \textbf{23.79} & 22.98 \\
% Spanish (Spain) & 22.80 & \textbf{23.87} & 23.07 \\
% Serbian (Cyrillic script) & 16.34 & \textbf{17.32} & 13.56 \\
% \midrule
% \multicolumn{4}{r}{\emph{Continued in the next table.}} \\
% \bottomrule
% \end{tabular}
% \caption{chrF scores on Global-PIQA using Mistral across standard, context, and end-to-end. --- continued.}
% \end{table}

% \begin{table}[p]
% \addtocounter{table}{-1}
% \centering
% \scriptsize
% \setlength{\tabcolsep}{4pt}
% \begin{tabular}{p{0.50\textwidth}ccc}
% \toprule
% \textbf{Language} & \textbf{Standard} & \textbf{Context} & \textbf{End-to-end} \\
% \midrule
% Serbian (Latin script) & 17.49 & \textbf{19.01} & 16.05 \\
% Swedish (Latin script) & 21.71 & \textbf{24.33} & 20.82 \\
% Swahili (Latin script) & 10.75 & 13.03 & \textbf{13.24} \\
% Tamil (Tamil script) & 13.48 & 16.94 & \textbf{17.78} \\
% Tagalog (Latin script) & 25.77 & \textbf{27.56} & 26.88 \\
% Thai (Thai script) & 11.83 & \textbf{13.47} & 12.36 \\
% Turkish (Latin script) & 18.94 & \textbf{19.94} & 19.69 \\
% Uyghur (Arabic script) & 8.23 & \textbf{10.40} & 3.55 \\
% Ukrainian (Cyrillic script) & 16.47 & \textbf{17.49} & 14.80 \\
% Urdu (Arabic script) & 13.11 & \textbf{16.07} & 13.27 \\
% Urdu (Latin script) & 13.68 & 11.59 & \textbf{12.02} \\
% Urhobo (Latin script) & 6.32 & \textbf{15.49} & 10.76 \\
% Uzbek (Latin script) & 13.48 & 13.46 & \textbf{16.10} \\
% Cantonese (Traditional) & 1.79 & \textbf{3.45} & 1.66 \\
% Malay (Latin script) & 17.49 & 20.77 & \textbf{25.73} \\
% Azerbaijani (Latin script) & 14.75 & \textbf{15.97} & 11.99 \\
% Gujarati (Gujarati script) & 6.41 & \textbf{9.64} & 8.53 \\
% Macedonian (Cyrillic script) & 17.52 & 17.41 & \textbf{15.18} \\
% Zulu (Latin script) & 9.93 & \textbf{13.90} & 11.52 \\
% Amharic (Ethiopic script) & 1.66 & \textbf{2.58} & 1.29 \\
% Assamese (Bengali script) & 8.10 & \textbf{8.86} & 2.63 \\
% Nigerian Pidgin (Latin script) & 19.35 & \textbf{20.81} & 20.24 \\
% Yoruba (Latin script) & 4.81 & \textbf{8.38} & 7.31 \\
% Mandarin Chinese (Simplified) & 2.70 & 6.12 & \textbf{7.19} \\
% Arabic (Arabic script) & 12.31 & \textbf{12.29} & 7.82 \\
% Japanese (Japanese script) & 4.11 & \textbf{6.27} & 2.70 \\
% Vietnamese (Latin script) & 12.82 & 14.38 & \textbf{17.69} \\
% Telugu (Telugu script) & 7.86 & 10.11 & \textbf{11.38} \\
% Marathi (Devanagari script) & 8.45 & \textbf{12.54} & 6.67 \\
% \bottomrule
% \end{tabular}
% \caption{chrF scores on Global-PIQA using Mistral across standard, context, and end-to-end. --- continued.}
% \end{table}





\clearpage
\begin{table}[p]
\centering
\scriptsize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{p{0.50\textwidth}ccc}
\toprule
\textbf{Language} & \textbf{Standard} & \textbf{Context} & \textbf{End-to-end} \\
\midrule
Mesopotamian Arabic (Arabic script) & 15.69 & \textbf{15.84} & 10.91 \\
Taizzi-Adeni Arabic (Arabic script) & \textbf{18.84} & 17.22 & 15.95 \\
Tunisian Arabic (Arabic script) & \textbf{18.26} & 17.11 & 12.83 \\
Gulf Arabic (Arabic script) & \textbf{12.77} & 12.58 & 10.18 \\
Tosk Albanian (Latin script) & 20.56 & \textbf{26.07} & 15.19 \\
Levantine Arabic (Jordan) & 20.27 & \textbf{20.76} & 16.86 \\
Levantine Arabic (Lebanon) & 24.17 & \textbf{25.12} & 14.69 \\
Levantine Arabic (Palestine) & 18.86 & \textbf{19.06} & 12.01 \\
Levantine Arabic (Syria) & \textbf{16.95} & 15.39 & 14.39 \\
Algerian Arabic (Arabic script) & \textbf{16.75} & 15.79 & 12.29 \\
Najdi Arabic (Arabic script) & 17.76 & \textbf{18.51} & 17.48 \\
Moroccan Arabic (Arabic script) & \textbf{15.90} & 12.98 & 13.82 \\
Egyptian Arabic (Arabic script) & \textbf{19.24} & 17.65 & 14.91 \\
Bambara (Latin script) & 1.51 & \textbf{3.28} & 0.99 \\
Belarusian (Cyrillic script) & 26.30 & \textbf{29.84} & 26.72 \\
Bengali (Bengali script) & 16.58 & 16.04 & \textbf{22.00} \\
Bengali (Latin script) & \textbf{20.04} & 6.33 & 5.38 \\
Bhojpuri (Devanagari script) & 15.80 & 15.30 & \textbf{16.43} \\
Bosnian (Latin script) & \textbf{28.53} & 27.25 & 22.79 \\
Burushaski (Arabic script) & 5.14 & 0.45 & \textbf{6.32} \\
Bulgarian (Cyrillic script) & 28.90 & \textbf{29.34} & 25.07 \\
Catalan (Latin script) & 22.91 & \textbf{24.42} & 20.33 \\
Czech (Latin script) & 14.78 & \textbf{18.62} & 16.74 \\
Central Kurdish (Arabic script) & 5.65 & \textbf{6.08} & 1.29 \\
Chakma (Latin script) & 1.06 & \textbf{6.55} & 0.36 \\
Mandarin Chinese (Traditional) & 7.19 & \textbf{9.66} & 7.63 \\
German (Latin script) & 22.15 & \textbf{22.31} & 16.85 \\
Dhundari (Devanagari script) & 13.84 & 13.97 & \textbf{14.16} \\
Estonian (Latin script) & 16.86 & \textbf{17.31} & 13.89 \\
\midrule
\multicolumn{4}{r}{\emph{Continued in the next table.}} \\
\bottomrule
\end{tabular}
\caption{chrF scores on Global-PIQA using GPT across standard, context, and end-to-end.}
\label{tab:global-piqa-gpt-chrf}
\end{table}

\begin{table}[p]
\addtocounter{table}{-1}
\centering
\scriptsize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{p{0.50\textwidth}ccc}
\toprule
\textbf{Language} & \textbf{Standard} & \textbf{Context} & \textbf{End-to-end} \\
\midrule
Ekpeye (Latin script) & 8.90 & \textbf{11.24} & 4.11 \\
Greek (Greek script) & 13.61 & \textbf{13.63} & 11.40 \\
English (Latin script) & 26.30 & \textbf{28.25} & 17.80 \\
Faroese (Latin script) & 18.14 & \textbf{20.21} & 14.43 \\
Finnish (Latin script) & 29.12 & \textbf{30.72} & 22.74 \\
French (Canada) & 27.93 & \textbf{28.94} & 25.40 \\
French (France) & 27.93 & \textbf{29.15} & 26.18 \\
Galician (Latin script) & 21.39 & \textbf{22.02} & 21.32 \\
Hausa (Latin script) & 25.92 & \textbf{26.77} & 22.70 \\
Hawaiian (Latin script) & 22.72 & \textbf{25.05} & 4.51 \\
Hebrew (Hebrew script) & 19.21 & \textbf{19.87} & 17.87 \\
Hindi (Devanagari script) & 20.39 & 20.10 & \textbf{21.63} \\
Croatian (Latin script) & 18.92 & \textbf{19.31} & 18.46 \\
Hungarian (Latin script) & 26.89 & \textbf{27.92} & 21.57 \\
Armenian (Armenian script) & 22.01 & \textbf{23.08} & 18.88 \\
Igbo (Latin script) & 18.63 & \textbf{20.42} & 17.75 \\
Idoma (Latin script) & \textbf{6.15} & 4.20 & 3.07 \\
Indonesian (Latin script) & 27.19 & 27.17 & \textbf{28.52} \\
Icelandic (Latin script) & 25.16 & \textbf{25.66} & 20.32 \\
Isoko (Latin script) & 2.68 & 2.68 & \textbf{7.50} \\
Italian (Latin script) & 24.09 & \textbf{24.61} & 18.07 \\
Javanese (Latin script) & 20.33 & \textbf{21.00} & 20.33 \\
Kannada (Kannada script) & 22.63 & 22.49 & \textbf{23.91} \\
Georgian (Georgian script) & 19.44 & \textbf{20.17} & 3.44 \\
Kazakh (Cyrillic script) & 24.95 & \textbf{25.92} & 22.12 \\
Kinyarwanda (Latin script) & 23.58 & \textbf{24.40} & 22.15 \\
Kyrgyz (Cyrillic script) & \textbf{26.51} & 25.23 & 21.45 \\
Korean (Hangul script) & 5.98 & \textbf{7.29} & 5.89 \\
Lingala (Latin script) & \textbf{19.89} & 18.35 & 3.70 \\
\midrule
\multicolumn{4}{r}{\emph{Continued in the next table.}} \\
\bottomrule
\end{tabular}
\caption{chrF scores on Global-PIQA using GPT across standard, context, and end-to-end. --- continued.}
\end{table}

\clearpage

\begin{table}[p]
\addtocounter{table}{-1}
\centering
\scriptsize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{p{0.50\textwidth}ccc}
\toprule
\textbf{Language} & \textbf{Standard} & \textbf{Context} & \textbf{End-to-end} \\
\midrule
Lithuanian (Latin script) & \textbf{22.28} & 22.05 & 16.63 \\
Luo (Latin script) & \textbf{2.84} & 2.00 & 0.55 \\
Malayalam (Malayalam script) & 18.74 & 19.86 & \textbf{20.03} \\
Meitei (Bengali script) & \textbf{8.73} & 2.59 & 2.56 \\
Meitei (Meitei Mayek script) & 0.33 & \textbf{0.92} & 0.77 \\
Naga Pidgin (Latin script) & 16.65 & \textbf{19.55} & 13.32 \\
Dutch (Latin script) & 27.97 & \textbf{29.16} & 21.43 \\
Norwegian Nynorsk (Latin script) & 24.67 & \textbf{25.62} & 18.68 \\
Norwegian Bokmal (Latin script) & 23.80 & \textbf{25.79} & 19.77 \\
Nepali (Devanagari script) & 22.91 & \textbf{24.01} & 23.39 \\
Punjabi (Gurmukhi script) & 19.05 & 18.60 & \textbf{19.36} \\
Persian (Arabic script) & 21.11 & \textbf{20.63} & 17.92 \\
Polish (Latin script) & 24.93 & 24.55 & 21.64 \\
Portuguese (Brazil) & 21.02 & 20.21 & 20.39 \\
Portuguese (Portugal) & 23.27 & \textbf{25.30} & 14.36 \\
Romanian (Latin script) & 21.76 & \textbf{23.40} & 16.66 \\
Russian (Cyrillic script) & 22.28 & \textbf{23.51} & 18.26 \\
Marwari (Devanagari script) & 14.37 & \textbf{16.79} & 12.58 \\
Sinhala (Sinhala script) & 12.40 & \textbf{13.00} & 12.81 \\
Slovak (Latin script) & 20.11 & \textbf{22.08} & 16.38 \\
Slovak & 13.74 & 14.30 & \textbf{15.07} \\
Slovenian (Latin script) & 20.00 & \textbf{20.09} & 16.61 \\
Slovenian & 12.32 & \textbf{12.49} & 8.84 \\
Sindhi (Arabic script) & 22.08 & \textbf{23.27} & 20.00 \\
Sindhi (Devanagari script) & \textbf{9.11} & 7.43 & 0.60 \\
Spanish (Mexico) & 25.95 & \textbf{26.67} & 21.19 \\
Spanish (Peru) & 23.61 & \textbf{24.13} & 19.91 \\
Spanish (Spain) & 26.32 & \textbf{27.14} & 21.80 \\
Serbian (Cyrillic script) & 17.50 & \textbf{17.51} & 14.88 \\
\midrule
\multicolumn{4}{r}{\emph{Continued in the next table.}} \\
\bottomrule
\end{tabular}
\caption{chrF scores on Global-PIQA using GPT across standard, context, and end-to-end. --- continued.}
\end{table}

\begin{table}[p]
\addtocounter{table}{-1}
\centering
\scriptsize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{p{0.50\textwidth}ccc}
\toprule
\textbf{Language} & \textbf{Standard} & \textbf{Context} & \textbf{End-to-end} \\
\midrule
Serbian (Latin script) & \textbf{17.82} & 17.59 & 14.59 \\
Swedish (Latin script) & 25.94 & \textbf{26.46} & 21.76 \\
Swahili (Latin script) & 25.49 & \textbf{26.52} & 17.18 \\
Tamil (Tamil script) & 24.44 & \textbf{27.50} & 19.57 \\
Tagalog (Latin script) & \textbf{31.27} & 30.14 & 24.72 \\
Thai (Thai script) & 14.98 & \textbf{17.68} & 13.53 \\
Turkish (Latin script) & 22.76 & \textbf{25.05} & 19.35 \\
Uyghur (Arabic script) & 12.22 & \textbf{13.31} & 5.25 \\
Ukrainian (Cyrillic script) & 18.67 & \textbf{19.04} & 17.16 \\
Urdu (Arabic script) & 20.04 & 17.95 & \textbf{21.63} \\
Urdu (Latin script) & 18.20 & \textbf{18.62} & 11.67 \\
Urhobo (Latin script) & 2.60 & 2.44 & \textbf{2.84} \\
Uzbek (Latin script) & 17.73 & 18.41 & \textbf{20.07} \\
Cantonese (Traditional) & 4.06 & \textbf{4.58} & 3.68 \\
Malay (Latin script) & 29.57 & \textbf{30.51} & 26.22 \\
Azerbaijani (Latin script) & 20.19 & 18.75 & \textbf{23.33} \\
Gujarati (Gujarati script) & 4.63 & 19.71 & \textbf{21.03} \\
Macedonian (Cyrillic script) & 17.35 & \textbf{17.99} & 15.92 \\
Zulu (Latin script) & 20.67 & \textbf{21.07} & 15.62 \\
Amharic (Ethiopic script) & 2.30 & \textbf{3.33} & 0.74 \\
Assamese (Bengali script) & 12.51 & 11.17 & \textbf{16.08} \\
Nigerian Pidgin (Latin script) & 23.70 & \textbf{26.44} & 21.46 \\
Yoruba (Latin script) & 9.63 & \textbf{20.01} & 11.26 \\
Mandarin Chinese (Simplified) & 6.12 & \textbf{6.95} & 4.84 \\
Arabic (Arabic script) & 17.25 & \textbf{18.16} & 17.12 \\
Japanese (Japanese script) & 9.18 & 6.66 & \textbf{7.53} \\
Vietnamese (Latin script) & 15.00 & \textbf{15.75} & 13.42 \\
Telugu (Telugu script) & 19.28 & 20.15 & \textbf{21.15} \\
Marathi (Devanagari script) & 21.65 & 21.47 & \textbf{26.99} \\
\bottomrule
\end{tabular}
\caption{chrF scores on Global-PIQA using GPT across standard, context, and end-to-end. --- continued.}
\end{table}









% \clearpage




% \begin{table}[p]
% \centering
% \scriptsize
% \setlength{\tabcolsep}{4pt}
% \begin{tabular}{p{0.50\textwidth}ccc}
% \toprule
% \textbf{Language} & \textbf{Standard} & \textbf{Context} & \textbf{End-to-end} \\
% \midrule
% Mesopotamian Arabic (Arabic script) & 9.92 & \textbf{10.71} & 8.87 \\
% Taizzi-Adeni Arabic (Arabic script) & 10.25 & \textbf{12.54} & 8.82 \\
% Tunisian Arabic (Arabic script) & \textbf{11.46} & 10.20 & 9.70 \\
% Gulf Arabic (Arabic script) & \textbf{11.01} & 10.23 & 8.45 \\
% Tosk Albanian (Latin script) & 12.42 & \textbf{13.89} & 12.18 \\
% Levantine Arabic (Jordan) & 13.65 & \textbf{15.15} & 9.96 \\
% Levantine Arabic (Lebanon) & 7.90 & \textbf{10.36} & 6.79 \\
% Levantine Arabic (Palestine) & 7.28 & \textbf{9.64} & 6.80 \\
% Levantine Arabic (Syria) & 7.37 & \textbf{9.16} & 6.80 \\
% Algerian Arabic (Arabic script) & \textbf{10.56} & 9.92 & 9.06 \\
% Najdi Arabic (Arabic script) & 11.39 & \textbf{14.47} & 9.78 \\
% Moroccan Arabic (Arabic script) & 10.54 & \textbf{10.61} & 9.08 \\
% Egyptian Arabic (Arabic script) & 12.81 & \textbf{13.27} & 8.65 \\
% Bambara (Latin script) & 5.32 & 10.29 & \textbf{13.25} \\
% Belarusian (Cyrillic script) & 13.93 & \textbf{19.60} & 16.24 \\
% Bengali (Bengali script) & 11.25 & \textbf{13.61} & 12.81 \\
% Bengali (Latin script) & 0.15 & 10.11 & \textbf{11.23} \\
% Bhojpuri (Devanagari script) & 11.72 & \textbf{12.82} & 11.57 \\
% Bosnian (Latin script) & 18.65 & \textbf{18.97} & 17.24 \\
% Burushaski (Arabic script) & 2.66 & 4.32 & \textbf{5.23} \\
% Bulgarian (Cyrillic script) & 16.58 & \textbf{19.13} & 13.83 \\
% Catalan (Latin script) & 15.24 & \textbf{16.44} & 16.01 \\
% Czech (Latin script) & 11.08 & \textbf{13.65} & 8.77 \\
% Central Kurdish (Arabic script) & 10.00 & \textbf{16.01} & 9.50 \\
% Chakma (Latin script) & 1.19 & 1.51 & \textbf{2.98} \\
% Mandarin Chinese (Traditional) & 3.84 & \textbf{8.71} & 4.98 \\
% German (Latin script) & 15.54 & \textbf{16.55} & 16.25 \\
% Dhundari (Devanagari script) & 10.69 & 11.36 & \textbf{11.51} \\
% Estonian (Latin script) & 14.39 & \textbf{18.64} & 11.24 \\
% Ekpeye (Latin script) & 3.89 & 6.54 & \textbf{11.05} \\
% \midrule
% \multicolumn{4}{r}{\emph{Continued in the next table.}} \\
% \bottomrule
% \end{tabular}
% \caption{chrF scores on Global-PIQA using Llama across standard, context, and end-to-end.}
% \label{tab:global-piqa-llama-chrf}
% \end{table}




% \begin{table}[p]
% \addtocounter{table}{-1}
% \centering
% \scriptsize
% \setlength{\tabcolsep}{4pt}
% \begin{tabular}{p{0.50\textwidth}ccc}
% \toprule
% \textbf{Language} & \textbf{Standard} & \textbf{Context} & \textbf{End-to-end} \\
% \midrule
% Greek (Greek script) & 9.82 & \textbf{13.67} & 7.81 \\
% English (Latin script) & \textbf{19.23} & 17.74 & 15.56 \\
% Faroese (Latin script) & 14.30 & \textbf{17.53} & 11.77 \\
% Finnish (Latin script) & 19.08 & \textbf{22.63} & 17.45 \\
% French (Canada) & 18.74 & \textbf{21.85} & 16.82 \\
% French (France) & 13.97 & 14.24 & \textbf{17.78} \\
% Galician (Latin script) & 15.41 & \textbf{20.54} & 16.85 \\
% Hausa (Latin script) & 11.76 & \textbf{13.13} & 8.45 \\
% Hawaiian (Latin script) & 12.81 & \textbf{15.85} & 11.55 \\
% Hebrew (Hebrew script) & 12.72 & \textbf{15.07} & 8.70 \\
% Hindi (Devanagari script) & 13.25 & \textbf{14.20} & 13.78 \\
% Croatian (Latin script) & 13.69 & \textbf{14.34} & 13.96 \\
% Hungarian (Latin script) & 16.63 & \textbf{17.92} & 14.42 \\
% Armenian (Armenian script) & 13.15 & \textbf{14.86} & 9.77 \\
% Igbo (Latin script) & 9.20 & \textbf{15.25} & 15.23 \\
% Idoma (Latin script) & 3.89 & 7.71 & \textbf{10.80} \\
% Indonesian (Latin script) & \textbf{21.30} & 18.78 & 17.89 \\
% Icelandic (Latin script) & 16.29 & \textbf{16.83} & 14.66 \\
% Isoko (Latin script) & 4.08 & 6.66 & \textbf{12.30} \\
% Italian (Latin script) & 12.81 & 21.37 & \textbf{24.10} \\
% Javanese (Latin script) & 12.83 & \textbf{14.10} & 11.08 \\
% Kannada (Kannada script) & 16.99 & \textbf{20.65} & 19.60 \\
% Georgian (Georgian script) & 13.82 & \textbf{16.76} & 13.33 \\
% Kazakh (Cyrillic script) & 14.95 & \textbf{20.10} & 18.14 \\
% Kinyarwanda (Latin script) & 8.80 & \textbf{12.86} & 11.21 \\
% Kyrgyz (Cyrillic script) & 14.99 & 16.85 & \textbf{17.10} \\
% Korean (Hangul script) & 4.04 & \textbf{4.89} & 4.30 \\
% Lingala (Latin script) & 8.32 & 10.08 & \textbf{10.56} \\
% Lithuanian (Latin script) & 12.55 & \textbf{14.12} & 10.95 \\
% Luo (Latin script) & 10.06 & 8.79 & \textbf{10.10} \\
% \midrule
% \multicolumn{4}{r}{\emph{Continued in the next table.}} \\
% \bottomrule
% \end{tabular}
% \caption{chrF scores on Global-PIQA using Llama across standard, context, and end-to-end. --- continued.}
% \end{table}

% \clearpage
% \begin{table}[p]
% \addtocounter{table}{-1}
% \centering
% \scriptsize
% \setlength{\tabcolsep}{4pt}
% \begin{tabular}{p{0.50\textwidth}ccc}
% \toprule
% \textbf{Language} & \textbf{Standard} & \textbf{Context} & \textbf{End-to-end} \\
% \midrule
% Malayalam (Malayalam script) & 15.69 & 19.07 & \textbf{19.12} \\
% Meitei (Bengali script) & 9.19 & 10.91 & \textbf{11.90} \\
% Meitei (Meitei Mayek script) & 0.06 & \textbf{14.47} & 13.26 \\
% Naga Pidgin (Latin script) & 7.55 & \textbf{11.15} & 9.09 \\
% Dutch (Latin script) & \textbf{21.72} & 17.94 & 18.39 \\
% Norwegian Nynorsk (Latin script) & 16.63 & \textbf{17.48} & 15.79 \\
% Norwegian Bokmal (Latin script) & 17.86 & 17.34 & \textbf{17.96} \\
% Nepali (Devanagari script) & 14.29 & \textbf{15.68} & 13.12 \\
% Punjabi (Gurmukhi script) & 12.34 & \textbf{15.27} & 14.37 \\
% Persian (Arabic script) & 14.63 & \textbf{18.55} & 12.95 \\
% Polish (Latin script) & 16.41 & \textbf{17.24} & 14.34 \\
% Portuguese (Brazil) & 16.65 & 18.74 & \textbf{22.17} \\
% Portuguese (Portugal) & 15.67 & \textbf{15.82} & 14.31 \\
% Romanian (Latin script) & 16.10 & \textbf{16.51} & 13.90 \\
% Russian (Cyrillic script) & 15.59 & \textbf{16.62} & 14.60 \\
% Marwari (Devanagari script) & 9.68 & \textbf{11.20} & 10.13 \\
% Sinhala (Sinhala script) & 8.53 & \textbf{9.76} & 9.36 \\
% Slovak (Latin script) & 13.62 & \textbf{17.80} & 16.23 \\
% Slovak & 10.97 & \textbf{12.06} & 8.36 \\
% Slovenian (Latin script) & 14.04 & \textbf{14.70} & 12.22 \\
% Slovenian & 9.77 & \textbf{9.96} & 7.95 \\
% Sindhi (Arabic script) & 11.69 & \textbf{13.76} & 12.26 \\
% Sindhi (Devanagari script) & 2.20 & \textbf{10.11} & 9.03 \\
% Spanish (Mexico) & 16.55 & 17.06 & \textbf{19.11} \\
% Spanish (Peru) & \textbf{18.86} & 17.86 & 18.13 \\
% Spanish (Spain) & 18.43 & \textbf{19.28} & 17.09 \\
% Serbian (Cyrillic script) & 5.93 & \textbf{10.92} & 9.76 \\
% Serbian (Latin script) & 13.30 & \textbf{13.77} & 10.81 \\
% Swedish (Latin script) & 19.74 & \textbf{20.51} & 15.88 \\
% Swahili (Latin script) & \textbf{14.80} & 12.76 & 13.55 \\
% \midrule
% \multicolumn{4}{r}{\emph{Continued in the next table.}} \\
% \bottomrule
% \end{tabular}
% \caption{chrF scores on Global-PIQA using Llama across standard, context, and end-to-end. --- continued.}
% \end{table}


% \begin{table}[p]
% \addtocounter{table}{-1}
% \centering
% \scriptsize
% \setlength{\tabcolsep}{4pt}
% \begin{tabular}{p{0.50\textwidth}ccc}
% \toprule
% \textbf{Language} & \textbf{Standard} & \textbf{Context} & \textbf{End-to-end} \\
% \midrule
% Tamil (Tamil script) & 21.73 & \textbf{25.13} & 21.00 \\
% Tagalog (Latin script) & 21.37 & \textbf{24.72} & 19.60 \\
% Thai (Thai script) & 12.84 & \textbf{15.19} & 8.68 \\
% Turkish (Latin script) & 17.12 & \textbf{19.41} & 16.27 \\
% Uyghur (Arabic script) & 6.64 & \textbf{11.13} & 10.83 \\
% Ukrainian (Cyrillic script) & 14.13 & \textbf{14.46} & 9.81 \\
% Urdu (Arabic script) & 12.89 & \textbf{15.78} & 12.65 \\
% Urdu (Latin script) & 5.32 & \textbf{13.47} & 10.48 \\
% Urhobo (Latin script) & 5.18 & 10.42 & \textbf{13.18} \\
% Uzbek (Latin script) & 11.83 & \textbf{16.24} & 15.19 \\
% Cantonese (Traditional) & 2.56 & \textbf{3.94} & 3.53 \\
% Malay (Latin script) & 23.64 & \textbf{28.85} & 16.03 \\
% Azerbaijani (Latin script) & \textbf{14.08} & 13.72 & 13.25 \\
% Gujarati (Gujarati script) & 13.36 & \textbf{15.95} & 15.61 \\
% Macedonian (Cyrillic script) & \textbf{15.27} & 14.91 & 13.04 \\
% Zulu (Latin script) & 8.79 & 10.01 & \textbf{12.27} \\
% Amharic (Ethiopic script) & 4.04 & \textbf{7.72} & 6.45 \\
% Assamese (Bengali script) & 9.74 & \textbf{12.59} & 12.21 \\
% Nigerian Pidgin (Latin script) & 16.14 & \textbf{21.15} & 13.67 \\
% Yoruba (Latin script) & 4.15 & 7.94 & \textbf{9.25} \\
% Mandarin Chinese (Simplified) & 3.49 & \textbf{6.46} & 4.48 \\
% Arabic (Arabic script) & \textbf{12.88} & 12.10 & 9.04 \\
% Japanese (Japanese script) & 5.55 & \textbf{5.62} & 4.99 \\
% Vietnamese (Latin script) & 10.64 & \textbf{14.42} & 11.57 \\
% Telugu (Telugu script) & 17.07 & \textbf{20.48} & 18.59 \\
% Marathi (Devanagari script) & 10.20 & \textbf{15.49} & 14.47 \\
% \bottomrule
% \end{tabular}
% \caption{chrF scores on Global-PIQA using Llama across standard, context, and end-to-end. --- continued.}
% \end{table}



% \clearpage

% \begin{table}[p]
% \centering
% \scriptsize
% \setlength{\tabcolsep}{4pt}
% \begin{tabular}{p{0.50\textwidth}ccc}
% \toprule
% \textbf{Language} & \textbf{Standard} & \textbf{Context} & \textbf{End-to-end} \\
% \midrule
% Mesopotamian Arabic (Arabic script) & 11.68 & \textbf{12.48} & 11.12 \\
% Taizzi-Adeni Arabic (Arabic script) & \textbf{13.49} & 13.19 & 12.70 \\
% Tunisian Arabic (Arabic script) & 11.47 & \textbf{13.31} & 12.33 \\
% Gulf Arabic (Arabic script) & 10.86 & \textbf{11.64} & 10.19 \\
% Tosk Albanian (Latin script) & 10.53 & \textbf{13.45} & 10.47 \\
% Levantine Arabic (Jordan) & 13.60 & \textbf{16.92} & 14.32 \\
% Levantine Arabic (Lebanon) & 12.84 & 14.46 & \textbf{15.08} \\
% Levantine Arabic (Palestine) & 10.97 & 11.63 & \textbf{12.33} \\
% Levantine Arabic (Syria) & 10.99 & 11.40 & \textbf{12.04} \\
% Algerian Arabic (Arabic script) & 11.34 & \textbf{13.39} & 10.13 \\
% Najdi Arabic (Arabic script) & 13.96 & \textbf{15.32} & 13.53 \\
% Moroccan Arabic (Arabic script) & 10.85 & \textbf{12.57} & 11.71 \\
% Egyptian Arabic (Arabic script) & 12.23 & 13.07 & \textbf{14.23} \\
% Bambara (Latin script) & 7.15 & 10.06 & \textbf{10.48} \\
% Belarusian (Cyrillic script) & 14.25 & \textbf{19.73} & 14.87 \\
% Bengali (Bengali script) & 10.95 & \textbf{12.85} & 10.94 \\
% Bengali (Latin script) & \textbf{3.59} & 0.58 & 1.43 \\
% Bhojpuri (Devanagari script) & 10.72 & \textbf{12.29} & 10.85 \\
% Bosnian (Latin script) & 20.45 & \textbf{21.10} & 17.62 \\
% Burushaski (Arabic script) & 3.62 & \textbf{5.35} & 4.31 \\
% Bulgarian (Cyrillic script) & 21.56 & \textbf{25.06} & 17.95 \\
% Catalan (Latin script) & 18.32 & 18.83 & \textbf{19.02} \\
% Czech (Latin script) & 12.02 & \textbf{14.98} & 12.74 \\
% Central Kurdish (Arabic script) & 11.19 & 14.25 & \textbf{14.36} \\
% Chakma (Latin script) & 3.30 & 4.90 & \textbf{5.50} \\
% Mandarin Chinese (Traditional) & 5.81 & 8.57 & \textbf{10.36} \\
% German (Latin script) & 17.32 & \textbf{19.32} & 17.90 \\
% Dhundari (Devanagari script) & 9.59 & 10.91 & \textbf{11.46} \\
% Estonian (Latin script) & 11.40 & \textbf{15.16} & 11.82 \\
% Ekpeye (Latin script) & 3.80 & 8.26 & \textbf{11.47} \\
% \midrule
% \multicolumn{4}{r}{\emph{Continued in the next table.}} \\
% \bottomrule
% \end{tabular}
% \caption{chrF scores on Global-PIQA using Qwen across standard, context, and end-to-end.}
% \label{tab:global-piqa-qwen-chrf}
% \end{table}




% \begin{table}[p]
% \addtocounter{table}{-1}
% \centering
% \scriptsize
% \setlength{\tabcolsep}{4pt}
% \begin{tabular}{p{0.50\textwidth}ccc}
% \toprule
% \textbf{Language} & \textbf{Standard} & \textbf{Context} & \textbf{End-to-end} \\
% \midrule
% Greek (Greek script) & 10.77 & 11.54 & \textbf{12.04} \\
% English (Latin script) & 23.24 & \textbf{26.18} & 23.52 \\
% Faroese (Latin script) & 12.79 & \textbf{15.76} & 11.96 \\
% Finnish (Latin script) & 19.90 & \textbf{21.54} & 18.72 \\
% French (Canada) & 25.77 & \textbf{28.10} & 25.67 \\
% French (France) & 21.63 & \textbf{23.01} & 21.56 \\
% Galician (Latin script) & \textbf{18.20} & 17.43 & 17.95 \\
% Hausa (Latin script) & 9.10 & \textbf{11.88} & 8.32 \\
% Hawaiian (Latin script) & 7.13 & \textbf{17.51} & 11.86 \\
% Hebrew (Hebrew script) & 10.79 & \textbf{14.28} & 13.25 \\
% Hindi (Devanagari script) & 12.95 & \textbf{15.21} & 13.72 \\
% Croatian (Latin script) & 16.77 & \textbf{17.30} & 13.53 \\
% Hungarian (Latin script) & 11.69 & \textbf{17.97} & 12.97 \\
% Armenian (Armenian script) & 14.15 & 16.35 & \textbf{17.53} \\
% Igbo (Latin script) & 6.66 & 13.58 & \textbf{18.09} \\
% Idoma (Latin script) & 2.99 & 9.91 & \textbf{10.34} \\
% Indonesian (Latin script) & 22.94 & \textbf{25.66} & 22.10 \\
% Icelandic (Latin script) & 14.57 & \textbf{18.60} & 14.74 \\
% Isoko (Latin script) & 2.25 & 7.89 & \textbf{13.19} \\
% Italian (Latin script) & 16.95 & \textbf{23.19} & 19.18 \\
% Javanese (Latin script) & 12.32 & \textbf{13.69} & 10.91 \\
% Kannada (Kannada script) & 11.40 & 18.79 & \textbf{20.11} \\
% Georgian (Georgian script) & 13.33 & 14.68 & \textbf{15.30} \\
% Kazakh (Cyrillic script) & 17.47 & 20.09 & \textbf{21.92} \\
% Kinyarwanda (Latin script) & 10.41 & \textbf{13.29} & 8.79 \\
% Kyrgyz (Cyrillic script) & 15.21 & 16.44 & \textbf{16.94} \\
% Korean (Hangul script) & 3.49 & 4.00 & \textbf{5.54} \\
% Lingala (Latin script) & 9.21 & \textbf{10.20} & 8.95 \\
% Lithuanian (Latin script) & \textbf{12.59} & 12.00 & 9.53 \\
% Luo (Latin script) & 4.46 & \textbf{9.83} & 7.01 \\
% \midrule
% \multicolumn{4}{r}{\emph{Continued in the next table.}} \\
% \bottomrule
% \end{tabular}
% \caption{chrF scores on Global-PIQA using Qwen across standard, context, and end-to-end --- continued.}
% \end{table}

% \clearpage

% \begin{table}[p]
% \addtocounter{table}{-1}
% \centering
% \scriptsize
% \setlength{\tabcolsep}{4pt}
% \begin{tabular}{p{0.50\textwidth}ccc}
% \toprule
% \textbf{Language} & \textbf{Standard} & \textbf{Context} & \textbf{End-to-end} \\
% \midrule
% Malayalam (Malayalam script) & 15.32 & 18.55 & \textbf{21.52} \\
% Meitei (Bengali script) & 7.14 & 7.22 & \textbf{12.09} \\
% Meitei (Meitei Mayek script) & 0.21 & 7.20 & \textbf{13.02} \\
% Naga Pidgin (Latin script) & 3.64 & \textbf{13.37} & 8.94 \\
% Dutch (Latin script) & 20.47 & \textbf{23.47} & 21.33 \\
% Norwegian Nynorsk (Latin script) & 10.85 & \textbf{17.76} & 15.69 \\
% Norwegian Bokmal (Latin script) & 17.96 & \textbf{19.79} & 18.33 \\
% Nepali (Devanagari script) & 15.66 & \textbf{16.34} & 16.02 \\
% Punjabi (Gurmukhi script) & 11.04 & 13.81 & \textbf{14.02} \\
% Persian (Arabic script) & 14.28 & 16.86 & \textbf{18.68} \\
% Polish (Latin script) & 16.98 & \textbf{19.53} & 15.96 \\
% Portuguese (Brazil) & 23.07 & 20.26 & \textbf{20.02} \\
% Portuguese (Portugal) & 18.76 & \textbf{20.16} & 16.08 \\
% Romanian (Latin script) & 17.62 & \textbf{18.58} & 16.13 \\
% Russian (Cyrillic script) & 18.65 & 19.69 & \textbf{20.53} \\
% Marwari (Devanagari script) & 11.39 & \textbf{12.78} & 11.42 \\
% Sinhala (Sinhala script) & 9.22 & \textbf{11.49} & 11.19 \\
% Slovak (Latin script) & 14.95 & 16.72 & \textbf{17.61} \\
% Slovak & 11.26 & \textbf{12.72} & 10.10 \\
% Slovenian (Latin script) & 15.57 & \textbf{17.12} & 14.13 \\
% Slovenian & \textbf{12.22} & 11.17 & 8.92 \\
% Sindhi (Arabic script) & 7.37 & \textbf{10.65} & 9.01 \\
% Sindhi (Devanagari script) & 0.16 & 2.72 & \textbf{10.61} \\
% Spanish (Mexico) & 23.07 & 24.29 & \textbf{25.26} \\
% Spanish (Peru) & 23.02 & \textbf{23.87} & 21.57 \\
% Spanish (Spain) & 23.18 & \textbf{24.56} & 22.27 \\
% Serbian (Cyrillic script) & 14.09 & \textbf{16.42} & 14.58 \\
% Serbian (Latin script) & 18.02 & \textbf{19.05} & 11.31 \\
% Swedish (Latin script) & 18.36 & \textbf{21.56} & 19.16 \\
% Swahili (Latin script) & 12.88 & \textbf{15.33} & 10.57 \\
% \midrule
% \multicolumn{4}{r}{\emph{Continued in the next table.}} \\
% \bottomrule
% \end{tabular}
% \caption{chrF scores on Global-PIQA using Qwen across standard, context, and end-to-end --- continued.}
% \end{table}



% \begin{table}[p]
% \addtocounter{table}{-1}
% \centering
% \scriptsize
% \setlength{\tabcolsep}{4pt}
% \begin{tabular}{p{0.50\textwidth}ccc}
% \toprule
% \textbf{Language} & \textbf{Standard} & \textbf{Context} & \textbf{End-to-end} \\
% \midrule
% Tamil (Tamil script) & 19.69 & 22.34 & \textbf{28.75} \\
% Tagalog (Latin script) & 23.85 & \textbf{27.51} & 24.10 \\
% Thai (Thai script) & 15.54 & \textbf{16.01} & 14.95 \\
% Turkish (Latin script) & 13.42 & 17.83 & \textbf{19.50} \\
% Uyghur (Arabic script) & 9.76 & \textbf{12.87} & 9.97 \\
% Ukrainian (Cyrillic script) & 14.97 & \textbf{15.56} & 13.86 \\
% Urdu (Arabic script) & 13.69 & \textbf{15.35} & 12.42 \\
% Urdu (Latin script) & \textbf{3.44} & 1.23 & 1.14 \\
% Urhobo (Latin script) & 6.78 & 15.13 & \textbf{15.39} \\
% Uzbek (Latin script) & 10.84 & \textbf{16.03} & 14.87 \\
% Cantonese (Traditional) & 2.75 & 3.73 & \textbf{4.68} \\
% Malay (Latin script) & 20.22 & 22.09 & \textbf{24.79} \\
% Azerbaijani (Latin script) & 13.96 & \textbf{16.16} & 13.29 \\
% Gujarati (Gujarati script) & 9.86 & 13.72 & \textbf{14.14} \\
% Macedonian (Cyrillic script) & 16.57 & \textbf{18.19} & 14.10 \\
% Zulu (Latin script) & 11.95 & \textbf{15.20} & 14.24 \\
% Amharic (Ethiopic script) & 2.49 & \textbf{6.51} & 4.67 \\
% Assamese (Bengali script) & 10.39 & \textbf{11.60} & 10.97 \\
% Nigerian Pidgin (Latin script) & 11.50 & \textbf{17.01} & 12.43 \\
% Yoruba (Latin script) & 5.01 & 10.35 & \textbf{12.70} \\
% Mandarin Chinese (Simplified) & 4.93 & \textbf{8.03} & 7.19 \\
% Arabic (Arabic script) & 12.43 & \textbf{13.18} & 12.82 \\
% Japanese (Japanese script) & 4.87 & 5.56 & \textbf{6.94} \\
% Vietnamese (Latin script) & 6.93 & \textbf{15.01} & 14.64 \\
% Telugu (Telugu script) & 14.56 & 17.28 & \textbf{21.35} \\
% Marathi (Devanagari script) & 12.48 & \textbf{16.91} & 15.55 \\
% \bottomrule
% \end{tabular}
% \caption{chrF scores on Global-PIQA using Qwen across standard, context, and end-to-end --- continued.}
% \end{table}








% \begin{table}[p]
% \centering
% \scriptsize
% \setlength{\tabcolsep}{4pt}
% \begin{tabular}{p{0.50\textwidth}ccc}
% \toprule
% \textbf{Language} & \textbf{Standard} & \textbf{Context} & \textbf{End-to-end} \\
% \midrule
% Mesopotamian Arabic (Arabic script) & 9.92 & \textbf{10.71} & 8.87 \\
% Taizzi-Adeni Arabic (Arabic script) & 10.25 & \textbf{12.54} & 8.82 \\
% Tunisian Arabic (Arabic script) & \textbf{11.46} & 10.20 & 9.70 \\
% Gulf Arabic (Arabic script) & \textbf{11.01} & 10.23 & 8.45 \\
% Tosk Albanian (Latin script) & 12.15 & \textbf{13.55} & 11.78 \\
% Levantine Arabic (Jordan) & 13.65 & \textbf{15.15} & 9.96 \\
% Levantine Arabic (Lebanon) & 7.90 & \textbf{10.36} & 6.79 \\
% Levantine Arabic (Palestine) & 7.28 & \textbf{9.64} & 6.80 \\
% Levantine Arabic (Syria) & 7.37 & \textbf{9.16} & 6.80 \\
% Algerian Arabic (Arabic script) & \textbf{10.56} & 9.92 & 9.06 \\
% Najdi Arabic (Arabic script) & 11.39 & \textbf{14.47} & 9.78 \\
% Moroccan Arabic (Arabic script) & 10.54 & \textbf{10.61} & 9.08 \\
% Egyptian Arabic (Arabic script) & 12.81 & \textbf{13.27} & 8.65 \\
% Bambara (Latin script) & 5.08 & 9.98 & \textbf{12.86} \\
% Belarusian (Cyrillic script) & 13.49 & \textbf{18.91} & 15.40 \\
% Bengali (Bengali script) & 11.08 & \textbf{13.46} & 12.57 \\
% Bengali (Latin script) & 0.14 & 9.60 & \textbf{10.73} \\
% Bhojpuri (Devanagari script) & 11.71 & \textbf{12.82} & 11.57 \\
% Bosnian (Latin script) & 18.27 & \textbf{18.61} & 16.90 \\
% Burushaski (Arabic script) & 2.66 & 4.32 & \textbf{5.23} \\
% Bulgarian (Cyrillic script) & 16.23 & \textbf{18.65} & 13.36 \\
% Catalan (Latin script) & 14.90 & \textbf{16.06} & 15.60 \\
% Czech (Latin script) & 10.79 & \textbf{13.28} & 8.47 \\
% Central Kurdish (Arabic script) & 10.00 & \textbf{16.01} & 9.50 \\
% Chakma (Latin script) & 1.17 & 1.45 & \textbf{2.86} \\
% Mandarin Chinese (Traditional) & 3.84 & \textbf{8.72} & 4.98 \\
% German (Latin script) & 14.54 & \textbf{15.54} & 15.29 \\
% Dhundari (Devanagari script) & 10.61 & 11.24 & \textbf{11.37} \\
% Estonian (Latin script) & 14.09 & \textbf{18.25} & 10.92 \\
% Ekpeye (Latin script) & 3.70 & 6.23 & \textbf{10.61} \\
% \midrule
% \multicolumn{4}{r}{\emph{Continued in the next table.}} \\
% \bottomrule
% \end{tabular}
% \caption{chrF scores on Global-PIQA using Llama across standard, context, and end-to-end.}
% \label{tab:global-piqa-llama-chrf}
% \end{table}


% \begin{table}[p]
% \addtocounter{table}{-1}
% \centering
% \scriptsize
% \setlength{\tabcolsep}{4pt}
% \begin{tabular}{p{0.50\textwidth}ccc}
% \toprule
% \textbf{Language} & \textbf{Standard} & \textbf{Context} & \textbf{End-to-end} \\
% \midrule
% Greek (Greek script) & 9.53 & \textbf{13.36} & 7.51 \\
% English (Latin script) & \textbf{18.85} & 17.43 & 15.29 \\
% Faroese (Latin script) & 14.04 & \textbf{17.21} & 11.45 \\
% Finnish (Latin script) & 18.69 & \textbf{22.27} & 17.07 \\
% French (Canada) & 18.49 & \textbf{21.65} & 16.58 \\
% French (France) & 13.57 & 13.97 & \textbf{17.37} \\
% Galician (Latin script) & 15.14 & \textbf{20.26} & 16.54 \\
% Hausa (Latin script) & 11.50 & \textbf{12.71} & 7.99 \\
% Hawaiian (Latin script) & 12.44 & \textbf{15.45} & 11.08 \\
% Hebrew (Hebrew script) & 12.72 & \textbf{15.07} & 8.70 \\
% Hindi (Devanagari script) & 13.23 & \textbf{14.13} & 13.73 \\
% Croatian (Latin script) & 13.44 & \textbf{14.07} & 13.34 \\
% Hungarian (Latin script) & 16.31 & \textbf{17.56} & 14.10 \\
% Armenian (Armenian script) & 12.82 & \textbf{14.40} & 9.41 \\
% Igbo (Latin script) & 8.55 & 15.01 & \textbf{15.23} \\
% Idoma (Latin script) & 3.62 & 7.24 & \textbf{10.30} \\
% Indonesian (Latin script) & \textbf{20.78} & 18.35 & 17.41 \\
% Icelandic (Latin script) & 15.88 & \textbf{16.36} & 14.24 \\
% Isoko (Latin script) & 3.92 & 6.43 & \textbf{11.94} \\
% Italian (Latin script) & 12.49 & 20.97 & \textbf{23.62} \\
% Javanese (Latin script) & 12.54 & \textbf{13.74} & 10.55 \\
% Kannada (Kannada script) & 16.99 & \textbf{20.65} & 19.60 \\
% Georgian (Georgian script) & 13.82 & \textbf{16.76} & 13.33 \\
% Kazakh (Cyrillic script) & 14.68 & \textbf{19.78} & 17.85 \\
% Kinyarwanda (Latin script) & 8.48 & \textbf{12.31} & 10.61 \\
% Kyrgyz (Cyrillic script) & 14.82 & 16.52 & \textbf{16.84} \\
% Korean (Hangul script) & 4.04 & \textbf{4.89} & 4.30 \\
% Lingala (Latin script) & 7.93 & 9.67 & \textbf{10.01} \\
% Lithuanian (Latin script) & 11.95 & \textbf{13.52} & 10.44 \\
% Luo (Latin script) & \textbf{9.64} & 8.29 & 9.55 \\
% \midrule
% \multicolumn{4}{r}{\emph{Continued in the next table.}} \\
% \bottomrule
% \end{tabular}
% \caption{chrF scores on Global-PIQA using Llama across standard, context, and end-to-end --- continued.}
% \end{table}



% \begin{table}[p]
% \addtocounter{table}{-1}
% \centering
% \scriptsize
% \setlength{\tabcolsep}{4pt}
% \begin{tabular}{p{0.50\textwidth}ccc}
% \toprule
% \textbf{Language} & \textbf{Standard} & \textbf{Context} & \textbf{End-to-end} \\
% \midrule
% Malayalam (Malayalam script) & 15.69 & 19.07 & \textbf{19.12} \\
% Meitei (Bengali script) & 8.93 & 10.60 & \textbf{11.65} \\
% Meitei (Meitei Mayek script) & 0.06 & \textbf{14.47} & 13.26 \\
% Naga Pidgin (Latin script) & 7.32 & \textbf{10.93} & 8.81 \\
% Dutch (Latin script) & \textbf{21.34} & 17.65 & 17.99 \\
% Norwegian Nynorsk (Latin script) & 16.20 & \textbf{17.02} & 15.32 \\
% Norwegian Bokmal (Latin script) & 17.35 & 16.86 & \textbf{17.43} \\
% Nepali (Devanagari script) & 14.29 & \textbf{15.68} & 13.12 \\
% Punjabi (Gurmukhi script) & 12.32 & \textbf{15.19} & 14.28 \\
% Persian (Arabic script) & 14.63 & \textbf{18.55} & 12.95 \\
% Polish (Latin script) & 15.96 & \textbf{16.85} & 13.95 \\
% Portuguese (Brazil) & 16.32 & 18.52 & \textbf{21.96} \\
% Portuguese (Portugal) & 14.97 & \textbf{15.35} & 13.83 \\
% Romanian (Latin script) & 15.78 & \textbf{16.29} & 13.49 \\
% Russian (Cyrillic script) & 15.09 & \textbf{16.13} & 14.17 \\
% Marwari (Devanagari script) & 9.68 & \textbf{11.20} & 10.14 \\
% Sinhala (Sinhala script) & 8.53 & \textbf{9.76} & 9.36 \\
% Slovak (Latin script) & 13.39 & \textbf{17.45} & 15.93 \\
% Slovak & 10.73 & \textbf{11.78} & 8.08 \\
% Slovenian (Latin script) & 13.68 & \textbf{14.34} & 11.93 \\
% Slovenian & 9.59 & \textbf{9.69} & 7.46 \\
% Sindhi (Arabic script) & 11.69 & \textbf{13.76} & 12.26 \\
% Sindhi (Devanagari script) & 2.20 & \textbf{10.05} & 8.99 \\
% Spanish (Mexico) & 15.94 & 16.62 & \textbf{18.55} \\
% Spanish (Peru) & \textbf{18.31} & 17.41 & 17.66 \\
% Spanish (Spain) & 18.03 & \textbf{18.85} & 16.69 \\
% Serbian (Cyrillic script) & 5.79 & \textbf{10.68} & 9.46 \\
% Serbian (Latin script) & 13.06 & \textbf{13.58} & 10.48 \\
% Swedish (Latin script) & 19.34 & \textbf{20.11} & 15.52 \\
% Swahili (Latin script) & \textbf{14.43} & 12.40 & 13.01 \\
% \midrule
% \multicolumn{4}{r}{\emph{Continued in the next table.}} \\
% \bottomrule
% \end{tabular}
% \caption{chrF scores on Global-PIQA using Llama across standard, context, and end-to-end --- continued.}
% \end{table}



% \begin{table}[p]
% \addtocounter{table}{-1}
% \centering
% \scriptsize
% \setlength{\tabcolsep}{4pt}
% \begin{tabular}{p{0.50\textwidth}ccc}
% \toprule
% \textbf{Language} & \textbf{Standard} & \textbf{Context} & \textbf{End-to-end} \\
% \midrule
% Tamil (Tamil script) & 21.73 & \textbf{25.13} & 21.00 \\
% Tagalog (Latin script) & 20.81 & \textbf{24.11} & 19.00 \\
% Thai (Thai script) & 12.78 & \textbf{15.09} & 8.61 \\
% Turkish (Latin script) & 16.81 & \textbf{19.02} & 15.87 \\
% Uyghur (Arabic script) & 6.65 & \textbf{11.13} & 10.83 \\
% Ukrainian (Cyrillic script) & 13.91 & \textbf{14.24} & 9.52 \\
% Urdu (Arabic script) & 12.89 & \textbf{15.79} & 12.65 \\
% Urdu (Latin script) & 5.18 & \textbf{13.12} & 10.18 \\
% Urhobo (Latin script) & 4.91 & 9.97 & \textbf{12.79} \\
% Uzbek (Latin script) & 11.57 & \textbf{15.93} & 14.87 \\
% Cantonese (Traditional) & 2.55 & \textbf{3.94} & 3.53 \\
% Malay (Latin script) & 23.13 & \textbf{28.34} & 15.62 \\
% Azerbaijani (Latin script) & \textbf{13.87} & 13.48 & 12.97 \\
% Gujarati (Gujarati script) & 13.36 & \textbf{15.95} & 15.61 \\
% Macedonian (Cyrillic script) & \textbf{14.95} & 14.61 & 12.57 \\
% Zulu (Latin script) & 8.46 & 9.52 & \textbf{11.68} \\
% Amharic (Ethiopic script) & 4.04 & \textbf{7.72} & 6.45 \\
% Assamese (Bengali script) & 9.38 & \textbf{12.30} & 11.90 \\
% Nigerian Pidgin (Latin script) & 15.70 & \textbf{20.67} & 13.05 \\
% Yoruba (Latin script) & 3.67 & 8.64 & \textbf{10.14} \\
% Mandarin Chinese (Simplified) & 3.48 & \textbf{6.46} & 4.48 \\
% Arabic (Arabic script) & \textbf{12.88} & 12.10 & 9.04 \\
% Japanese (Japanese script) & 5.55 & \textbf{5.62} & 4.99 \\
% Vietnamese (Latin script) & 10.30 & \textbf{13.97} & 11.19 \\
% Telugu (Telugu script) & 17.07 & \textbf{20.48} & 18.59 \\
% Marathi (Devanagari script) & 10.20 & \textbf{15.49} & 14.47 \\
% \bottomrule
% \end{tabular}
% \caption{chrF scores on Global-PIQA using Llama across standard cascade, context, and end-to-end --- continued.}
% \end{table}



% \begin{table}[p]
% \centering
% \scriptsize
% \setlength{\tabcolsep}{4pt}
% \begin{tabular}{p{0.50\textwidth}ccc}
% \toprule
% \textbf{Language} & \textbf{Standard} & \textbf{Context} & \textbf{End-to-end} \\
% \midrule
% Mesopotamian Arabic (Arabic script) & 11.68 & \textbf{12.48} & 11.12 \\
% Taizzi-Adeni Arabic (Arabic script) & \textbf{13.49} & 13.19 & 12.70 \\
% Tunisian Arabic (Arabic script) & 11.47 & \textbf{13.31} & 12.33 \\
% Gulf Arabic (Arabic script) & 10.86 & \textbf{11.64} & 10.19 \\
% Tosk Albanian (Latin script) & 10.24 & \textbf{13.08} & 10.09 \\
% Levantine Arabic (Jordan) & 13.60 & \textbf{16.92} & 14.32 \\
% Levantine Arabic (Lebanon) & 12.84 & 14.46 & \textbf{15.08} \\
% Levantine Arabic (Palestine) & 10.97 & 11.63 & \textbf{12.33} \\
% Levantine Arabic (Syria) & 10.99 & 11.40 & \textbf{12.04} \\
% Algerian Arabic (Arabic script) & 11.34 & \textbf{13.39} & 10.13 \\
% Najdi Arabic (Arabic script) & 13.96 & \textbf{15.32} & 13.53 \\
% Moroccan Arabic (Arabic script) & 10.85 & \textbf{12.57} & 11.71 \\
% Egyptian Arabic (Arabic script) & 12.23 & 13.07 & \textbf{14.23} \\
% Bambara (Latin script) & 6.97 & 9.75 & \textbf{10.22} \\
% Belarusian (Cyrillic script) & 13.66 & \textbf{19.10} & 14.22 \\
% Bengali (Bengali script) & 10.74 & \textbf{12.46} & 10.58 \\
% Bengali (Latin script) & \textbf{3.43} & 0.54 & 1.42 \\
% Bhojpuri (Devanagari script) & 10.72 & \textbf{12.29} & 10.84 \\
% Bosnian (Latin script) & 19.98 & \textbf{20.77} & 17.30 \\
% Burushaski (Arabic script) & 3.62 & \textbf{5.35} & 4.31 \\
% Bulgarian (Cyrillic script) & 21.29 & \textbf{24.71} & 17.61 \\
% Catalan (Latin script) & 17.97 & 18.45 & \textbf{18.60} \\
% Czech (Latin script) & 11.76 & \textbf{14.62} & 12.46 \\
% Central Kurdish (Arabic script) & 11.19 & 14.25 & \textbf{14.36} \\
% Chakma (Latin script) & 3.24 & 4.71 & \textbf{5.16} \\
% Mandarin Chinese (Traditional) & 5.81 & 8.57 & \textbf{10.36} \\
% German (Latin script) & 16.53 & \textbf{18.35} & 16.87 \\
% Dhundari (Devanagari script) & 9.57 & 10.73 & \textbf{11.20} \\
% Estonian (Latin script) & 11.21 & \textbf{14.86} & 11.57 \\
% Ekpeye (Latin script) & 3.71 & 7.88 & \textbf{11.07} \\
% \midrule
% \multicolumn{4}{r}{\emph{Continued in the next table.}} \\
% \bottomrule
% \end{tabular}
% \caption{chrF scores on Global-PIQA using Qwen across standard, context, and end-to-end.}
% \label{tab:global-piqa-qwen-chrf}
% \end{table}



% \begin{table}[p]
% \addtocounter{table}{-1}
% \centering
% \scriptsize
% \setlength{\tabcolsep}{4pt}
% \begin{tabular}{p{0.50\textwidth}ccc}
% \toprule
% \textbf{Language} & \textbf{Standard} & \textbf{Context} & \textbf{End-to-end} \\
% \midrule
% Greek (Greek script) & 10.54 & 11.30 & \textbf{11.77} \\
% English (Latin script) & 22.77 & \textbf{25.59} & 23.10 \\
% Faroese (Latin script) & 12.59 & \textbf{15.47} & 11.62 \\
% Finnish (Latin script) & 19.64 & \textbf{21.19} & 18.48 \\
% French (Canada) & 25.52 & \textbf{27.88} & 25.46 \\
% French (France) & 21.37 & \textbf{22.72} & 21.14 \\
% Galician (Latin script) & \textbf{17.89} & 17.16 & 17.65 \\
% Hausa (Latin script) & 8.83 & \textbf{11.52} & 8.00 \\
% Hawaiian (Latin script) & 6.91 & \textbf{17.07} & 11.50 \\
% Hebrew (Hebrew script) & 10.78 & \textbf{14.27} & 13.25 \\
% Hindi (Devanagari script) & 12.93 & \textbf{15.13} & 13.65 \\
% Croatian (Latin script) & 16.47 & \textbf{17.00} & 13.16 \\
% Hungarian (Latin script) & 11.51 & \textbf{17.61} & 12.69 \\
% Armenian (Armenian script) & 13.80 & 15.91 & \textbf{17.15} \\
% Igbo (Latin script) & 6.24 & 12.06 & \textbf{16.53} \\
% Idoma (Latin script) & 2.92 & 9.41 & \textbf{9.84} \\
% Indonesian (Latin script) & 22.40 & \textbf{25.08} & 21.70 \\
% Icelandic (Latin script) & 14.29 & \textbf{18.13} & 14.29 \\
% Isoko (Latin script) & 2.23 & 7.62 & \textbf{12.92} \\
% Italian (Latin script) & 16.55 & \textbf{22.73} & 18.82 \\
% Javanese (Latin script) & 12.10 & \textbf{13.34} & 10.56 \\
% Kannada (Kannada script) & 11.40 & 18.79 & \textbf{20.11} \\
% Georgian (Georgian script) & 13.33 & 14.68 & \textbf{15.30} \\
% Kazakh (Cyrillic script) & 17.20 & 19.74 & \textbf{21.57} \\
% Kinyarwanda (Latin script) & 10.03 & \textbf{12.76} & 8.49 \\
% Kyrgyz (Cyrillic script) & 14.98 & 16.15 & \textbf{16.69} \\
% Korean (Hangul script) & 3.49 & 4.00 & \textbf{5.54} \\
% Lingala (Latin script) & 8.79 & \textbf{9.79} & 8.64 \\
% Lithuanian (Latin script) & \textbf{12.10} & 11.44 & 9.17 \\
% Luo (Latin script) & 4.35 & \textbf{9.35} & 6.74 \\
% \midrule
% \multicolumn{4}{r}{\emph{Continued in the next table.}} \\
% \bottomrule
% \end{tabular}
% \caption{chrF scores on Global-PIQA using Qwen across standard, context, and end-to-end --- continued.}
% \end{table}



% \begin{table}[p]
% \addtocounter{table}{-1}
% \centering
% \scriptsize
% \setlength{\tabcolsep}{4pt}
% \begin{tabular}{p{0.50\textwidth}ccc}
% \toprule
% \textbf{Language} & \textbf{Standard} & \textbf{Context} & \textbf{End-to-end} \\
% \midrule
% Malayalam (Malayalam script) & 15.32 & 18.55 & \textbf{21.52} \\
% Meitei (Bengali script) & 7.06 & 7.16 & \textbf{11.74} \\
% Meitei (Meitei Mayek script) & 0.21 & 7.20 & \textbf{13.02} \\
% Naga Pidgin (Latin script) & 3.61 & \textbf{13.03} & 8.69 \\
% Dutch (Latin script) & 20.18 & \textbf{23.12} & 21.01 \\
% Norwegian Nynorsk (Latin script) & 10.65 & \textbf{17.40} & 15.30 \\
% Norwegian Bokmal (Latin script) & 17.47 & \textbf{19.25} & 17.86 \\
% Nepali (Devanagari script) & 15.66 & \textbf{16.34} & 16.02 \\
% Punjabi (Gurmukhi script) & 11.03 & 13.79 & \textbf{14.00} \\
% Persian (Arabic script) & 14.28 & 16.86 & \textbf{18.68} \\
% Polish (Latin script) & 16.49 & \textbf{19.06} & 15.56 \\
% Portuguese (Brazil) & \textbf{23.00} & 20.18 & 19.77 \\
% Portuguese (Portugal) & 18.10 & \textbf{19.47} & 15.50 \\
% Romanian (Latin script) & 17.33 & \textbf{18.25} & 15.82 \\
% Russian (Cyrillic script) & 18.21 & 19.28 & \textbf{19.96} \\
% Marwari (Devanagari script) & 11.39 & \textbf{12.78} & 11.42 \\
% Sinhala (Sinhala script) & 9.22 & \textbf{11.49} & 11.19 \\
% Slovak (Latin script) & 14.71 & 16.43 & \textbf{17.35} \\
% Slovak & 10.94 & \textbf{12.40} & 9.83 \\
% Slovenian (Latin script) & 15.24 & \textbf{16.83} & 13.87 \\
% Slovenian & 11.92 & \textbf{10.93} & 8.66 \\
% Sindhi (Arabic script) & 7.37 & \textbf{10.65} & 9.01 \\
% Sindhi (Devanagari script) & 0.16 & 2.65 & \textbf{10.48} \\
% Spanish (Mexico) & 22.61 & 23.95 & \textbf{24.74} \\
% Spanish (Peru) & 22.51 & \textbf{23.36} & 21.08 \\
% Spanish (Spain) & 22.71 & \textbf{24.10} & 21.78 \\
% Serbian (Cyrillic script) & 13.91 & \textbf{16.18} & 14.34 \\
% Serbian (Latin script) & 17.78 & \textbf{18.81} & 11.08 \\
% Swedish (Latin script) & 18.01 & \textbf{21.20} & 18.75 \\
% Swahili (Latin script) & 12.60 & \textbf{14.97} & 10.34 \\
% \midrule
% \multicolumn{4}{r}{\emph{Continued in the next table.}} \\
% \bottomrule
% \end{tabular}
% \caption{chrF scores on Global-PIQA using Qwen across standard, context, and end-to-end --- continued.}
% \end{table}


% \begin{table}[p]
% \addtocounter{table}{-1}
% \centering
% \scriptsize
% \setlength{\tabcolsep}{4pt}
% \begin{tabular}{p{0.50\textwidth}ccc}
% \toprule
% \textbf{Language} & \textbf{Standard} & \textbf{Context} & \textbf{End-to-end} \\
% \midrule
% Tamil (Tamil script) & 19.69 & 22.34 & \textbf{28.75} \\
% Tagalog (Latin script) & 23.40 & \textbf{26.95} & 23.55 \\
% Thai (Thai script) & 15.40 & \textbf{15.91} & 14.80 \\
% Turkish (Latin script) & 13.19 & 17.44 & \textbf{19.17} \\
% Uyghur (Arabic script) & 9.76 & \textbf{12.87} & 9.96 \\
% Ukrainian (Cyrillic script) & 14.68 & \textbf{15.25} & 13.63 \\
% Urdu (Arabic script) & 13.69 & \textbf{15.35} & 12.42 \\
% Urdu (Latin script) & \textbf{3.37} & 1.19 & 1.12 \\
% Urhobo (Latin script) & 6.56 & 14.77 & \textbf{14.87} \\
% Uzbek (Latin script) & 10.67 & \textbf{15.75} & 14.63 \\
% Cantonese (Traditional) & 2.72 & 3.71 & \textbf{4.68} \\
% Malay (Latin script) & 19.80 & 21.69 & \textbf{24.24} \\
% Azerbaijani (Latin script) & 13.74 & \textbf{15.88} & 13.01 \\
% Gujarati (Gujarati script) & 9.86 & 13.72 & \textbf{14.14} \\
% Macedonian (Cyrillic script) & 16.20 & \textbf{17.89} & 13.73 \\
% Zulu (Latin script) & 11.38 & \textbf{14.58} & 13.58 \\
% Amharic (Ethiopic script) & 2.49 & \textbf{6.51} & 4.67 \\
% Assamese (Bengali script) & 10.00 & \textbf{11.22} & 10.61 \\
% Nigerian Pidgin (Latin script) & 11.26 & \textbf{16.63} & 12.02 \\
% Yoruba (Latin script) & 4.03 & 7.68 & \textbf{9.46} \\
% Mandarin Chinese (Simplified) & 4.92 & \textbf{8.02} & 7.19 \\
% Arabic (Arabic script) & 12.43 & \textbf{13.18} & 12.82 \\
% Japanese (Japanese script) & 4.87 & 5.56 & \textbf{6.94} \\
% Vietnamese (Latin script) & 6.73 & \textbf{14.66} & 14.27 \\
% Telugu (Telugu script) & 14.56 & 17.28 & \textbf{21.35} \\
% Marathi (Devanagari script) & 12.48 & \textbf{16.91} & 15.55 \\
% \bottomrule
% \end{tabular}
% \caption{chrF scores on Global-PIQA using Qwen across standard cascade, context, and end-to-end --- continued.}
% \end{table}

==> latex/tables/gpt/mc_math.tex <==
\begin{table}[htbp]
\centering
\small
\begin{tabular}{lccc}
\toprule
Dataset & \cstd & \etoe & \cctx \\
\midrule
Global MMLU & \textbf{70.40} & 61.90 & 69.84 \\
MCSQA & 68.33 & \textbf{72.08} & 67.92 \\
Belebele & 53.50 & \textbf{71.43} & 58.24 \\
Global-PIQA & \textbf{80.69} & 49.02 & 76.95 \\
MGSM & \textbf{87.27} & 83.94 & 82.12 \\
MMath & \textbf{38.33} & 36.00 & 38.00 \\
\bottomrule
\end{tabular}
\caption{Overall multiple-choice accuracy for GPT-4o-mini.}
\end{table}



\begin{table}[htbp]
\centering
\small
\begin{tabular}{lccc}
\toprule
Dataset & \cstd & \etoe & \cctx \\
\midrule
Aya & 14.65 & \textbf{15.96} & 15.52\\
BLEnD & 17.26 & \textbf{22.10} & 17.26 \\
Global-PIQA-OE & 18.15 & 15.41 & \textbf{18.73} \\
MKQA & 26.25 & 23.03 & \textbf{27.92} \\
\bottomrule
\end{tabular}
\caption{Overall open-ended chrf scores for GPT-4o-mini.}
\end{table}






==> latex/tables/llama/mc_math.tex <==
% \begin{table}[htbp]
% \centering
% \begin{tabular}{lccc}
% \toprule
% Dataset & \cstd & \etoe & \cctx \\
% \midrule
% Global MMLU & 40.76\% & 36.12\% & \textbf{43.12\%} \\
% MCSQA & 64.62\% & \textbf{67.12\%} & 65.12\% \\
% Belebele & 56.89\% & 53.50\% & \textbf{58.18\%} \\
% Global-PIQA & 65.60\% & 61.95\% & \textbf{66.24\%} \\
% MGSM & 38.91\% & \textbf{49.64\%} & 47.09\% \\
% MMath & 13.50\% & 14.10\% & \textbf{16.00\%} \\
% \bottomrule
% \end{tabular}
% \caption{Overall multiple-choice accuracy for Llama-3.1-8B-Instruct.}
% \end{table}

\begin{table}[htbp]
\centering
\begin{tabular}{lccc}
\toprule
Dataset & \cstd & \etoe & \cctx \\
\midrule
Aya & 9.56 & 11.27 & \textbf{14.26}\\
BLEnD & 9.51 & 11.99 & \textbf{12.19} \\
Global-PIQA-OE & 11.99 & 12.46 & \textbf{14.31}\\
MKQA & 13.36 & 11.51 & \textbf{14.62} \\
\bottomrule
\end{tabular}
\caption{Overall open-ended chrf scores for Llama-3.1-8B-Instruct.}
\end{table}




\begin{longtable}{lccc}
\caption{Llama-3.1-8B-Instruct accuracy on Global MMLU: High-resource (22), Mid-resource (11) and Low-resource (9).} \\
\toprule
Language & \cstd & \etoe & \cctx \\
\midrule
\endfirsthead
\multicolumn{4}{c}{\tablename\ \thetable{} -- continued} \\
\toprule
Language & \cstd & \etoe & \cctx \\
\midrule
\endhead
\midrule
\multicolumn{4}{r}{\textit{Continued on next page}} \\
\endfoot
\bottomrule
\endlastfoot
\multicolumn{4}{l}{\textit{High-resource (22)}} \\
\midrule
Arabic & 47.00\% & 41.00\% & \textbf{50.00\%} \\
Chinese & \textbf{54.00\%} & 35.00\% & 54.00\% \\
Czech & 48.00\% & 34.00\% & \textbf{49.00\%} \\
Dutch & 43.00\% & 44.00\% & \textbf{46.00\%} \\
English & 52.00\% & \textbf{62.00\%} & 57.00\% \\
French & 42.00\% & 39.00\% & \textbf{46.00\%} \\
German & 44.00\% & \textbf{48.00\%} & 48.00\% \\
Greek & 35.00\% & 36.00\% & \textbf{43.00\%} \\
Indonesian & 50.00\% & 32.00\% & \textbf{54.00\%} \\
Italian & 45.00\% & 40.00\% & \textbf{48.00\%} \\
Japanese & 42.00\% & 36.00\% & \textbf{46.00\%} \\
Korean & 39.00\% & 34.00\% & \textbf{41.00\%} \\
Persian & 42.00\% & \textbf{43.00\%} & 42.00\% \\
Polish & \textbf{47.00\%} & 38.00\% & 47.00\% \\
Portuguese & 40.00\% & 37.00\% & \textbf{50.00\%} \\
Romanian & 46.00\% & 41.00\% & \textbf{48.00\%} \\
Russian & 47.00\% & 32.00\% & \textbf{51.00\%} \\
Spanish & 43.00\% & 39.00\% & \textbf{45.00\%} \\
Swedish & \textbf{46.00\%} & 42.00\% & 44.00\% \\
Turkish & 43.00\% & 40.00\% & \textbf{45.00\%} \\
Ukrainian & 38.00\% & 36.00\% & \textbf{41.00\%} \\
Vietnamese & 36.00\% & 39.00\% & \textbf{40.00\%} \\
\textbf{Avg} & 44.05\% & 39.45\% & \textbf{47.05\%} \\
\midrule
\multicolumn{4}{l}{\textit{Mid-resource (11)}} \\
\midrule
Bengali & 42.00\% & 33.00\% & \textbf{46.00\%} \\
Hebrew & \textbf{40.00\%} & 35.00\% & 38.00\% \\
Hindi & 36.00\% & 36.00\% & \textbf{40.00\%} \\
Kyrgyz & 35.00\% & 31.00\% & \textbf{37.00\%} \\
Lithuanian & 42.00\% & 33.00\% & \textbf{44.00\%} \\
Malay & 41.00\% & 42.00\% & \textbf{44.00\%} \\
Nepali & 43.00\% & 39.00\% & \textbf{49.00\%} \\
Serbian & 41.00\% & 34.00\% & \textbf{43.00\%} \\
Sinhala & 37.00\% & 34.00\% & \textbf{39.00\%} \\
Swahili & 37.00\% & \textbf{40.00\%} & 38.00\% \\
Telugu & 41.00\% & 25.00\% & \textbf{43.00\%} \\
\textbf{Avg} & 39.55\% & 34.73\% & \textbf{41.91\%} \\
\midrule
\multicolumn{4}{l}{\textit{Low-resource (9)}} \\
\midrule
Amharic & \textbf{37.00\%} & 29.00\% & 36.00\% \\
Chichewa & 28.00\% & 26.00\% & \textbf{30.00\%} \\
Filipino & 49.00\% & 32.00\% & \textbf{52.00\%} \\
Hausa & 30.00\% & \textbf{36.00\%} & 29.00\% \\
Igbo & 31.00\% & 29.00\% & \textbf{32.00\%} \\
Malagasy & \textbf{36.00\%} & 26.00\% & 34.00\% \\
Shona & 30.00\% & 29.00\% & \textbf{33.00\%} \\
Somali & \textbf{34.00\%} & 30.00\% & 31.00\% \\
Yoruba & 33.00\% & 30.00\% & \textbf{38.00\%} \\
\textbf{Avg} & 34.22\% & 29.67\% & \textbf{35.00\%} \\
\midrule
\textbf{Overall (42)} & 40.76\% & 36.12\% & \textbf{43.12\%} \\
\end{longtable}

\begin{longtable}{lccc}
\caption{Llama-3.1-8B-Instruct cccuracy on MCSQA: High-resource (8).} \\
\toprule
Language & \cstd & \etoe & \cctx \\
\midrule
\endfirsthead
\multicolumn{4}{c}{\tablename\ \thetable{} -- continued} \\
\toprule
Language & \cstd & \etoe & \cctx \\
\midrule
\endhead
\midrule
\multicolumn{4}{r}{\textit{Continued on next page}} \\
\endfoot
\bottomrule
\endlastfoot
\multicolumn{4}{l}{\textit{High-resource (8)}} \\
\midrule
Chinese & 60.00\% & \textbf{64.00\%} & 60.00\% \\
Dutch & 73.00\% & \textbf{79.00\%} & 74.00\% \\
English & 67.00\% & \textbf{77.00\%} & 66.00\% \\
French & 72.00\% & 70.00\% & \textbf{74.00\%} \\
German & 65.00\% & \textbf{71.00\%} & 65.00\% \\
Japanese & 72.00\% & \textbf{74.00\%} & 73.00\% \\
Portuguese & \textbf{73.00\%} & 64.00\% & 72.00\% \\
Russian & 35.00\% & \textbf{38.00\%} & 37.00\% \\
\textbf{Avg} & 64.62\% & \textbf{67.12\%} & 65.12\% \\
\midrule
\textbf{Overall (8)} & 64.62\% & \textbf{67.12\%} & 65.12\% \\
\end{longtable}




\begin{longtable}{lccc}
\caption{Llama-3.1-8B-Instruct accuracy on Belebele: High-resource (31), Mid-resource (42) and Low-resource (48).} \\
\toprule
Language & \cstd & \etoe & \cctx \\
\midrule
\endfirsthead
\multicolumn{4}{c}{\tablename\ \thetable{} -- continued} \\
\toprule
Language & \cstd & \etoe & \cctx \\
\midrule
\endhead
\midrule
\multicolumn{4}{r}{\textit{Continued on next page}} \\
\endfoot
\bottomrule
\endlastfoot
\multicolumn{4}{l}{\textit{High-resource (31)}} \\
\midrule
Chinese (Simplified) & 53.33\% & \textbf{80.00\%} & 63.33\% \\
Chinese (Traditional) & 63.33\% & \textbf{86.67\%} & 70.00\% \\
Czech & 76.67\% & \textbf{86.67\%} & 76.67\% \\
Danish & 76.67\% & \textbf{83.33\%} & 76.67\% \\
Dutch & \textbf{90.00\%} & 86.67\% & 90.00\% \\
Egyptian Arabic & \textbf{66.67\%} & 53.33\% & 66.67\% \\
English & 80.00\% & \textbf{90.00\%} & 83.33\% \\
French & 80.00\% & \textbf{83.33\%} & 80.00\% \\
German & 86.67\% & \textbf{90.00\%} & 90.00\% \\
Greek & 83.33\% & 73.33\% & \textbf{86.67\%} \\
Hungarian & 76.67\% & \textbf{80.00\%} & 76.67\% \\
Indonesian & \textbf{80.00\%} & 70.00\% & 80.00\% \\
Italian & 76.67\% & \textbf{80.00\%} & 80.00\% \\
Japanese & \textbf{63.33\%} & 60.00\% & 63.33\% \\
Korean & \textbf{76.67\%} & 70.00\% & 76.67\% \\
Mesopotamian Arabic & \textbf{66.67\%} & 53.33\% & 63.33\% \\
Modern Standard Arabic & 70.00\% & 73.33\% & \textbf{80.00\%} \\
Modern Standard Arabic (Romanized) & 20.00\% & \textbf{23.33\%} & 20.00\% \\
Najdi Arabic & 50.00\% & \textbf{53.33\%} & 53.33\% \\
North Levantine Arabic & \textbf{56.67\%} & 53.33\% & 53.33\% \\
Polish & 86.67\% & 76.67\% & \textbf{90.00\%} \\
Portuguese & 80.00\% & \textbf{93.33\%} & 80.00\% \\
Romanian & 70.00\% & \textbf{73.33\%} & 73.33\% \\
Russian & 66.67\% & \textbf{76.67\%} & 66.67\% \\
Slovak & \textbf{86.67\%} & 63.33\% & 86.67\% \\
Spanish & 93.33\% & \textbf{96.67\%} & 93.33\% \\
Swedish & 76.67\% & 76.67\% & \textbf{80.00\%} \\
Turkish & 66.67\% & \textbf{73.33\%} & 66.67\% \\
Ukrainian & \textbf{73.33\%} & 60.00\% & 73.33\% \\
Vietnamese & 83.33\% & 83.33\% & \textbf{86.67\%} \\
Western Persian & \textbf{76.67\%} & 66.67\% & 76.67\% \\
\textbf{Avg} & 72.69\% & 73.23\% & \textbf{74.30\%} \\
\midrule
\multicolumn{4}{l}{\textit{Mid-resource (42)}} \\
\midrule
Afrikaans & \textbf{86.67\%} & 83.33\% & 86.67\% \\
Armenian & 73.33\% & 63.33\% & \textbf{76.67\%} \\
Basque & \textbf{73.33\%} & 56.67\% & 73.33\% \\
Bengali & \textbf{53.33\%} & 53.33\% & 53.33\% \\
Bengali (Romanized) & \textbf{40.00\%} & 30.00\% & 40.00\% \\
Bulgarian & \textbf{80.00\%} & 76.67\% & 80.00\% \\
Burmese & 33.33\% & \textbf{43.33\%} & 36.67\% \\
Catalan & 76.67\% & \textbf{83.33\%} & 76.67\% \\
Croatian & 83.33\% & 80.00\% & \textbf{86.67\%} \\
Eastern Panjabi & \textbf{40.00\%} & 36.67\% & 40.00\% \\
Finnish & 66.67\% & \textbf{83.33\%} & 70.00\% \\
Georgian & \textbf{66.67\%} & 56.67\% & 66.67\% \\
Gujarati & \textbf{56.67\%} & 53.33\% & 56.67\% \\
Hebrew & \textbf{80.00\%} & 66.67\% & 80.00\% \\
Hindi & \textbf{66.67\%} & 60.00\% & 63.33\% \\
Hindi (Romanized) & 46.67\% & \textbf{53.33\%} & 46.67\% \\
Icelandic & \textbf{80.00\%} & 60.00\% & 80.00\% \\
Kannada & 60.00\% & 56.67\% & \textbf{63.33\%} \\
Kazakh & \textbf{60.00\%} & 60.00\% & 60.00\% \\
Khmer & \textbf{53.33\%} & 20.00\% & 53.33\% \\
Kyrgyz & 66.67\% & 63.33\% & \textbf{73.33\%} \\
Lithuanian & 66.67\% & 56.67\% & \textbf{70.00\%} \\
Macedonian & 60.00\% & \textbf{86.67\%} & 70.00\% \\
Malayalam & 46.67\% & 43.33\% & \textbf{50.00\%} \\
Marathi & 73.33\% & \textbf{86.67\%} & 73.33\% \\
Nepali & 40.00\% & \textbf{56.67\%} & 40.00\% \\
North Azerbaijani & 60.00\% & \textbf{63.33\%} & 60.00\% \\
Northern Uzbek & 70.00\% & 70.00\% & \textbf{73.33\%} \\
Norwegian Bokmål & \textbf{83.33\%} & 83.33\% & 83.33\% \\
Serbian & 76.67\% & 76.67\% & \textbf{80.00\%} \\
Sinhala & 46.67\% & 23.33\% & \textbf{50.00\%} \\
Sinhala (Romanized) & 30.00\% & 26.67\% & \textbf{33.33\%} \\
Slovenian & 70.00\% & 73.33\% & \textbf{76.67\%} \\
Standard Malay & \textbf{90.00\%} & 83.33\% & 90.00\% \\
Swahili & 56.67\% & 50.00\% & \textbf{66.67\%} \\
Tagalog & 53.33\% & \textbf{56.67\%} & 56.67\% \\
Tamil & 50.00\% & \textbf{60.00\%} & 50.00\% \\
Telugu & 40.00\% & \textbf{46.67\%} & 40.00\% \\
Thai & 60.00\% & \textbf{73.33\%} & 66.67\% \\
Tosk Albanian & 86.67\% & 80.00\% & \textbf{90.00\%} \\
Urdu & \textbf{90.00\%} & 70.00\% & 90.00\% \\
Urdu (Romanized) & \textbf{33.33\%} & 16.67\% & 33.33\% \\
\textbf{Avg} & 62.54\% & 60.08\% & \textbf{64.44\%} \\
\midrule
\multicolumn{4}{l}{\textit{Low-resource (48)}} \\
\midrule
Amharic & \textbf{33.33\%} & 20.00\% & 33.33\% \\
Assamese & 50.00\% & \textbf{56.67\%} & 53.33\% \\
Bambara & \textbf{26.67\%} & 20.00\% & 23.33\% \\
Cebuano & \textbf{60.00\%} & 50.00\% & 56.67\% \\
Central Kurdish & \textbf{73.33\%} & 60.00\% & 70.00\% \\
Estonian & 70.00\% & 66.67\% & \textbf{76.67\%} \\
Ganda & \textbf{33.33\%} & 26.67\% & 26.67\% \\
Guarani & 30.00\% & \textbf{36.67\%} & 30.00\% \\
Haitian Creole & \textbf{63.33\%} & 33.33\% & 63.33\% \\
Halh Mongolian & 46.67\% & 33.33\% & \textbf{50.00\%} \\
Hausa & 43.33\% & 30.00\% & \textbf{50.00\%} \\
Igbo & 40.00\% & 16.67\% & \textbf{43.33\%} \\
Ilocano & \textbf{46.67\%} & 43.33\% & 46.67\% \\
Javanese & \textbf{66.67\%} & 56.67\% & 66.67\% \\
Jingpho & 20.00\% & 16.67\% & \textbf{23.33\%} \\
Kabuverdianu & \textbf{63.33\%} & 46.67\% & 63.33\% \\
Kinyarwanda & 23.33\% & \textbf{30.00\%} & 23.33\% \\
Lao & 30.00\% & 26.67\% & \textbf{36.67\%} \\
Lingala & \textbf{23.33\%} & 23.33\% & 23.33\% \\
Luo & \textbf{23.33\%} & 23.33\% & 23.33\% \\
Maltese & 66.67\% & 56.67\% & \textbf{70.00\%} \\
Maori & \textbf{60.00\%} & 33.33\% & 60.00\% \\
Nepali (Romanized) & 46.67\% & 46.67\% & \textbf{50.00\%} \\
Nigerian Fulfulde & 36.67\% & 23.33\% & \textbf{40.00\%} \\
Northern Sotho & \textbf{30.00\%} & 30.00\% & 30.00\% \\
Nyanja & 33.33\% & \textbf{46.67\%} & 33.33\% \\
Odia & 53.33\% & 33.33\% & \textbf{56.67\%} \\
Plateau Malagasy & 26.67\% & \textbf{36.67\%} & 26.67\% \\
Shan & 26.67\% & \textbf{30.00\%} & 23.33\% \\
Shona & \textbf{36.67\%} & 26.67\% & 36.67\% \\
Sindhi & 53.33\% & 46.67\% & \textbf{56.67\%} \\
Somali & 16.67\% & \textbf{23.33\%} & 16.67\% \\
Southern Pashto & 56.67\% & 43.33\% & \textbf{60.00\%} \\
Southern Sotho & 26.67\% & \textbf{33.33\%} & 30.00\% \\
Standard Latvian & 60.00\% & \textbf{73.33\%} & 56.67\% \\
Standard Tibetan & \textbf{36.67\%} & 13.33\% & 33.33\% \\
Sundanese & \textbf{53.33\%} & 43.33\% & 53.33\% \\
Swati & \textbf{46.67\%} & 33.33\% & 46.67\% \\
Tajik & 66.67\% & 50.00\% & \textbf{70.00\%} \\
Tigrinya & 23.33\% & 23.33\% & \textbf{26.67\%} \\
Tsonga & 30.00\% & \textbf{40.00\%} & 33.33\% \\
Tswana & \textbf{30.00\%} & 26.67\% & 26.67\% \\
Waray & \textbf{56.67\%} & 26.67\% & 56.67\% \\
West Central Oromo & \textbf{43.33\%} & 23.33\% & 43.33\% \\
Wolof & \textbf{36.67\%} & 13.33\% & 33.33\% \\
Xhosa & \textbf{23.33\%} & 16.67\% & 23.33\% \\
Yoruba & 26.67\% & \textbf{36.67\%} & 20.00\% \\
Zulu & \textbf{33.33\%} & 33.33\% & 33.33\% \\
\textbf{Avg} & 41.74\% & 35.00\% & \textbf{42.29\%} \\
\midrule
\textbf{Overall (121)} & 56.89\% & 53.50\% & \textbf{58.18\%} \\
\end{longtable}

\begin{longtable}{lccc}
\caption{Llama-3.1-8B-Instruct accuracy on Global PIQA: High-resource (44), Mid-resource (42) and Low-resource (30).} \\
\toprule
Language & \cstd & \etoe & \cctx \\
\midrule
\endfirsthead
\multicolumn{4}{c}{\tablename\ \thetable{} -- continued} \\
\toprule
Language & \cstd & \etoe & \cctx \\
\midrule
\endhead
\midrule
\multicolumn{4}{r}{\textit{Continued on next page}} \\
\endfoot
\bottomrule
\endlastfoot
\multicolumn{4}{l}{\textit{High-resource (44)}} \\
\midrule
Algerian Arabic & 50.00\% & \textbf{60.00\%} & 46.67\% \\
Burushaski & 40.00\% & \textbf{43.33\%} & 40.00\% \\
Cantonese & \textbf{70.00\%} & 60.00\% & 70.00\% \\
Chinese (Simplified) & 56.67\% & 56.67\% & \textbf{60.00\%} \\
Chinese (Traditional) & \textbf{56.67\%} & 50.00\% & 53.33\% \\
Czech & \textbf{73.33\%} & 63.33\% & 73.33\% \\
Dutch & \textbf{70.00\%} & 66.67\% & 70.00\% \\
Egyptian Arabic & \textbf{60.00\%} & 36.67\% & 56.67\% \\
English & \textbf{73.33\%} & 73.33\% & 73.33\% \\
French (Canada) & 86.67\% & 80.00\% & \textbf{90.00\%} \\
French (France) & \textbf{73.33\%} & 66.67\% & 73.33\% \\
German & 66.67\% & 66.67\% & \textbf{73.33\%} \\
Greek & 60.00\% & 56.67\% & \textbf{63.33\%} \\
Gulf Arabic & 40.00\% & \textbf{66.67\%} & 36.67\% \\
Hungarian & \textbf{83.33\%} & 83.33\% & 83.33\% \\
Indonesian & 83.33\% & \textbf{86.67\%} & 86.67\% \\
Italian & \textbf{76.67\%} & 60.00\% & 76.67\% \\
Japanese & 70.00\% & 53.33\% & \textbf{73.33\%} \\
Korean & 53.33\% & \textbf{60.00\%} & 53.33\% \\
Mesopotamian Arabic & \textbf{63.33\%} & 63.33\% & 60.00\% \\
Modern Standard Arabic & \textbf{63.33\%} & 60.00\% & 63.33\% \\
Moroccan Arabic & 50.00\% & \textbf{53.33\%} & 50.00\% \\
Najdi Arabic & 76.67\% & 63.33\% & \textbf{80.00\%} \\
North Levantine Arabic (Jordan) & \textbf{60.00\%} & 46.67\% & 60.00\% \\
North Levantine Arabic (Lebanon) & \textbf{73.33\%} & 70.00\% & 73.33\% \\
North Levantine Arabic (Palestine) & \textbf{56.67\%} & 56.67\% & 56.67\% \\
North Levantine Arabic (Syria) & \textbf{70.00\%} & 60.00\% & 70.00\% \\
Polish & 50.00\% & \textbf{60.00\%} & 53.33\% \\
Portuguese (Brazil) & 66.67\% & \textbf{80.00\%} & 66.67\% \\
Portuguese (Portugal) & \textbf{93.33\%} & 86.67\% & 93.33\% \\
Romanian & 90.00\% & 86.67\% & \textbf{93.33\%} \\
Russian & 80.00\% & 56.67\% & \textbf{83.33\%} \\
Slovak & 60.00\% & \textbf{70.00\%} & 56.67\% \\
Slovak (SARI) & 53.33\% & \textbf{60.00\%} & 53.33\% \\
Spanish (Mexico) & \textbf{76.67\%} & 76.67\% & 76.67\% \\
Spanish (Peru) & \textbf{90.00\%} & 83.33\% & 90.00\% \\
Spanish (Spain) & 66.67\% & \textbf{90.00\%} & 63.33\% \\
Swedish & 66.67\% & \textbf{80.00\%} & 70.00\% \\
Ta'izzi-Adeni Arabic & 60.00\% & \textbf{66.67\%} & 63.33\% \\
Tunisian Arabic & \textbf{63.33\%} & 63.33\% & 63.33\% \\
Turkish & 76.67\% & \textbf{80.00\%} & 76.67\% \\
Ukrainian & \textbf{80.00\%} & 76.67\% & 80.00\% \\
Vietnamese & \textbf{60.00\%} & 53.33\% & 60.00\% \\
Western Persian & 70.00\% & 36.67\% & \textbf{76.67\%} \\
\textbf{Avg} & 67.27\% & 65.23\% & \textbf{67.88\%} \\
\midrule
\multicolumn{4}{l}{\textit{Mid-resource (42)}} \\
\midrule
Armenian & 60.00\% & \textbf{70.00\%} & 63.33\% \\
Belarusian & \textbf{80.00\%} & 63.33\% & 80.00\% \\
Bengali & 80.00\% & 80.00\% & \textbf{83.33\%} \\
Bengali (Romanized) & 33.33\% & \textbf{43.33\%} & 33.33\% \\
Bosnian & 86.67\% & \textbf{90.00\%} & 86.67\% \\
Bulgarian & \textbf{86.67\%} & 73.33\% & 86.67\% \\
Catalan & \textbf{76.67\%} & 66.67\% & 76.67\% \\
Croatian & \textbf{83.33\%} & 70.00\% & 83.33\% \\
Eastern Panjabi & \textbf{63.33\%} & 63.33\% & 63.33\% \\
Finnish & \textbf{63.33\%} & 56.67\% & 63.33\% \\
Galician & 66.67\% & 60.00\% & \textbf{70.00\%} \\
Georgian & 56.67\% & \textbf{63.33\%} & 56.67\% \\
Gujarati & \textbf{90.00\%} & 76.67\% & 90.00\% \\
Hebrew & 60.00\% & 60.00\% & \textbf{63.33\%} \\
Hindi & \textbf{80.00\%} & 76.67\% & 80.00\% \\
Icelandic & \textbf{86.67\%} & 76.67\% & 86.67\% \\
Kannada & 76.67\% & 70.00\% & \textbf{83.33\%} \\
Kazakh & 50.00\% & \textbf{60.00\%} & 50.00\% \\
Kyrgyz & 60.00\% & \textbf{63.33\%} & 60.00\% \\
Lithuanian & 66.67\% & \textbf{76.67\%} & 63.33\% \\
Macedonian & 76.67\% & 66.67\% & \textbf{80.00\%} \\
Malayalam & \textbf{60.00\%} & 43.33\% & 60.00\% \\
Marathi & \textbf{90.00\%} & 60.00\% & 90.00\% \\
Nepali & \textbf{70.00\%} & 70.00\% & 70.00\% \\
North Azerbaijani & \textbf{76.67\%} & 50.00\% & 76.67\% \\
Northern Uzbek & 56.67\% & \textbf{60.00\%} & 53.33\% \\
Norwegian Bokmål & \textbf{80.00\%} & 60.00\% & 80.00\% \\
Norwegian Nynorsk & 83.33\% & 63.33\% & \textbf{86.67\%} \\
Serbian (Cyrillic) & \textbf{56.67\%} & 53.33\% & 53.33\% \\
Serbian (Latin) & \textbf{70.00\%} & 60.00\% & 70.00\% \\
Sinhala & 46.67\% & \textbf{56.67\%} & 53.33\% \\
Slovenian & \textbf{73.33\%} & 40.00\% & 73.33\% \\
Slovenian (CERK) & 43.33\% & 46.67\% & \textbf{53.33\%} \\
Standard Malay & \textbf{86.67\%} & 86.67\% & 86.67\% \\
Swahili & \textbf{76.67\%} & 66.67\% & 76.67\% \\
Tagalog & \textbf{76.67\%} & 60.00\% & 76.67\% \\
Tamil & 60.00\% & \textbf{70.00\%} & 60.00\% \\
Telugu & \textbf{90.00\%} & 66.67\% & 90.00\% \\
Thai & \textbf{83.33\%} & 76.67\% & 83.33\% \\
Tosk Albanian & \textbf{63.33\%} & 46.67\% & 63.33\% \\
Urdu & \textbf{86.67\%} & 73.33\% & 86.67\% \\
Urdu (Romanized) & 56.67\% & \textbf{70.00\%} & 56.67\% \\
\textbf{Avg} & 70.72\% & 64.44\% & \textbf{71.51\%} \\
\midrule
\multicolumn{4}{l}{\textit{Low-resource (30)}} \\
\midrule
Amharic & \textbf{60.00\%} & 50.00\% & 56.67\% \\
Assamese & \textbf{83.33\%} & 73.33\% & 83.33\% \\
Bambara & 43.33\% & \textbf{53.33\%} & 43.33\% \\
Bhojpuri & 56.67\% & \textbf{70.00\%} & 63.33\% \\
Central Kurdish & \textbf{56.67\%} & 53.33\% & 56.67\% \\
Dhundari & \textbf{80.00\%} & 46.67\% & 80.00\% \\
Ekpeye & \textbf{56.67\%} & 43.33\% & 56.67\% \\
Estonian & \textbf{53.33\%} & 53.33\% & 50.00\% \\
Faroese & 46.67\% & 46.67\% & \textbf{53.33\%} \\
Hausa & \textbf{46.67\%} & 43.33\% & 46.67\% \\
Hawaiian & 43.33\% & \textbf{56.67\%} & 43.33\% \\
Idoma & \textbf{40.00\%} & 40.00\% & 40.00\% \\
Igbo & \textbf{50.00\%} & 30.00\% & 50.00\% \\
Isoko & 50.00\% & \textbf{70.00\%} & 53.33\% \\
Javanese & 53.33\% & \textbf{56.67\%} & 50.00\% \\
Kinyarwanda & 63.33\% & 46.67\% & \textbf{66.67\%} \\
Kumzari & \textbf{53.33\%} & 36.67\% & 53.33\% \\
Lingala & 43.33\% & \textbf{53.33\%} & 43.33\% \\
Luo & \textbf{43.33\%} & 40.00\% & 43.33\% \\
Marwari & \textbf{73.33\%} & 66.67\% & 73.33\% \\
Meitei (Bengali script) & 66.67\% & 40.00\% & \textbf{70.00\%} \\
Meitei (Meitei script) & 43.33\% & \textbf{50.00\%} & 46.67\% \\
Nagamese & 43.33\% & \textbf{46.67\%} & 40.00\% \\
Nigerian Pidgin & \textbf{80.00\%} & 80.00\% & 80.00\% \\
Sindhi & \textbf{100.00\%} & 96.67\% & 100.00\% \\
Sindhi (Devanagari) & 63.33\% & 56.67\% & \textbf{66.67\%} \\
Urhobo & 46.67\% & \textbf{53.33\%} & 43.33\% \\
Uyghur & \textbf{46.67\%} & 46.67\% & 43.33\% \\
Yoruba & 43.33\% & \textbf{50.00\%} & 43.33\% \\
Zulu & 50.00\% & \textbf{60.00\%} & 53.33\% \\
\textbf{Avg} & 56.00\% & 53.67\% & \textbf{56.44\%} \\
\midrule
\textbf{Overall (116)} & 65.60\% & 61.95\% & \textbf{66.24\%} \\
\end{longtable}

\begin{longtable}{lccc}
\caption{Llama-3.1-8B-Instruct accuracy on MGSM: High-resource (7) and Mid-resource (4).} \\
\toprule
Language & \cstd & \etoe & \cctx \\
\midrule
\endfirsthead
\multicolumn{4}{c}{\tablename\ \thetable{} -- continued} \\
\toprule
Language & \cstd & \etoe & \cctx \\
\midrule
\endhead
\midrule
\multicolumn{4}{r}{\textit{Continued on next page}} \\
\endfoot
\bottomrule
\endlastfoot
\multicolumn{4}{l}{\textit{High-resource (7)}} \\
\midrule
Chinese & 37.00\% & \textbf{54.00\%} & 49.00\% \\
English & 36.00\% & \textbf{65.00\%} & 56.00\% \\
French & 43.00\% & 48.00\% & \textbf{54.00\%} \\
German & 44.00\% & \textbf{56.00\%} & 55.00\% \\
Japanese & 36.00\% & \textbf{46.00\%} & 43.00\% \\
Russian & 51.00\% & 56.00\% & \textbf{63.00\%} \\
Spanish & 48.00\% & \textbf{55.00\%} & 49.00\% \\
\textbf{Avg} & 42.14\% & \textbf{54.29\%} & 52.71\% \\
\midrule
\multicolumn{4}{l}{\textit{Mid-resource (4)}} \\
\midrule
Bengali & 27.00\% & \textbf{38.00\%} & 23.00\% \\
Swahili & 50.00\% & 42.00\% & \textbf{54.00\%} \\
Telugu & 26.00\% & 35.00\% & \textbf{36.00\%} \\
Thai & 30.00\% & \textbf{51.00\%} & 36.00\% \\
\textbf{Avg} & 33.25\% & \textbf{41.50\%} & 37.25\% \\
\midrule
\textbf{Overall (11)} & 38.91\% & \textbf{49.64\%} & 47.09\% \\
\end{longtable}

\begin{longtable}{lccc}
\caption{Llama-3.1-8B-Instruct accuracy on MMath: High-resource (9) and Mid-resource (1).} \\
\toprule
Language & \cstd & \etoe & \cctx \\
\midrule
\endfirsthead
\multicolumn{4}{c}{\tablename\ \thetable{} -- continued} \\
\toprule
Language & \cstd & \etoe & \cctx \\
\midrule
\endhead
\midrule
\multicolumn{4}{r}{\textit{Continued on next page}} \\
\endfoot
\bottomrule
\endlastfoot
\multicolumn{4}{l}{\textit{High-resource (9)}} \\
\midrule
Arabic & 18.00\% & 8.00\% & \textbf{21.00\%} \\
Chinese & 11.00\% & \textbf{14.00\%} & 13.00\% \\
English & 15.00\% & \textbf{20.00\%} & 18.00\% \\
French & 15.00\% & 15.00\% & \textbf{16.00\%} \\
Japanese & 12.00\% & \textbf{15.00\%} & 15.00\% \\
Korean & 9.00\% & \textbf{15.00\%} & 11.00\% \\
Portuguese & 14.00\% & 15.00\% & \textbf{20.00\%} \\
Spanish & 16.00\% & 17.00\% & \textbf{18.00\%} \\
Vietnamese & 14.00\% & 10.00\% & \textbf{17.00\%} \\
\textbf{Avg} & 13.78\% & 14.33\% & \textbf{16.56\%} \\
\midrule
\multicolumn{4}{l}{\textit{Mid-resource (1)}} \\
\midrule
Thai & 11.00\% & \textbf{12.00\%} & 11.00\% \\
\textbf{Avg} & 11.00\% & \textbf{12.00\%} & 11.00\% \\
\midrule
\textbf{Overall (10)} & 13.50\% & 14.10\% & \textbf{16.00\%} \\
\end{longtable}



\begin{longtable}{lccc}
\caption{Llama-3.1-8B-Instruct chrF on Aya: High-resource (4), Mid-resource (1) and Low-resource (1).} \\
\toprule
Language & \cstd & \etoe & \cctx \\
\midrule
\endfirsthead
\multicolumn{4}{c}{\tablename\ \thetable{} -- continued} \\
\toprule
Language & \cstd & \etoe & \cctx \\
\midrule
\endhead
\midrule
\multicolumn{4}{r}{\textit{Continued on next page}} \\
\endfoot
\bottomrule
\endlastfoot

\multicolumn{4}{l}{\textit{High-resource (4)}} \\
\midrule
Arabic & 8.67 & 9.43 & \textbf{13.63} \\
Chinese & 5.02 & 6.46 & \textbf{10.49} \\
Portuguese & 19.72 & 22.54 & \textbf{27.29} \\
Turkish & 14.33 & 15.64 & \textbf{20.94} \\
\textbf{Avg} & 11.94 & 13.52 & \textbf{18.09} \\
\midrule

\multicolumn{4}{l}{\textit{Mid-resource (1)}} \\
\midrule
Telugu & 7.93 & 11.01 & \textbf{11.09} \\
\textbf{Avg} & 7.93 & 11.01 & \textbf{11.09} \\
\midrule

\multicolumn{4}{l}{\textit{Low-resource (1)}} \\
\midrule
Yoruba & 1.66 & \textbf{2.55} & 2.11 \\
\textbf{Avg} & 1.66 & \textbf{2.55} & 2.11 \\
\midrule

\textbf{Overall (6)} & 9.56 & 11.27 & \textbf{14.26} \\
\end{longtable}


\begin{longtable}{lccc}
\caption{Llama-3.1-8B-Instruct chrF on BLEnD: High-resource (9), Mid-resource (1) and Low-resource (4).} \\
\toprule
Language & \cstd & \etoe & \cctx \\
\midrule
\endfirsthead
\multicolumn{4}{c}{\tablename\ \thetable{} -- continued} \\
\toprule
Language & \cstd & \etoe & \cctx \\
\midrule
\endhead
\midrule
\multicolumn{4}{r}{\textit{Continued on next page}} \\
\endfoot
\bottomrule
\endlastfoot

\multicolumn{4}{l}{\textit{High-resource (9)}} \\
\midrule
Arabic & 11.82 & 12.13 & \textbf{12.82} \\
Chinese & 5.23 & \textbf{26.31} & 8.95 \\
Greek & 11.50 & 13.32 & \textbf{14.23} \\
Indonesian & 13.27 & 12.11 & \textbf{16.63} \\
Korean (KP) & 2.95 & 5.32 & \textbf{5.71} \\
Korean (KR) & 6.42 & \textbf{11.29} & 8.43 \\
Persian & 11.72 & 12.88 & \textbf{13.58} \\
Spanish (ES) & 14.97 & 13.79 & \textbf{18.01} \\
Spanish (MX) & 14.94 & 14.70 & \textbf{16.66} \\
\textbf{Avg} & 10.31 & 13.54 & \textbf{12.78} \\
\midrule

\multicolumn{4}{l}{\textit{Mid-resource (1)}} \\
\midrule
Azerbaijani & 10.20 & 13.04 & \textbf{15.07} \\
\textbf{Avg} & 10.20 & 13.04 & \textbf{15.07} \\
\midrule

\multicolumn{4}{l}{\textit{Low-resource (4)}} \\
\midrule
Amharic & 4.59 & 4.05 & \textbf{5.65} \\
Assamese & 9.08 & 11.17 & \textbf{11.79} \\
Hausa & 6.20 & 6.77 & \textbf{9.04} \\
Javanese & 9.74 & 9.93 & \textbf{13.45} \\
\textbf{Avg} & 7.40 & 7.98 & \textbf{9.98} \\
\midrule

\textbf{Overall (14)} & 9.47 & 11.91 & \textbf{12.14} \\
\end{longtable}



\begin{longtable}{lccc}
\caption{Llama-3.1-8B-Instruct chrF on Global-PIQA-OE: High-resource (44), Mid-resource (42) and Low-resource (30).} \\
\toprule
Language & \cstd & \etoe & \cctx \\
\midrule
\endfirsthead
\multicolumn{4}{c}{\tablename\ \thetable{} -- continued} \\
\toprule
Language & \cstd & \etoe & \cctx \\
\midrule
\endhead
\midrule
\multicolumn{4}{r}{\textit{Continued on next page}} \\
\endfoot
\bottomrule
\endlastfoot
\multicolumn{4}{l}{\textit{High-resource (44)}} \\
\midrule
Algerian Arabic & \textbf{10.56} & 9.06 & 9.92 \\
Burushaski & 2.66 & \textbf{5.23} & 4.32 \\
Cantonese & 2.56 & 3.53 & \textbf{3.94} \\
Chinese (Simplified) & 3.49 & 4.48 & \textbf{6.46} \\
Chinese (Traditional) & 3.84 & 4.98 & \textbf{8.71} \\
Czech & 11.08 & 8.77 & \textbf{13.65} \\
Dutch & \textbf{21.72} & 18.39 & 17.94 \\
Egyptian Arabic & 12.81 & 8.65 & \textbf{13.27} \\
English & \textbf{19.23} & 15.56 & 17.74 \\
French (Canada) & 18.74 & 16.82 & \textbf{21.85} \\
French (France) & 13.97 & \textbf{17.78} & 14.24 \\
German & 15.54 & 16.25 & \textbf{16.55} \\
Greek & 9.82 & 7.81 & \textbf{13.67} \\
Gulf Arabic & \textbf{11.01} & 8.45 & 10.23 \\
Hungarian & 16.63 & 14.42 & \textbf{17.92} \\
Indonesian & \textbf{21.30} & 17.89 & 18.78 \\
Italian & 12.81 & \textbf{24.10} & 21.37 \\
Japanese & 5.55 & 4.99 & \textbf{5.62} \\
Korean & 4.04 & 4.30 & \textbf{4.89} \\
Mesopotamian Arabic & 9.92 & 8.87 & \textbf{10.71} \\
Modern Standard Arabic & \textbf{12.88} & 9.04 & 12.10 \\
Moroccan Arabic & 10.54 & 9.08 & \textbf{10.61} \\
Najdi Arabic & 11.39 & 9.78 & \textbf{14.47} \\
North Levantine Arabic (Jordan) & 13.65 & 9.96 & \textbf{15.15} \\
North Levantine Arabic (Lebanon) & 7.90 & 6.79 & \textbf{10.36} \\
North Levantine Arabic (Palestine) & 7.28 & 6.80 & \textbf{9.64} \\
North Levantine Arabic (Syria) & 7.37 & 6.80 & \textbf{9.16} \\
Polish & 16.41 & 14.34 & \textbf{17.24} \\
Portuguese (Brazil) & 16.65 & \textbf{22.17} & 18.74 \\
Portuguese (Portugal) & 15.67 & 14.31 & \textbf{15.82} \\
Romanian & 16.10 & 13.90 & \textbf{16.51} \\
Russian & 15.59 & 14.60 & \textbf{16.62} \\
Slovak & 13.62 & 16.23 & \textbf{17.80} \\
Slovak (SARI) & 10.97 & 8.36 & \textbf{12.06} \\
Spanish (Mexico) & 16.55 & \textbf{19.11} & 17.06 \\
Spanish (Peru) & \textbf{18.86} & 18.13 & 17.86 \\
Spanish (Spain) & 18.43 & 17.09 & \textbf{19.28} \\
Swedish & 19.74 & 15.88 & \textbf{20.51} \\
Ta'izzi-Adeni Arabic & 10.25 & 8.82 & \textbf{12.54} \\
Tunisian Arabic & \textbf{11.46} & 9.70 & 10.20 \\
Turkish & 17.12 & 16.27 & \textbf{19.41} \\
Ukrainian & 14.13 & 9.81 & \textbf{14.46} \\
Vietnamese & 10.64 & 11.57 & \textbf{14.42} \\
Western Persian & 14.63 & 12.95 & \textbf{18.55} \\
\textbf{Avg} & 12.62 & 11.86 & \textbf{13.92} \\
\midrule
\multicolumn{4}{l}{\textit{Mid-resource (42)}} \\
\midrule
Armenian & 13.15 & 9.77 & \textbf{14.86} \\
Belarusian & 13.93 & 16.24 & \textbf{19.60} \\
Bengali & 11.25 & 12.81 & \textbf{13.61} \\
Bengali (Romanized) & 0.15 & \textbf{11.23} & 10.11 \\
Bosnian & 18.65 & 17.24 & \textbf{18.97} \\
Bulgarian & 16.58 & 13.83 & \textbf{19.13} \\
Catalan & 15.24 & 16.01 & \textbf{16.44} \\
Croatian & 13.69 & 13.96 & \textbf{14.34} \\
Eastern Panjabi & 12.34 & 14.37 & \textbf{15.27} \\
Finnish & 19.08 & 17.45 & \textbf{22.63} \\
Galician & 15.41 & 16.85 & \textbf{20.54} \\
Georgian & 13.82 & 13.33 & \textbf{16.76} \\
Gujarati & 13.36 & 15.61 & \textbf{15.95} \\
Hebrew & 12.72 & 8.70 & \textbf{15.07} \\
Hindi & 13.25 & 13.78 & \textbf{14.20} \\
Icelandic & 16.29 & 14.66 & \textbf{16.83} \\
Kannada & 16.99 & 19.60 & \textbf{20.65} \\
Kazakh & 14.95 & 18.14 & \textbf{20.10} \\
Kyrgyz & 14.99 & \textbf{17.10} & 16.85 \\
Lithuanian & 12.55 & 10.95 & \textbf{14.12} \\
Macedonian & \textbf{15.27} & 13.04 & 14.91 \\
Malayalam & 15.69 & \textbf{19.12} & 19.07 \\
Marathi & 10.20 & 14.47 & \textbf{15.49} \\
Nepali & 14.29 & 13.12 & \textbf{15.68} \\
North Azerbaijani & \textbf{14.08} & 13.25 & 13.72 \\
Northern Uzbek & 11.83 & 15.19 & \textbf{16.24} \\
Norwegian Bokmål & 17.86 & \textbf{17.96} & 17.34 \\
Norwegian Nynorsk & 16.63 & 15.79 & \textbf{17.48} \\
Serbian (Cyrillic) & 5.93 & 9.76 & \textbf{10.92} \\
Serbian (Latin) & 13.30 & 10.81 & \textbf{13.77} \\
Sinhala & 8.53 & 9.36 & \textbf{9.76} \\
Slovenian & 14.04 & 12.22 & \textbf{14.70} \\
Slovenian (CERK) & 9.77 & 7.95 & \textbf{9.96} \\
Standard Malay & 23.64 & 16.03 & \textbf{28.85} \\
Swahili & \textbf{14.80} & 13.55 & 12.76 \\
Tagalog & 21.37 & 19.60 & \textbf{24.72} \\
Tamil & 21.73 & 21.00 & \textbf{25.13} \\
Telugu & 17.07 & 18.59 & \textbf{20.48} \\
Thai & 12.84 & 8.68 & \textbf{15.19} \\
Tosk Albanian & 12.42 & 12.18 & \textbf{13.89} \\
Urdu & 12.89 & 12.65 & \textbf{15.78} \\
Urdu (Romanized) & 5.32 & 10.48 & \textbf{13.47} \\
\textbf{Avg} & 14.00 & 14.20 & \textbf{16.56} \\
\midrule
\multicolumn{4}{l}{\textit{Low-resource (30)}} \\
\midrule
Amharic & 4.04 & 6.45 & \textbf{7.72} \\
Assamese & 9.74 & 12.21 & \textbf{12.59} \\
Bambara & 5.32 & \textbf{13.25} & 10.29 \\
Bhojpuri & 11.72 & 11.57 & \textbf{12.82} \\
Central Kurdish & 10.00 & 9.50 & \textbf{16.01} \\
Dhundari & 10.69 & \textbf{11.51} & 11.36 \\
Ekpeye & 3.89 & \textbf{11.05} & 6.54 \\
Estonian & 14.39 & 11.24 & \textbf{18.64} \\
Faroese & 14.30 & 11.77 & \textbf{17.53} \\
Hausa & 11.76 & 8.45 & \textbf{13.13} \\
Hawaiian & 12.81 & 11.55 & \textbf{15.85} \\
Idoma & 3.89 & \textbf{10.80} & 7.71 \\
Igbo & 9.20 & 15.23 & \textbf{15.25} \\
Isoko & 4.08 & \textbf{12.30} & 6.66 \\
Javanese & 12.83 & 11.08 & \textbf{14.10} \\
Kinyarwanda & 8.80 & 11.21 & \textbf{12.86} \\
Kumzari & 1.19 & \textbf{2.98} & 1.51 \\
Lingala & 8.32 & \textbf{10.56} & 10.08 \\
Luo & 10.06 & \textbf{10.10} & 8.79 \\
Marwari & 9.68 & 10.13 & \textbf{11.20} \\
Meitei (Bengali script) & 9.19 & \textbf{11.90} & 10.91 \\
Meitei (Meitei script) & 0.06 & 13.26 & \textbf{14.47} \\
Nagamese & 7.55 & 9.09 & \textbf{11.15} \\
Nigerian Pidgin & 16.14 & 13.67 & \textbf{21.15} \\
Sindhi & 11.69 & 12.26 & \textbf{13.76} \\
Sindhi (Devanagari) & 2.20 & 9.03 & \textbf{10.11} \\
Urhobo & 5.18 & \textbf{13.18} & 10.42 \\
Uyghur & 6.64 & 10.83 & \textbf{11.13} \\
Yoruba & 4.15 & \textbf{9.25} & 7.94 \\
Zulu & 8.79 & \textbf{12.27} & 10.01 \\
\textbf{Avg} & 8.28 & 10.92 & \textbf{11.72} \\
\midrule
\textbf{Overall (116)} & 11.99 & 12.46 & \textbf{14.31} \\
\end{longtable}


\begin{longtable}{lccc}
\caption{Llama-3.1-8B-Instruct chrF on MKQA: High-resource (19), Mid-resource (6) and Low-resource (0).} \\
\toprule
Language & \cstd & \etoe & \cctx \\
\midrule
\endfirsthead
\multicolumn{4}{c}{\tablename\ \thetable{} -- continued} \\
\toprule
Language & \cstd & \etoe & \cctx \\
\midrule
\endhead
\midrule
\multicolumn{4}{r}{\textit{Continued on next page}} \\
\endfoot
\bottomrule
\endlastfoot
\multicolumn{4}{l}{\textit{High-resource (19)}} \\
\midrule
Arabic & 11.73 & 10.47 & \textbf{12.47} \\
Chinese (HK) & 4.72 & 7.61 & \textbf{8.07} \\
Chinese (Simplified) & 7.91 & 9.31 & \textbf{10.88} \\
Chinese (Traditional) & 5.24 & \textbf{7.89} & 7.68 \\
Danish & 17.48 & 8.65 & \textbf{17.57} \\
Dutch & 15.01 & 12.11 & \textbf{15.20} \\
French & 16.79 & 17.05 & \textbf{18.38} \\
German & 16.41 & 14.44 & \textbf{17.44} \\
Hungarian & 13.82 & 14.32 & \textbf{15.36} \\
Italian & 16.91 & 15.35 & \textbf{17.25} \\
Japanese & 14.23 & 12.73 & \textbf{15.90} \\
Korean & 6.71 & 5.09 & \textbf{7.07} \\
Polish & 16.25 & 15.35 & \textbf{18.12} \\
Portuguese & 15.99 & 10.77 & \textbf{17.07} \\
Russian & 13.93 & 12.09 & \textbf{14.58} \\
Spanish & 16.39 & 14.52 & \textbf{16.93} \\
Swedish & 17.31 & 10.32 & \textbf{17.64} \\
Turkish & \textbf{14.33} & 10.95 & 13.32 \\
Vietnamese & 13.79 & 13.07 & \textbf{14.45} \\
\textbf{Avg} & 13.42 & 11.69 & \textbf{14.49} \\
\midrule
\multicolumn{4}{l}{\textit{Mid-resource (6)}} \\
\midrule
Finnish & 16.24 & 15.20 & \textbf{18.57} \\
Hebrew & 13.86 & 12.43 & \textbf{17.15} \\
Khmer & 3.50 & 3.51 & \textbf{4.46} \\
Malay & \textbf{16.02} & 10.30 & 15.31 \\
Norwegian & 16.47 & 9.79 & \textbf{17.28} \\
Thai & 13.04 & 14.39 & \textbf{17.29} \\
\textbf{Avg} & 13.19 & 10.94 & \textbf{15.01} \\
\midrule
\textbf{Overall (25)} & 13.36 & 11.51 & \textbf{14.62} \\
\end{longtable}


==> latex/tables/mistral/mc_math.tex <==
\begin{table}[htbp]
\centering
\begin{tabular}{lccc}
\toprule
Dataset & \cstd & \etoe & \cctx \\
\midrule
Global MMLU & 26.29\% & 26.36\% & \textbf{32.07\%} \\
MCSQA & 57.12\% & \textbf{60.38\%} & 59.12\% \\
Belebele & 24.60\% & \textbf{33.69\%} & 25.92\% \\
Global-PIQA & 51.72\% & 50.60\% & \textbf{59.11\%} \\
MGSM & \textbf{26.82\%} & 20.18\% & 23.09\% \\
MMath & 3.60\% & 3.70\% & \textbf{3.90\%} \\
\bottomrule
\end{tabular}
\caption{Overall multiple-choice accuracy for Mistral-7B-Instruct.}
\end{table}

\begin{table}[htbp]
\centering
\begin{tabular}{lccc}
\toprule
Dataset & \cstd & \etoe & \cctx \\
\midrule
Aya & 9.71 & \textbf{12.61} & 11.99 \\
BLEnD & 8.32 & 7.20 & \textbf{9.10} \\
Global-PIQA-OE & 12.90 & 12.32 & \textbf{14.58} \\
MKQA & 11.29 & 10.17 & \textbf{12.09} \\
\bottomrule
\end{tabular}
\caption{Overall open-ended chrF for Mistral-7B-Instruct}
\end{table}





\begin{longtable}{lccc}
\caption{Mistral-7B-Instruct accuracy on Global MMLU: High-resource (22), Mid-resource (11) and Low-resource (9).} \\
\toprule
Language & \cstd & \etoe & \cctx \\
\midrule
\endfirsthead
\multicolumn{4}{c}{\tablename\ \thetable{} -- continued} \\
\toprule
Language & \cstd & \etoe & \cctx \\
\midrule
\endhead
\midrule
\multicolumn{4}{r}{\textit{Continued on next page}} \\
\endfoot
\bottomrule
\endlastfoot
\multicolumn{4}{l}{\textit{High-resource (22)}} \\
\midrule
Arabic & 23.00\% & 14.00\% & \textbf{28.00\%} \\
Chinese & 27.00\% & \textbf{33.00\%} & 31.00\% \\
Czech & 33.00\% & 27.00\% & \textbf{39.00\%} \\
Dutch & 34.00\% & 41.00\% & \textbf{42.00\%} \\
English & 32.00\% & 39.00\% & \textbf{40.00\%} \\
French & 33.00\% & 35.00\% & \textbf{42.00\%} \\
German & 31.00\% & 31.00\% & \textbf{35.00\%} \\
Greek & 25.00\% & 28.00\% & \textbf{29.00\%} \\
Indonesian & 27.00\% & 26.00\% & \textbf{36.00\%} \\
Italian & 31.00\% & 40.00\% & \textbf{45.00\%} \\
Japanese & 30.00\% & 26.00\% & \textbf{42.00\%} \\
Korean & 28.00\% & 27.00\% & \textbf{31.00\%} \\
Persian & 36.00\% & 24.00\% & \textbf{38.00\%} \\
Polish & 38.00\% & 35.00\% & \textbf{43.00\%} \\
Portuguese & 26.00\% & 30.00\% & \textbf{36.00\%} \\
Romanian & 34.00\% & 26.00\% & \textbf{37.00\%} \\
Russian & 30.00\% & 38.00\% & \textbf{39.00\%} \\
Spanish & 34.00\% & 31.00\% & \textbf{41.00\%} \\
Swedish & 26.00\% & \textbf{37.00\%} & 37.00\% \\
Turkish & 32.00\% & 33.00\% & \textbf{37.00\%} \\
Ukrainian & 34.00\% & 31.00\% & \textbf{43.00\%} \\
Vietnamese & 27.00\% & \textbf{31.00\%} & 29.00\% \\
\textbf{Avg} & 30.50\% & 31.05\% & \textbf{37.27\%} \\
\midrule
\multicolumn{4}{l}{\textit{Mid-resource (11)}} \\
\midrule
Bengali & 20.00\% & 24.00\% & \textbf{29.00\%} \\
Hebrew & 28.00\% & 21.00\% & \textbf{32.00\%} \\
Hindi & 25.00\% & 29.00\% & \textbf{32.00\%} \\
Kyrgyz & 19.00\% & \textbf{21.00\%} & 21.00\% \\
Lithuanian & 23.00\% & 23.00\% & \textbf{26.00\%} \\
Malay & 31.00\% & 25.00\% & \textbf{38.00\%} \\
Nepali & 21.00\% & \textbf{28.00\%} & 26.00\% \\
Serbian & 28.00\% & 30.00\% & \textbf{35.00\%} \\
Sinhala & 20.00\% & 4.00\% & \textbf{23.00\%} \\
Swahili & 22.00\% & 23.00\% & \textbf{29.00\%} \\
Telugu & 14.00\% & 12.00\% & \textbf{21.00\%} \\
\textbf{Avg} & 22.82\% & 21.82\% & \textbf{28.36\%} \\
\midrule
\multicolumn{4}{l}{\textit{Low-resource (9)}} \\
\midrule
Amharic & 29.00\% & 6.00\% & \textbf{31.00\%} \\
Chichewa & 15.00\% & \textbf{22.00\%} & 15.00\% \\
Filipino & 28.00\% & 25.00\% & \textbf{34.00\%} \\
Hausa & 13.00\% & 20.00\% & \textbf{22.00\%} \\
Igbo & 15.00\% & \textbf{28.00\%} & 20.00\% \\
Malagasy & 25.00\% & 23.00\% & \textbf{28.00\%} \\
Shona & 22.00\% & 22.00\% & \textbf{25.00\%} \\
Somali & 19.00\% & 19.00\% & \textbf{21.00\%} \\
Yoruba & 16.00\% & \textbf{19.00\%} & 19.00\% \\
\textbf{Avg} & 20.22\% & 20.44\% & \textbf{23.89\%} \\
\midrule
\textbf{Overall (42)} & 26.29\% & 26.36\% & \textbf{32.07\%} \\
\end{longtable}

\begin{longtable}{lccc}
\caption{Mistral-7B-Instruct accuracy on MCSQA: High-resource (8).} \\
\toprule
Language & \cstd & \etoe & \cctx \\
\midrule
\endfirsthead
\multicolumn{4}{c}{\tablename\ \thetable{} -- continued} \\
\toprule
Language & \cstd & \etoe & \cctx \\
\midrule
\endhead
\midrule
\multicolumn{4}{r}{\textit{Continued on next page}} \\
\endfoot
\bottomrule
\endlastfoot
\multicolumn{4}{l}{\textit{High-resource (8)}} \\
\midrule
Chinese & 55.00\% & \textbf{63.00\%} & 59.00\% \\
Dutch & 69.00\% & 67.00\% & \textbf{75.00\%} \\
English & 65.00\% & 65.00\% & \textbf{69.00\%} \\
French & 54.00\% & \textbf{62.00\%} & 58.00\% \\
German & 58.00\% & 59.00\% & \textbf{61.00\%} \\
Japanese & \textbf{66.00\%} & 63.00\% & 64.00\% \\
Portuguese & 57.00\% & \textbf{63.00\%} & 56.00\% \\
Russian & 33.00\% & \textbf{41.00\%} & 31.00\% \\
\textbf{Avg} & 57.12\% & \textbf{60.38\%} & 59.12\% \\
\midrule
\textbf{Overall (8)} & 57.12\% & \textbf{60.38\%} & 59.12\% \\
\end{longtable}

\begin{longtable}{lccc}
\caption{Mistral-7B-Instruct accuracy on Belebele: High-resource (31), Mid-resource (42) and Low-resource (48).} \\
\toprule
Language & \cstd & \etoe & \cctx \\
\midrule
\endfirsthead
\multicolumn{4}{c}{\tablename\ \thetable{} -- continued} \\
\toprule
Language & \cstd & \etoe & \cctx \\
\midrule
\endhead
\midrule
\multicolumn{4}{r}{\textit{Continued on next page}} \\
\endfoot
\bottomrule
\endlastfoot
\multicolumn{4}{l}{\textit{High-resource (31)}} \\
\midrule
Chinese (Simplified) & 30.00\% & \textbf{66.67\%} & 26.67\% \\
Chinese (Traditional) & 33.33\% & \textbf{56.67\%} & 40.00\% \\
Czech & 20.00\% & \textbf{63.33\%} & 16.67\% \\
Danish & 23.33\% & \textbf{56.67\%} & 26.67\% \\
Dutch & 26.67\% & \textbf{60.00\%} & 46.67\% \\
Egyptian Arabic & \textbf{33.33\%} & 33.33\% & 23.33\% \\
English & 56.67\% & \textbf{66.67\%} & 56.67\% \\
French & 33.33\% & \textbf{63.33\%} & 30.00\% \\
German & 26.67\% & \textbf{60.00\%} & 36.67\% \\
Greek & 20.00\% & \textbf{36.67\%} & 26.67\% \\
Hungarian & 16.67\% & \textbf{60.00\%} & 23.33\% \\
Indonesian & 20.00\% & \textbf{43.33\%} & 26.67\% \\
Italian & 40.00\% & \textbf{56.67\%} & 56.67\% \\
Japanese & 36.67\% & \textbf{50.00\%} & 36.67\% \\
Korean & 16.67\% & \textbf{46.67\%} & 20.00\% \\
Mesopotamian Arabic & 20.00\% & \textbf{46.67\%} & 23.33\% \\
Modern Standard Arabic & 50.00\% & \textbf{56.67\%} & 33.33\% \\
Modern Standard Arabic (Romanized) & \textbf{23.33\%} & 13.33\% & 16.67\% \\
Najdi Arabic & 20.00\% & \textbf{36.67\%} & 20.00\% \\
North Levantine Arabic & 20.00\% & \textbf{33.33\%} & 23.33\% \\
Polish & 26.67\% & \textbf{56.67\%} & 30.00\% \\
Portuguese & 23.33\% & \textbf{63.33\%} & 33.33\% \\
Romanian & 16.67\% & \textbf{50.00\%} & 23.33\% \\
Russian & 33.33\% & \textbf{60.00\%} & 30.00\% \\
Slovak & 16.67\% & \textbf{40.00\%} & 20.00\% \\
Spanish & 40.00\% & \textbf{56.67\%} & 40.00\% \\
Swedish & 26.67\% & \textbf{70.00\%} & 26.67\% \\
Turkish & 36.67\% & \textbf{43.33\%} & 36.67\% \\
Ukrainian & 43.33\% & \textbf{50.00\%} & 50.00\% \\
Vietnamese & 26.67\% & \textbf{56.67\%} & 30.00\% \\
Western Persian & 43.33\% & \textbf{50.00\%} & 43.33\% \\
\textbf{Avg} & 29.03\% & \textbf{51.72\%} & 31.40\% \\
\midrule
\multicolumn{4}{l}{\textit{Mid-resource (42)}} \\
\midrule
Afrikaans & 30.00\% & \textbf{43.33\%} & 30.00\% \\
Armenian & 16.67\% & \textbf{36.67\%} & 16.67\% \\
Basque & \textbf{30.00\%} & 16.67\% & 26.67\% \\
Bengali & \textbf{30.00\%} & 23.33\% & 26.67\% \\
Bengali (Romanized) & \textbf{23.33\%} & 16.67\% & 20.00\% \\
Bulgarian & 26.67\% & \textbf{53.33\%} & 26.67\% \\
Burmese & \textbf{23.33\%} & 10.00\% & 23.33\% \\
Catalan & 20.00\% & \textbf{76.67\%} & 23.33\% \\
Croatian & 30.00\% & \textbf{63.33\%} & 33.33\% \\
Eastern Panjabi & 20.00\% & \textbf{26.67\%} & 16.67\% \\
Finnish & 26.67\% & \textbf{40.00\%} & 23.33\% \\
Georgian & 16.67\% & \textbf{20.00\%} & 13.33\% \\
Gujarati & \textbf{26.67\%} & 20.00\% & 26.67\% \\
Hebrew & 33.33\% & 40.00\% & \textbf{43.33\%} \\
Hindi & 30.00\% & 26.67\% & \textbf{40.00\%} \\
Hindi (Romanized) & 20.00\% & \textbf{26.67\%} & 16.67\% \\
Icelandic & 23.33\% & \textbf{43.33\%} & 36.67\% \\
Kannada & 10.00\% & \textbf{20.00\%} & 16.67\% \\
Kazakh & 10.00\% & \textbf{30.00\%} & 13.33\% \\
Khmer & 13.33\% & 16.67\% & \textbf{26.67\%} \\
Kyrgyz & 16.67\% & \textbf{26.67\%} & 20.00\% \\
Lithuanian & 33.33\% & \textbf{43.33\%} & 40.00\% \\
Macedonian & 40.00\% & \textbf{60.00\%} & 36.67\% \\
Malayalam & 10.00\% & \textbf{23.33\%} & 13.33\% \\
Marathi & 26.67\% & \textbf{43.33\%} & 30.00\% \\
Nepali & 13.33\% & \textbf{20.00\%} & 20.00\% \\
North Azerbaijani & \textbf{43.33\%} & 33.33\% & 43.33\% \\
Northern Uzbek & 36.67\% & 26.67\% & \textbf{40.00\%} \\
Norwegian Bokmål & 30.00\% & \textbf{40.00\%} & 13.33\% \\
Serbian & 36.67\% & \textbf{56.67\%} & 36.67\% \\
Sinhala & \textbf{20.00\%} & 3.33\% & 16.67\% \\
Sinhala (Romanized) & 20.00\% & 20.00\% & \textbf{23.33\%} \\
Slovenian & 26.67\% & \textbf{50.00\%} & 23.33\% \\
Standard Malay & 30.00\% & \textbf{43.33\%} & 33.33\% \\
Swahili & 13.33\% & \textbf{33.33\%} & 16.67\% \\
Tagalog & 26.67\% & \textbf{33.33\%} & 23.33\% \\
Tamil & 20.00\% & \textbf{40.00\%} & 20.00\% \\
Telugu & 26.67\% & \textbf{33.33\%} & 20.00\% \\
Thai & 23.33\% & \textbf{30.00\%} & 23.33\% \\
Tosk Albanian & 26.67\% & \textbf{33.33\%} & 26.67\% \\
Urdu & 46.67\% & 30.00\% & \textbf{53.33\%} \\
Urdu (Romanized) & \textbf{36.67\%} & 20.00\% & 26.67\% \\
\textbf{Avg} & 25.32\% & \textbf{33.17\%} & 26.19\% \\
\midrule
\multicolumn{4}{l}{\textit{Low-resource (48)}} \\
\midrule
Amharic & \textbf{30.00\%} & 13.33\% & 16.67\% \\
Assamese & 33.33\% & 16.67\% & \textbf{43.33\%} \\
Bambara & 13.33\% & \textbf{16.67\%} & 13.33\% \\
Cebuano & \textbf{36.67\%} & 30.00\% & 36.67\% \\
Central Kurdish & \textbf{30.00\%} & 26.67\% & 16.67\% \\
Estonian & 23.33\% & \textbf{26.67\%} & 26.67\% \\
Ganda & 3.33\% & \textbf{20.00\%} & 6.67\% \\
Guarani & 20.00\% & \textbf{36.67\%} & 20.00\% \\
Haitian Creole & 23.33\% & \textbf{30.00\%} & 26.67\% \\
Halh Mongolian & \textbf{30.00\%} & 13.33\% & 30.00\% \\
Hausa & \textbf{23.33\%} & 16.67\% & 23.33\% \\
Igbo & 13.33\% & 13.33\% & \textbf{16.67\%} \\
Ilocano & 33.33\% & 26.67\% & \textbf{36.67\%} \\
Javanese & 16.67\% & \textbf{26.67\%} & 16.67\% \\
Jingpho & 10.00\% & \textbf{13.33\%} & 10.00\% \\
Kabuverdianu & 20.00\% & \textbf{33.33\%} & 23.33\% \\
Kinyarwanda & \textbf{20.00\%} & 20.00\% & 16.67\% \\
Lao & 26.67\% & 23.33\% & \textbf{33.33\%} \\
Lingala & 13.33\% & \textbf{23.33\%} & 13.33\% \\
Luo & 16.67\% & 16.67\% & \textbf{20.00\%} \\
Maltese & 30.00\% & 23.33\% & \textbf{36.67\%} \\
Maori & \textbf{26.67\%} & 16.67\% & 26.67\% \\
Nepali (Romanized) & 20.00\% & \textbf{26.67\%} & 20.00\% \\
Nigerian Fulfulde & \textbf{23.33\%} & 23.33\% & 23.33\% \\
Northern Sotho & 23.33\% & \textbf{30.00\%} & 23.33\% \\
Nyanja & 16.67\% & 20.00\% & \textbf{23.33\%} \\
Odia & \textbf{20.00\%} & 13.33\% & 16.67\% \\
Plateau Malagasy & 13.33\% & \textbf{30.00\%} & 13.33\% \\
Shan & \textbf{23.33\%} & 13.33\% & 16.67\% \\
Shona & 20.00\% & \textbf{33.33\%} & 16.67\% \\
Sindhi & 23.33\% & 20.00\% & \textbf{26.67\%} \\
Somali & 10.00\% & \textbf{23.33\%} & 10.00\% \\
Southern Pashto & \textbf{16.67\%} & 16.67\% & 16.67\% \\
Southern Sotho & 20.00\% & 13.33\% & \textbf{23.33\%} \\
Standard Latvian & 30.00\% & \textbf{36.67\%} & 23.33\% \\
Standard Tibetan & \textbf{13.33\%} & 6.67\% & 13.33\% \\
Sundanese & 23.33\% & \textbf{30.00\%} & 30.00\% \\
Swati & \textbf{26.67\%} & 26.67\% & 26.67\% \\
Tajik & 20.00\% & \textbf{23.33\%} & 23.33\% \\
Tigrinya & 6.67\% & \textbf{23.33\%} & 13.33\% \\
Tsonga & 26.67\% & 16.67\% & \textbf{30.00\%} \\
Tswana & \textbf{23.33\%} & 20.00\% & 23.33\% \\
Waray & 30.00\% & \textbf{43.33\%} & 30.00\% \\
West Central Oromo & 6.67\% & \textbf{13.33\%} & 10.00\% \\
Wolof & \textbf{33.33\%} & 30.00\% & 33.33\% \\
Xhosa & 13.33\% & 16.67\% & \textbf{23.33\%} \\
Yoruba & 16.67\% & 10.00\% & \textbf{23.33\%} \\
Zulu & 20.00\% & \textbf{36.67\%} & 20.00\% \\
\textbf{Avg} & 21.11\% & \textbf{22.50\%} & 22.15\% \\
\midrule
\textbf{Overall (121)} & 24.60\% & \textbf{33.69\%} & 25.92\% \\
\end{longtable}

\begin{longtable}{lccc}
\caption{Mistral-7B-Instruct accuracy on Global-PIQA: High-resource (44), Mid-resource (42) and Low-resource (30).} \\
\toprule
Language & \cstd & \etoe & \cctx \\
\midrule
\endfirsthead
\multicolumn{4}{c}{\tablename\ \thetable{} -- continued} \\
\toprule
Language & \cstd & \etoe & \cctx \\
\midrule
\endhead
\midrule
\multicolumn{4}{r}{\textit{Continued on next page}} \\
\endfoot
\bottomrule
\endlastfoot
\multicolumn{4}{l}{\textit{High-resource (44)}} \\
\midrule
Algerian Arabic & 40.00\% & 36.67\% & \textbf{60.00\%} \\
Burushaski & 26.67\% & \textbf{40.00\%} & 40.00\% \\
Cantonese & 60.00\% & 46.67\% & \textbf{66.67\%} \\
Chinese (Simplified) & 56.67\% & 63.33\% & \textbf{70.00\%} \\
Chinese (Traditional) & 40.00\% & \textbf{56.67\%} & 53.33\% \\
Czech & 56.67\% & 40.00\% & \textbf{70.00\%} \\
Dutch & 60.00\% & 56.67\% & \textbf{66.67\%} \\
Egyptian Arabic & 40.00\% & \textbf{53.33\%} & 50.00\% \\
English & 63.33\% & \textbf{76.67\%} & 66.67\% \\
French (Canada) & 76.67\% & 50.00\% & \textbf{80.00\%} \\
French (France) & \textbf{66.67\%} & 63.33\% & 66.67\% \\
German & 46.67\% & \textbf{50.00\%} & 50.00\% \\
Greek & 30.00\% & \textbf{50.00\%} & 40.00\% \\
Gulf Arabic & 63.33\% & 43.33\% & \textbf{70.00\%} \\
Hungarian & 83.33\% & 80.00\% & \textbf{86.67\%} \\
Indonesian & 76.67\% & 73.33\% & \textbf{83.33\%} \\
Italian & 60.00\% & 43.33\% & \textbf{70.00\%} \\
Japanese & 60.00\% & 63.33\% & \textbf{66.67\%} \\
Korean & 46.67\% & 43.33\% & \textbf{56.67\%} \\
Mesopotamian Arabic & 53.33\% & \textbf{70.00\%} & 63.33\% \\
Modern Standard Arabic & 53.33\% & \textbf{60.00\%} & 46.67\% \\
Moroccan Arabic & 40.00\% & \textbf{66.67\%} & 56.67\% \\
Najdi Arabic & 46.67\% & 30.00\% & \textbf{53.33\%} \\
North Levantine Arabic (Jordan) & 66.67\% & 40.00\% & \textbf{70.00\%} \\
North Levantine Arabic (Lebanon) & 50.00\% & 66.67\% & \textbf{70.00\%} \\
North Levantine Arabic (Palestine) & 46.67\% & 50.00\% & \textbf{63.33\%} \\
North Levantine Arabic (Syria) & 50.00\% & 53.33\% & \textbf{60.00\%} \\
Polish & 46.67\% & 46.67\% & \textbf{53.33\%} \\
Portuguese (Brazil) & 50.00\% & \textbf{76.67\%} & 70.00\% \\
Portuguese (Portugal) & 73.33\% & 66.67\% & \textbf{80.00\%} \\
Romanian & 86.67\% & 73.33\% & \textbf{93.33\%} \\
Russian & 60.00\% & 56.67\% & \textbf{66.67\%} \\
Slovak & 53.33\% & 36.67\% & \textbf{60.00\%} \\
Slovak (SARI) & \textbf{63.33\%} & 36.67\% & 63.33\% \\
Spanish (Mexico) & 76.67\% & 80.00\% & \textbf{90.00\%} \\
Spanish (Peru) & 83.33\% & 70.00\% & \textbf{90.00\%} \\
Spanish (Spain) & 66.67\% & 66.67\% & \textbf{70.00\%} \\
Swedish & 60.00\% & \textbf{66.67\%} & 66.67\% \\
Ta'izzi-Adeni Arabic & 63.33\% & 53.33\% & \textbf{73.33\%} \\
Tunisian Arabic & \textbf{56.67\%} & 53.33\% & 56.67\% \\
Turkish & 60.00\% & 66.67\% & \textbf{73.33\%} \\
Ukrainian & 56.67\% & 56.67\% & \textbf{73.33\%} \\
Vietnamese & 46.67\% & 43.33\% & \textbf{53.33\%} \\
Western Persian & 46.67\% & \textbf{50.00\%} & 50.00\% \\
\textbf{Avg} & 57.05\% & 56.06\% & \textbf{65.45\%} \\
\midrule
\multicolumn{4}{l}{\textit{Mid-resource (42)}} \\
\midrule
Armenian & 10.00\% & \textbf{53.33\%} & 20.00\% \\
Belarusian & 53.33\% & 36.67\% & \textbf{63.33\%} \\
Bengali & 30.00\% & \textbf{53.33\%} & 43.33\% \\
Bengali (Romanized) & 30.00\% & 16.67\% & \textbf{36.67\%} \\
Bosnian & 90.00\% & 73.33\% & \textbf{93.33\%} \\
Bulgarian & 56.67\% & 53.33\% & \textbf{73.33\%} \\
Catalan & 66.67\% & 40.00\% & \textbf{73.33\%} \\
Croatian & 66.67\% & 63.33\% & \textbf{76.67\%} \\
Eastern Panjabi & 43.33\% & \textbf{56.67\%} & 56.67\% \\
Finnish & 56.67\% & 56.67\% & \textbf{60.00\%} \\
Galician & 56.67\% & 43.33\% & \textbf{63.33\%} \\
Georgian & \textbf{60.00\%} & 46.67\% & 56.67\% \\
Gujarati & 40.00\% & 36.67\% & \textbf{46.67\%} \\
Hebrew & 46.67\% & 33.33\% & \textbf{53.33\%} \\
Hindi & \textbf{63.33\%} & 53.33\% & 63.33\% \\
Icelandic & 56.67\% & 40.00\% & \textbf{66.67\%} \\
Kannada & 36.67\% & \textbf{56.67\%} & 50.00\% \\
Kazakh & 23.33\% & \textbf{33.33\%} & 30.00\% \\
Kyrgyz & \textbf{63.33\%} & 20.00\% & 63.33\% \\
Lithuanian & 60.00\% & \textbf{80.00\%} & 56.67\% \\
Macedonian & 60.00\% & 60.00\% & \textbf{73.33\%} \\
Malayalam & 43.33\% & 23.33\% & \textbf{46.67\%} \\
Marathi & 60.00\% & 43.33\% & \textbf{66.67\%} \\
Nepali & 60.00\% & 60.00\% & \textbf{63.33\%} \\
North Azerbaijani & 36.67\% & \textbf{50.00\%} & 46.67\% \\
Northern Uzbek & 46.67\% & 46.67\% & \textbf{60.00\%} \\
Norwegian Bokmål & \textbf{76.67\%} & 60.00\% & 76.67\% \\
Norwegian Nynorsk & 43.33\% & \textbf{53.33\%} & 46.67\% \\
Serbian (Cyrillic) & \textbf{70.00\%} & 33.33\% & 53.33\% \\
Serbian (Latin) & 53.33\% & \textbf{63.33\%} & 53.33\% \\
Sinhala & 36.67\% & 10.00\% & \textbf{40.00\%} \\
Slovenian & 53.33\% & 40.00\% & \textbf{60.00\%} \\
Slovenian (CERK) & 36.67\% & \textbf{50.00\%} & 40.00\% \\
Standard Malay & 70.00\% & \textbf{76.67\%} & 73.33\% \\
Swahili & 60.00\% & 56.67\% & \textbf{63.33\%} \\
Tagalog & \textbf{60.00\%} & 50.00\% & 50.00\% \\
Tamil & \textbf{33.33\%} & 26.67\% & 33.33\% \\
Telugu & \textbf{40.00\%} & 33.33\% & 36.67\% \\
Thai & 46.67\% & 56.67\% & \textbf{60.00\%} \\
Tosk Albanian & \textbf{60.00\%} & 43.33\% & 60.00\% \\
Urdu & 60.00\% & 60.00\% & \textbf{73.33\%} \\
Urdu (Romanized) & 56.67\% & 30.00\% & \textbf{60.00\%} \\
\textbf{Avg} & 51.75\% & 46.98\% & \textbf{56.75\%} \\
\midrule
\multicolumn{4}{l}{\textit{Low-resource (30)}} \\
\midrule
Amharic & 40.00\% & 26.67\% & \textbf{53.33\%} \\
Assamese & 33.33\% & \textbf{60.00\%} & 40.00\% \\
Bambara & 36.67\% & 30.00\% & \textbf{50.00\%} \\
Bhojpuri & 46.67\% & 43.33\% & \textbf{53.33\%} \\
Central Kurdish & 33.33\% & \textbf{50.00\%} & 43.33\% \\
Dhundari & 50.00\% & 56.67\% & \textbf{63.33\%} \\
Ekpeye & 40.00\% & \textbf{56.67\%} & 43.33\% \\
Estonian & 36.67\% & \textbf{46.67\%} & 40.00\% \\
Faroese & 43.33\% & 43.33\% & \textbf{70.00\%} \\
Hausa & 46.67\% & 50.00\% & \textbf{56.67\%} \\
Hawaiian & 36.67\% & 43.33\% & \textbf{53.33\%} \\
Idoma & 30.00\% & 40.00\% & \textbf{50.00\%} \\
Igbo & 33.33\% & 43.33\% & \textbf{50.00\%} \\
Isoko & 50.00\% & 36.67\% & \textbf{53.33\%} \\
Javanese & 53.33\% & 50.00\% & \textbf{63.33\%} \\
Kinyarwanda & 43.33\% & 26.67\% & \textbf{50.00\%} \\
Kumzari & 36.67\% & 46.67\% & \textbf{56.67\%} \\
Lingala & 33.33\% & \textbf{60.00\%} & 43.33\% \\
Luo & 36.67\% & \textbf{66.67\%} & 50.00\% \\
Marwari & \textbf{60.00\%} & 56.67\% & 60.00\% \\
Meitei (Bengali script) & 40.00\% & 33.33\% & \textbf{50.00\%} \\
Meitei (Meitei script) & 50.00\% & 43.33\% & \textbf{53.33\%} \\
Nagamese & 43.33\% & 53.33\% & \textbf{66.67\%} \\
Nigerian Pidgin & 66.67\% & \textbf{80.00\%} & 73.33\% \\
Sindhi & \textbf{66.67\%} & 36.67\% & 60.00\% \\
Sindhi (Devanagari) & 56.67\% & \textbf{60.00\%} & 43.33\% \\
Urhobo & 36.67\% & 40.00\% & \textbf{50.00\%} \\
Uyghur & 50.00\% & \textbf{53.33\%} & 53.33\% \\
Yoruba & 40.00\% & 36.67\% & \textbf{46.67\%} \\
Zulu & 46.67\% & \textbf{60.00\%} & 53.33\% \\
\textbf{Avg} & 43.89\% & 47.67\% & \textbf{53.11\%} \\
\midrule
\textbf{Overall (116)} & 51.72\% & 50.60\% & \textbf{59.11\%} \\
\end{longtable}

\begin{longtable}{lccc}
\caption{Mistral-7B-Instruct accuracy on MGSM: High-resource (7) and Mid-resource (4).} \\
\toprule
Language & \cstd & \etoe & \cctx \\
\midrule
\endfirsthead
\multicolumn{4}{c}{\tablename\ \thetable{} -- continued} \\
\toprule
Language & \cstd & \etoe & \cctx \\
\midrule
\endhead
\midrule
\multicolumn{4}{r}{\textit{Continued on next page}} \\
\endfoot
\bottomrule
\endlastfoot
\multicolumn{4}{l}{\textit{High-resource (7)}} \\
\midrule
Chinese & 32.00\% & \textbf{36.00\%} & 25.00\% \\
English & 41.00\% & 41.00\% & \textbf{42.00\%} \\
French & \textbf{37.00\%} & 32.00\% & 37.00\% \\
German & \textbf{33.00\%} & 18.00\% & 29.00\% \\
Japanese & \textbf{26.00\%} & 18.00\% & 21.00\% \\
Russian & \textbf{38.00\%} & 29.00\% & 33.00\% \\
Spanish & \textbf{36.00\%} & 22.00\% & 35.00\% \\
\textbf{Avg} & \textbf{34.71\%} & 28.00\% & 31.71\% \\
\midrule
\multicolumn{4}{l}{\textit{Mid-resource (4)}} \\
\midrule
Bengali & \textbf{17.00\%} & 4.00\% & 5.00\% \\
Swahili & \textbf{7.00\%} & 3.00\% & 7.00\% \\
Telugu & \textbf{5.00\%} & 3.00\% & 3.00\% \\
Thai & \textbf{23.00\%} & 16.00\% & 17.00\% \\
\textbf{Avg} & \textbf{13.00\%} & 6.50\% & 8.00\% \\
\midrule
\textbf{Overall (11)} & \textbf{26.82\%} & 20.18\% & 23.09\% \\
\end{longtable}

\begin{longtable}{lccc}
\caption{Mistral-7B-Instruct accuracy on MMath: High-resource (9) and Mid-resource (1).} \\
\toprule
Language & \cstd & \etoe & \cctx \\
\midrule
\endfirsthead
\multicolumn{4}{c}{\tablename\ \thetable{} -- continued} \\
\toprule
Language & \cstd & \etoe & \cctx \\
\midrule
\endhead
\midrule
\multicolumn{4}{r}{\textit{Continued on next page}} \\
\endfoot
\bottomrule
\endlastfoot
\multicolumn{4}{l}{\textit{High-resource (9)}} \\
\midrule
Arabic & \textbf{6.00\%} & 0.00\% & 6.00\% \\
Chinese & \textbf{5.00\%} & 5.00\% & 5.00\% \\
English & \textbf{5.00\%} & 5.00\% & 5.00\% \\
French & 5.00\% & 4.00\% & \textbf{7.00\%} \\
Japanese & 1.00\% & \textbf{4.00\%} & 2.00\% \\
Korean & \textbf{2.00\%} & 1.00\% & 2.00\% \\
Portuguese & 3.00\% & \textbf{6.00\%} & 3.00\% \\
Spanish & 2.00\% & \textbf{4.00\%} & 2.00\% \\
Vietnamese & 2.00\% & \textbf{4.00\%} & 2.00\% \\
\textbf{Avg} & 3.44\% & 3.67\% & \textbf{3.78\%} \\
\midrule
\multicolumn{4}{l}{\textit{Mid-resource (1)}} \\
\midrule
Thai & \textbf{5.00\%} & 4.00\% & 5.00\% \\
\textbf{Avg} & \textbf{5.00\%} & 4.00\% & 5.00\% \\
\midrule
\textbf{Overall (10)} & 3.60\% & 3.70\% & \textbf{3.90\%} \\
\end{longtable}

\begin{longtable}{lccc}
\caption{Mistral-7B-Instruct chrF on Aya: High-resource (4), Mid-resource (1) and Low-resource (1).} \\
\toprule
Language & \cstd & \etoe & \cctx \\
\midrule
\endfirsthead
\multicolumn{4}{c}{\tablename\ \thetable{} -- continued} \\
\toprule
Language & \cstd & \etoe & \cctx \\
\midrule
\endhead
\midrule
\multicolumn{4}{r}{\textit{Continued on next page}} \\
\endfoot
\bottomrule
\endlastfoot
\multicolumn{4}{l}{\textit{High-resource (4)}} \\
\midrule
Arabic & 9.25 & 9.18 & \textbf{11.21} \\
Chinese & 4.87 & \textbf{10.12} & 8.35 \\
Portuguese & 22.52 & \textbf{26.96} & 26.79 \\
Turkish & 15.41 & 17.67 & \textbf{18.02} \\
\textbf{Avg} & 13.01 & 15.98 & \textbf{16.09} \\
\midrule
\multicolumn{4}{l}{\textit{Mid-resource (1)}} \\
\midrule
Telugu & 3.36 & \textbf{8.19} & 5.09 \\
\textbf{Avg} & 3.36 & \textbf{8.19} & 5.09 \\
\midrule
\multicolumn{4}{l}{\textit{Low-resource (1)}} \\
\midrule
Yoruba & 2.86 & \textbf{3.51} & 2.50 \\
\textbf{Avg} & 2.86 & \textbf{3.51} & 2.50 \\
\midrule
\textbf{Overall (6)} & 9.71 & \textbf{12.60} & 11.99 \\
\end{longtable}



\begin{longtable}{lccc}
\caption{Mistral-7B-Instruct chrF on BLEnD: High-resource (9), Mid-resource (1) and Low-resource (4).} \\
\toprule
Language & \cstd & \etoe & \cctx \\
\midrule
\endfirsthead
\multicolumn{4}{c}{\tablename\ \thetable{} -- continued} \\
\toprule
Language & \cstd & \etoe & \cctx \\
\midrule
\endhead
\midrule
\multicolumn{4}{r}{\textit{Continued on next page}} \\
\endfoot
\bottomrule
\endlastfoot
\multicolumn{4}{l}{\textit{High-resource (9)}} \\
\midrule
Arabic & 10.47 & 5.23 & \textbf{10.80} \\
Chinese & 6.03 & \textbf{8.37} & 7.53 \\
Greek & 10.65 & 5.68 & \textbf{11.28} \\
Indonesian & 13.16 & 13.09 & \textbf{13.18} \\
Korean (KP) & 1.85 & \textbf{4.34} & 3.64 \\
Korean (KR) & 4.43 & 4.41 & \textbf{5.33} \\
Persian & \textbf{9.16} & 5.52 & 9.15 \\
Spanish (ES) & 15.81 & \textbf{17.41} & 16.52 \\
Spanish (MX) & 15.29 & 16.06 & \textbf{16.89} \\
\textbf{Avg} & 9.65 & 8.90 & \textbf{10.48} \\
\midrule
\multicolumn{4}{l}{\textit{Mid-resource (1)}} \\
\midrule
Azerbaijani & 8.81 & 6.83 & \textbf{9.31} \\
\textbf{Avg} & 8.81 & 6.83 & \textbf{9.31} \\
\midrule
\multicolumn{4}{l}{\textit{Low-resource (4)}} \\
\midrule
Amharic & 1.39 & 0.82 & \textbf{2.51} \\
Assamese & 6.16 & 2.49 & \textbf{7.74} \\
Hausa & 3.66 & \textbf{3.84} & 3.54 \\
Javanese & 8.95 & 5.86 & \textbf{9.24} \\
\textbf{Avg} & 5.04 & 3.25 & \textbf{5.76} \\
\midrule
\textbf{Overall (14)} & 8.27 & 7.14 & \textbf{9.05} \\
\end{longtable}



\begin{longtable}{lccc}
\caption{Mistral-7B-Instruct chrF on Global-PIQA-OE: High-resource (44), Mid-resource (42) and Low-resource (30).} \\
\toprule
Language & \cstd & \etoe & \cctx \\
\midrule
\endfirsthead
\multicolumn{4}{c}{\tablename\ \thetable{} -- continued} \\
\toprule
Language & \cstd & \etoe & \cctx \\
\midrule
\endhead
\midrule
\multicolumn{4}{r}{\textit{Continued on next page}} \\
\endfoot
\bottomrule
\endlastfoot
\multicolumn{4}{l}{\textit{High-resource (44)}} \\
\midrule
Algerian Arabic & \textbf{12.25} & 5.37 & 12.00 \\
Burushaski & 2.92 & 3.64 & \textbf{5.28} \\
Cantonese & 1.79 & 1.66 & \textbf{3.45} \\
Chinese (Simplified) & 2.70 & \textbf{7.19} & 6.12 \\
Chinese (Traditional) & 2.87 & \textbf{9.21} & 7.00 \\
Czech & 14.27 & 14.49 & \textbf{15.87} \\
Dutch & \textbf{23.82} & 23.43 & 22.12 \\
Egyptian Arabic & 14.01 & 5.79 & \textbf{15.06} \\
English & 21.18 & \textbf{25.88} & 24.93 \\
French (Canada) & 24.10 & 22.63 & \textbf{24.52} \\
French (France) & 20.78 & 20.38 & \textbf{21.38} \\
German & 19.28 & 18.55 & \textbf{20.31} \\
Greek & 10.08 & 10.36 & \textbf{11.00} \\
Gulf Arabic & 11.47 & 5.65 & \textbf{12.41} \\
Hungarian & 21.76 & 17.07 & \textbf{21.96} \\
Indonesian & \textbf{22.96} & 21.92 & 22.88 \\
Italian & 18.80 & 21.24 & \textbf{22.88} \\
Japanese & 4.11 & 2.70 & \textbf{6.27} \\
Korean & 3.34 & 3.83 & \textbf{5.02} \\
Mesopotamian Arabic & 12.67 & 5.13 & \textbf{14.31} \\
Modern Standard Arabic & \textbf{12.31} & 7.82 & 12.29 \\
Moroccan Arabic & 12.14 & 5.77 & \textbf{12.48} \\
Najdi Arabic & 15.86 & 7.73 & \textbf{17.24} \\
North Levantine Arabic (Jordan) & 15.56 & 10.06 & \textbf{17.53} \\
North Levantine Arabic (Lebanon) & 12.53 & 5.47 & \textbf{12.77} \\
North Levantine Arabic (Palestine) & 11.06 & 5.06 & \textbf{11.55} \\
North Levantine Arabic (Syria) & 11.82 & 6.02 & \textbf{12.83} \\
Polish & 19.63 & 17.51 & \textbf{20.28} \\
Portuguese (Brazil) & 18.81 & \textbf{19.04} & 18.49 \\
Portuguese (Portugal) & 18.98 & \textbf{20.91} & 20.28 \\
Romanian & 19.73 & 18.21 & \textbf{20.20} \\
Russian & 20.71 & \textbf{22.50} & 21.98 \\
Slovak & 15.81 & \textbf{17.14} & 17.08 \\
Slovak (SARI) & 11.03 & 10.12 & \textbf{11.82} \\
Spanish (Mexico) & 25.11 & 25.92 & \textbf{26.49} \\
Spanish (Peru) & 23.18 & 22.98 & \textbf{23.79} \\
Spanish (Spain) & 22.80 & 23.07 & \textbf{23.87} \\
Swedish & 21.71 & 20.82 & \textbf{24.33} \\
Ta'izzi-Adeni Arabic & 13.65 & 5.27 & \textbf{16.13} \\
Tunisian Arabic & 12.79 & 5.48 & \textbf{13.66} \\
Turkish & 18.94 & 19.69 & \textbf{19.94} \\
Ukrainian & 16.47 & 14.80 & \textbf{17.49} \\
Vietnamese & 12.82 & \textbf{17.69} & 14.38 \\
Western Persian & 15.35 & 14.67 & \textbf{17.70} \\
\textbf{Avg} & 15.09 & 13.41 & \textbf{16.35} \\
\midrule
\multicolumn{4}{l}{\textit{Mid-resource (42)}} \\
\midrule
Armenian & 11.47 & \textbf{15.42} & 14.00 \\
Belarusian & 12.64 & 15.78 & \textbf{18.36} \\
Bengali & 8.86 & 4.61 & \textbf{10.40} \\
Bengali (Romanized) & 7.00 & \textbf{11.54} & 4.92 \\
Bosnian & \textbf{23.91} & 21.04 & 23.53 \\
Bulgarian & 23.91 & 20.38 & \textbf{24.04} \\
Catalan & 20.56 & 17.68 & \textbf{21.41} \\
Croatian & \textbf{16.26} & 16.06 & 15.29 \\
Eastern Panjabi & 8.53 & 7.45 & \textbf{8.69} \\
Finnish & 19.55 & 17.43 & \textbf{20.73} \\
Galician & 18.64 & 20.07 & \textbf{22.22} \\
Georgian & 10.30 & 11.52 & \textbf{11.56} \\
Gujarati & 6.41 & 8.53 & \textbf{9.64} \\
Hebrew & 13.78 & 9.33 & \textbf{16.00} \\
Hindi & 10.74 & 11.60 & \textbf{13.22} \\
Icelandic & 17.49 & 15.03 & \textbf{18.06} \\
Kannada & 11.79 & \textbf{17.25} & 13.51 \\
Kazakh & 11.74 & 11.81 & \textbf{13.33} \\
Kyrgyz & \textbf{11.23} & 9.47 & 10.99 \\
Lithuanian & \textbf{11.39} & 8.62 & 10.55 \\
Macedonian & \textbf{17.52} & 15.18 & 17.41 \\
Malayalam & 10.33 & \textbf{13.36} & 12.64 \\
Marathi & 8.45 & 6.67 & \textbf{12.54} \\
Nepali & 11.13 & 11.11 & \textbf{14.98} \\
North Azerbaijani & 14.75 & 11.99 & \textbf{15.97} \\
Northern Uzbek & 13.48 & \textbf{16.10} & 13.46 \\
Norwegian Bokmål & 20.31 & 19.91 & \textbf{20.62} \\
Norwegian Nynorsk & 18.70 & 17.78 & \textbf{19.92} \\
Serbian (Cyrillic) & 16.34 & 13.56 & \textbf{17.32} \\
Serbian (Latin) & 17.49 & 16.05 & \textbf{19.01} \\
Sinhala & 5.40 & 4.47 & \textbf{6.58} \\
Slovenian & 17.23 & 17.44 & \textbf{18.29} \\
Slovenian (CERK) & \textbf{11.76} & 9.61 & 11.52 \\
Standard Malay & 17.49 & \textbf{25.73} & 20.77 \\
Swahili & 10.75 & \textbf{13.24} & 13.03 \\
Tagalog & 25.77 & 26.88 & \textbf{27.56} \\
Tamil & 13.48 & \textbf{17.78} & 16.94 \\
Telugu & 7.86 & \textbf{11.38} & 10.11 \\
Thai & 11.83 & 12.36 & \textbf{13.47} \\
Tosk Albanian & 13.28 & 12.54 & \textbf{14.24} \\
Urdu & 13.11 & 13.27 & \textbf{16.07} \\
Urdu (Romanized) & \textbf{13.68} & 12.02 & 11.59 \\
\textbf{Avg} & 13.96 & 14.02 & \textbf{15.35} \\
\midrule
\multicolumn{4}{l}{\textit{Low-resource (30)}} \\
\midrule
Amharic & 1.66 & 1.29 & \textbf{2.58} \\
Assamese & 8.10 & 2.63 & \textbf{8.86} \\
Bambara & 5.91 & 9.78 & \textbf{9.91} \\
Bhojpuri & 8.57 & 5.98 & \textbf{10.07} \\
Central Kurdish & 8.41 & 4.87 & \textbf{12.70} \\
Dhundari & 7.45 & 4.92 & \textbf{10.25} \\
Ekpeye & 4.38 & \textbf{6.28} & 4.64 \\
Estonian & 14.14 & 9.94 & \textbf{14.62} \\
Faroese & 14.58 & 14.52 & \textbf{17.55} \\
Hausa & 9.90 & \textbf{10.45} & 9.48 \\
Hawaiian & 11.99 & 12.62 & \textbf{16.53} \\
Idoma & 5.59 & \textbf{7.95} & 7.90 \\
Igbo & 9.51 & 15.30 & \textbf{17.16} \\
Isoko & 5.40 & 8.30 & \textbf{10.06} \\
Javanese & 15.19 & 11.69 & \textbf{15.59} \\
Kinyarwanda & 9.55 & 11.07 & \textbf{12.44} \\
Kumzari & 3.11 & \textbf{4.55} & 1.17 \\
Lingala & 9.86 & \textbf{11.97} & 11.56 \\
Luo & 9.01 & \textbf{11.71} & 10.18 \\
Marwari & 9.21 & 7.15 & \textbf{11.17} \\
Meitei (Bengali script) & 2.65 & 1.89 & \textbf{2.88} \\
Meitei (Meitei script) & 0.01 & 3.32 & \textbf{10.38} \\
Nagamese & 12.73 & 10.05 & \textbf{13.14} \\
Nigerian Pidgin & 19.35 & 20.24 & \textbf{20.81} \\
Sindhi & 7.17 & 3.70 & \textbf{9.97} \\
Sindhi (Devanagari) & 3.91 & 4.61 & \textbf{7.68} \\
Urhobo & 6.32 & 10.76 & \textbf{15.49} \\
Uyghur & 8.23 & 3.55 & \textbf{10.40} \\
Yoruba & 4.81 & 7.31 & \textbf{8.38} \\
Zulu & 9.93 & 11.52 & \textbf{13.90} \\
\textbf{Avg} & 8.22 & 8.33 & \textbf{10.91} \\
\midrule
\textbf{Overall (116)} & 12.90 & 12.32 & \textbf{14.58} \\
\end{longtable}



\begin{longtable}{lccc}
\caption{Mistral-7B-Instruct chrF on MKQA: High-resource (19) and Mid-resource (6).} \\
\toprule
Language & \cstd & \etoe & \cctx \\
\midrule
\endfirsthead
\multicolumn{4}{c}{\tablename\ \thetable{} -- continued} \\
\toprule
Language & \cstd & \etoe & \cctx \\
\midrule
\endhead
\midrule
\multicolumn{4}{r}{\textit{Continued on next page}} \\
\endfoot
\bottomrule
\endlastfoot
\multicolumn{4}{l}{\textit{High-resource (19)}} \\
\midrule
Arabic & 10.03 & 5.79 & \textbf{10.55} \\
Chinese (HK) & 5.43 & 3.90 & \textbf{6.10} \\
Chinese (Simplified) & 3.96 & 3.04 & \textbf{4.82} \\
Chinese (Traditional) & 3.63 & 2.75 & \textbf{4.10} \\
Danish & 15.62 & 14.22 & \textbf{16.59} \\
Dutch & 14.06 & \textbf{16.62} & 14.54 \\
French & 15.33 & 15.93 & \textbf{16.32} \\
German & 16.36 & 15.34 & \textbf{17.47} \\
Hungarian & 14.59 & 14.04 & \textbf{15.24} \\
Italian & 16.42 & 15.67 & \textbf{17.27} \\
Japanese & 6.40 & 4.07 & \textbf{10.74} \\
Korean & 3.88 & 2.46 & \textbf{4.70} \\
Polish & 14.64 & 13.01 & \textbf{15.19} \\
Portuguese & 15.53 & 16.29 & \textbf{16.32} \\
Russian & 12.46 & 11.10 & \textbf{12.91} \\
Spanish & 14.98 & \textbf{17.72} & 15.63 \\
Swedish & 15.97 & 14.52 & \textbf{17.28} \\
Turkish & \textbf{13.52} & 8.84 & \textbf{13.52} \\
Vietnamese & 11.69 & 10.48 & \textbf{12.44} \\
\textbf{Avg} & 11.82 & 10.83 & \textbf{12.72} \\
\midrule
\multicolumn{4}{l}{\textit{Mid-resource (6)}} \\
\midrule
Finnish & 11.74 & 10.62 & \textbf{12.33} \\
Hebrew & 7.96 & 4.86 & \textbf{8.36} \\
Khmer & 1.87 & \textbf{2.58} & 2.13 \\
Malay & 13.38 & 11.44 & \textbf{13.61} \\
Norwegian & 14.98 & 13.37 & \textbf{15.72} \\
Thai & 7.84 & 5.55 & \textbf{8.48} \\
\textbf{Avg} & 9.63 & 8.07 & \textbf{10.11} \\
\midrule
\textbf{Overall (25)} & 11.29 & 10.17 & \textbf{12.09} \\
\end{longtable}


==> latex/tables/mkqa.tex <==
% \clearpage
% \begin{table}[t]
% \centering
% \small
% \setlength{\tabcolsep}{4pt}
% \begin{tabular}{lccc}
% \toprule
% \textbf{Language} & \textbf{Standard} & \textbf{Context} & \textbf{End-to-end} \\
% \midrule
% German & 16.36 & \textbf{17.47} & 15.34 \\
% Spanish & 14.98 & 15.63 & \textbf{17.72} \\
% Finnish & 11.74 & \textbf{12.33} & 10.62 \\
% French & 15.33 & \textbf{16.32} & 15.93 \\
% Hungarian & 14.59 & \textbf{15.24} & 14.04 \\
% Italian & 16.42 & \textbf{17.27} & 15.67 \\
% Korean & 3.88 & \textbf{4.70} & 2.46 \\
% Dutch & 14.06 & 14.54 & \textbf{16.62} \\
% Polish & 14.64 & \textbf{15.19} & 13.01 \\
% Portuguese & 15.53 & \textbf{16.32} & 16.29 \\
% Russian & 12.46 & \textbf{12.91} & 11.10 \\
% Swedish & 15.97 & \textbf{17.28} & 14.52 \\
% Turkish & 13.52 & \textbf{13.52} & 8.84 \\
% Chinese (Hong Kong) & 5.43 & \textbf{6.10} & 3.90 \\
% Chinese (Taiwan) & 3.63 & \textbf{4.10} & 2.75 \\
% Arabic & 10.03 & \textbf{10.55} & 5.79 \\
% Danish & 15.62 & \textbf{16.59} & 14.22 \\
% Hebrew & 7.96 & \textbf{8.36} & 4.86 \\
% Japanese & 6.40 & \textbf{10.74} & 4.07 \\
% Khmer & 1.87 & 2.13 & \textbf{2.58} \\
% Malay & 13.38 & \textbf{13.61} & 11.44 \\
% Norwegian & 14.98 & \textbf{15.72} & 13.37 \\
% Thai & 7.84 & \textbf{8.48} & 5.55 \\
% Vietnamese & 11.69 & \textbf{12.44} & 10.48 \\
% Chinese (Simplified) & 3.96 & \textbf{4.82} & 3.04 \\
% \midrule
% \textbf{Avg} & 11.63 & \textbf{12.54} & 10.36 \\
% \bottomrule
% \end{tabular}
% \caption{chrF scores on MKQA using Mistral across standard, context, and end-to-end.}
% \label{tab:mkqa-mistral-chrf}
% \end{table}

\clearpage


\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lccc}
\toprule
\textbf{Language} & \textbf{Standard} & \textbf{Context} & \textbf{End-to-end} \\
\midrule
German & 26.87 & 30.88 & \textbf{37.32} \\
Spanish & 27.65 & 28.92 & \textbf{34.82} \\
Finnish & 29.83 & \textbf{32.99} & 22.64 \\
French & 32.69 & \textbf{34.89} & 32.41 \\
Hungarian & 30.13 & \textbf{34.07} & 24.96 \\
Italian & 33.52 & \textbf{34.09} & 22.91 \\
Korean & \textbf{13.72} & 12.47 & 4.23 \\
Dutch & 25.12 & 28.32 & \textbf{36.95} \\
Polish & 30.77 & 31.06 & \textbf{35.41} \\
Portuguese & 28.27 & \textbf{29.57} & 26.82 \\
Russian & 25.59 & \textbf{29.77} & 18.51 \\
Swedish & 33.37 & \textbf{36.70} & 25.99 \\
Turkish & 29.19 & \textbf{30.16} & 25.16 \\
Chinese (Hong Kong) & 15.88 & \textbf{16.95} & 9.91 \\
Chinese (Taiwan) & \textbf{20.65} & 18.21 & 5.52 \\
Arabic & 21.79 & \textbf{24.68} & 19.36 \\
Danish & 40.54 & \textbf{44.15} & 25.22 \\
Hebrew & 25.42 & \textbf{25.55} & 10.77 \\
Japanese & 29.05 & \textbf{33.21} & 23.87 \\
Khmer & 2.07 & 2.69 & \textbf{13.03} \\
Malay & 29.16 & \textbf{30.16} & 19.43 \\
Norwegian & 33.98 & \textbf{36.82} & 30.71 \\
Thai & 21.96 & 22.79 & \textbf{30.69} \\
Vietnamese & 27.92 & \textbf{32.32} & 24.17 \\
Chinese (Simplified) & \textbf{21.20} & 16.47 & 15.03 \\
\bottomrule
\end{tabular}
\caption{chrF scores on MKQA using GPT across standard, context, and end-to-end.}
\label{tab:mkqa-gpt-chrf}
\end{table}



% \begin{table*}[t]
% \centering
% \small
% \setlength{\tabcolsep}{5pt}
% \begin{tabular}{lccc}
% \toprule
% \textbf{Language} & \textbf{Standard} & \textbf{Context} & \textbf{End-to-end} \\
% \midrule
% German & 16.41 & \textbf{17.44} & 14.44 \\
% Spanish & 16.39 & \textbf{16.93} & 14.52 \\
% Finnish & 16.24 & \textbf{18.57} & 15.20 \\
% French & 16.79 & \textbf{18.38} & 17.05 \\
% Hungarian & 13.82 & \textbf{15.36} & 14.32 \\
% Italian & 16.91 & \textbf{17.25} & 15.35 \\
% Korean & 6.71 & \textbf{7.07} & 5.09 \\
% Dutch & 15.01 & \textbf{15.20} & 12.11 \\
% Polish & 16.25 & \textbf{18.12} & 15.35 \\
% Portuguese & 15.99 & \textbf{17.07} & 10.77 \\
% Russian & 13.93 & \textbf{14.58} & 12.09 \\
% Swedish & 17.31 & \textbf{17.64} & 10.32 \\
% Turkish & \textbf{14.33} & 13.32 & 10.95 \\
% Chinese (Hong Kong) & 4.72 & \textbf{8.07} & 7.61 \\
% Chinese (Taiwan) & 5.24 & 7.68 & \textbf{7.89} \\
% Arabic & 11.73 & \textbf{12.47} & 10.47 \\
% Danish & 17.48 & \textbf{17.57} & 8.65 \\
% Hebrew & 13.86 & \textbf{17.15} & 12.43 \\
% Japanese & 14.23 & \textbf{15.90} & 12.73 \\
% Khmer & 3.50 & \textbf{4.46} & 3.51 \\
% Malay & \textbf{16.02} & 15.31 & 10.30 \\
% Norwegian & 16.47 & \textbf{17.28} & 9.79 \\
% Thai & 13.04 & \textbf{17.29} & 14.39 \\
% Vietnamese & 13.79 & \textbf{14.45} & 13.07 \\
% Chinese (Simplified) & 7.91 & \textbf{10.88} & 9.31 \\
% \bottomrule
% \end{tabular}
% \caption{chrF scores on MKQA using Llama across standard, context, and end-to-end.}
% \label{tab:mkqa-llama-chrf}
% \end{table*}


% \begin{table*}[t]
% \centering
% \small
% \setlength{\tabcolsep}{5pt}
% \begin{tabular}{lccc}
% \toprule
% \textbf{Language} & \textbf{Standard} & \textbf{Context} & \textbf{End-to-end} \\
% \midrule
% German & 20.12 & \textbf{20.66} & 19.28 \\
% Spanish & \textbf{21.16} & 20.58 & 19.84 \\
% Finnish & 16.24 & \textbf{16.59} & 11.01 \\
% French & \textbf{20.57} & 20.22 & 20.14 \\
% Hungarian & 14.26 & \textbf{14.63} & 11.43 \\
% Italian & 20.62 & \textbf{20.91} & 20.86 \\
% Korean & \textbf{6.43} & 5.44 & 5.35 \\
% Dutch & \textbf{20.71} & 20.55 & 20.21 \\
% Polish & 18.13 & \textbf{18.43} & 16.78 \\
% Portuguese & 20.09 & 20.34 & \textbf{20.38} \\
% Russian & \textbf{16.76} & 15.04 & 14.61 \\
% Swedish & 20.29 & \textbf{20.85} & 20.32 \\
% Turkish & \textbf{17.37} & 16.52 & 13.80 \\
% Chinese (Hong Kong) & 8.53 & \textbf{9.66} & 8.42 \\
% Chinese (Taiwan) & \textbf{7.68} & 7.21 & 7.65 \\
% Arabic & \textbf{14.18} & 13.99 & 13.19 \\
% Danish & 19.57 & \textbf{20.06} & 16.38 \\
% Hebrew & 11.57 & \textbf{12.11} & 8.61 \\
% Japanese & \textbf{12.10} & 11.17 & 10.36 \\
% Khmer & \textbf{4.48} & 4.43 & 2.82 \\
% Malay & 19.10 & 19.84 & \textbf{21.70} \\
% Norwegian & 19.29 & \textbf{19.32} & 18.05 \\
% Thai & 13.90 & \textbf{13.91} & 11.39 \\
% Vietnamese & 17.36 & 17.19 & \textbf{19.02} \\
% Chinese (Simplified) & 9.94 & 6.99 & \textbf{10.46} \\
% \bottomrule
% \end{tabular}
% \caption{chrF scores on MKQA using Qwen across standard, context, and end-to-end.}
% \label{tab:mkqa-qwen-chrf}
% \end{table*}



% \begin{table*}[t]
% \centering
% \small
% \setlength{\tabcolsep}{5pt}
% \begin{tabular}{lccc}
% \toprule
% \textbf{Language} & \textbf{Standard} & \textbf{Context} & \textbf{End-to-end} \\
% \midrule
% German & 15.77 & \textbf{16.81} & 13.88 \\
% Spanish & 15.58 & \textbf{16.18} & 13.96 \\
% Finnish & 15.68 & \textbf{17.99} & 14.70 \\
% French & 16.08 & \textbf{17.73} & 16.43 \\
% Hungarian & 13.13 & \textbf{14.66} & 13.76 \\
% Italian & 16.24 & \textbf{16.61} & 14.82 \\
% Korean & 6.69 & \textbf{7.02} & 5.03 \\
% Dutch & 14.27 & \textbf{14.52} & 11.72 \\
% Polish & 15.61 & \textbf{17.47} & 14.78 \\
% Portuguese & 15.33 & \textbf{16.39} & 10.31 \\
% Russian & 13.35 & \textbf{14.00} & 11.56 \\
% Swedish & 16.60 & \textbf{16.96} & 9.96 \\
% Turkish & \textbf{13.70} & 12.82 & 10.52 \\
% Chinese (Hong Kong) & 4.62 & \textbf{7.90} & 7.46 \\
% Chinese (Taiwan) & 5.18 & 7.59 & \textbf{7.83} \\
% Arabic & 11.72 & \textbf{12.45} & 10.45 \\
% Danish & 16.83 & \textbf{16.95} & 8.33 \\
% Hebrew & 13.83 & \textbf{17.10} & 12.41 \\
% Japanese & 13.80 & \textbf{15.79} & 12.68 \\
% Khmer & 3.48 & \textbf{4.40} & 3.42 \\
% Malay & \textbf{15.28} & 14.67 & 9.89 \\
% Norwegian & 15.76 & \textbf{16.55} & 9.37 \\
% Thai & 13.04 & \textbf{17.23} & 14.31 \\
% Vietnamese & 13.05 & \textbf{13.70} & 12.46 \\
% Chinese (Simplified) & 7.88 & \textbf{10.82} & 9.20 \\
% \bottomrule
% \end{tabular}
% \caption{chrF scores on MKQA using Llama across standard, context, and end-to-end.}
% \label{tab:mkqa-llama-chrf}
% \end{table*}












% \begin{table*}[t]
% \centering
% \small
% \setlength{\tabcolsep}{5pt}
% \begin{tabular}{lccc}
% \toprule
% \textbf{Language} & \textbf{Standard} & \textbf{Context} & \textbf{End-to-end} \\
% \midrule
% German & 19.24 & \textbf{19.78} & 18.37 \\
% Spanish & \textbf{20.16} & 19.66 & 18.85 \\
% Finnish & \textbf{15.56} & 15.93 & 10.49 \\
% French & \textbf{19.69} & 19.37 & 19.31 \\
% Hungarian & 13.42 & \textbf{13.78} & 10.70 \\
% Italian & 19.72 & \textbf{20.02} & 19.96 \\
% Korean & \textbf{6.34} & 5.33 & 5.22 \\
% Dutch & \textbf{19.87} & 19.73 & 19.40 \\
% Polish & 17.36 & \textbf{17.66} & 15.97 \\
% Portuguese & 19.13 & 19.41 & \textbf{19.52} \\
% Russian & \textbf{15.98} & 14.39 & 13.93 \\
% Swedish & 19.40 & \textbf{19.95} & 19.39 \\
% Turkish & \textbf{16.61} & 15.78 & 13.04 \\
% Chinese (Hong Kong) & 8.15 & \textbf{9.24} & 8.13 \\
% Chinese (Taiwan) & 7.56 & 7.07 & \textbf{7.58} \\
% Arabic & \textbf{14.15} & 13.96 & 13.16 \\
% Danish & 18.71 & \textbf{19.19} & 15.60 \\
% Hebrew & 11.51 & \textbf{12.04} & 8.56 \\
% Japanese & \textbf{11.99} & 11.03 & 10.23 \\
% Khmer & \textbf{4.34} & 4.31 & 2.73 \\
% Malay & 18.21 & 18.94 & \textbf{20.72} \\
% Norwegian & 18.33 & \textbf{18.34} & 17.13 \\
% Thai & \textbf{13.81} & 13.74 & 11.25 \\
% Vietnamese & 16.31 & 16.19 & \textbf{18.03} \\
% Chinese (Simplified) & 9.86 & 6.86 & \textbf{10.34} \\
% \bottomrule
% \end{tabular}
% \caption{chrF scores on MKQA using Qwen across standard cascade, context, and end-to-end.}
% \label{tab:mkqa-qwen-chrf}
% \end{table*}

==> latex/tables/qwen/mc_math.tex <==
\begin{table}[htbp]
\centering
\begin{tabular}{lccc}
\toprule
Dataset & standard & end\_to\_end & context \\
\midrule
Global MMLU & \textbf{56.69\%} & 46.62\% & 55.38\% \\
MCSQA & 69.25\% & \textbf{71.25\%} & 63.62\% \\
Belebele & 56.25\% & 53.88\% & \textbf{57.88\%} \\
PIQA & \textbf{63.91\%} & 62.56\% & 54.45\% \\
MGSM & 64.00\% & \textbf{70.27\%} & 64.64\% \\
MMath & 35.00\% & 30.60\% & \textbf{35.20\%} \\
\bottomrule
\end{tabular}
\caption{Overall Accuracy on Qwen-2.5-7B-Instruct}
\end{table}

\begin{longtable}{lccc}
\caption{Global MMLU (4200 samples, 42 languages): High-resource (22), Mid-resource (11) and Low-resource (9) on Qwen-2.5-7B-Instruct} \\
\toprule
Language & standard & end\_to\_end & context \\
\midrule
\endfirsthead
\multicolumn{4}{c}{\tablename\ \thetable{} -- continued} \\
\toprule
Language & standard & end\_to\_end & context \\
\midrule
\endhead
\midrule
\multicolumn{4}{r}{\textit{Continued on next page}} \\
\endfoot
\bottomrule
\endlastfoot
\multicolumn{4}{l}{\textit{High-resource (22)}} \\
\midrule
Arabic & \textbf{63.00\%} & 42.00\% & 62.00\% \\
Chinese & \textbf{69.00\%} & 67.00\% & 69.00\% \\
Czech & \textbf{73.00\%} & 56.00\% & 72.00\% \\
Dutch & \textbf{75.00\%} & 57.00\% & 71.00\% \\
English & \textbf{76.00\%} & 73.00\% & 76.00\% \\
French & \textbf{72.00\%} & 71.00\% & 71.00\% \\
German & \textbf{76.00\%} & 63.00\% & 74.00\% \\
Greek & \textbf{62.00\%} & 31.00\% & 62.00\% \\
Indonesian & \textbf{71.00\%} & 60.00\% & 70.00\% \\
Italian & \textbf{70.00\%} & 62.00\% & 69.00\% \\
Japanese & \textbf{64.00\%} & 62.00\% & 60.00\% \\
Korean & \textbf{59.00\%} & 43.00\% & 59.00\% \\
Persian & \textbf{67.00\%} & 44.00\% & 66.00\% \\
Polish & \textbf{70.00\%} & 51.00\% & 66.00\% \\
Portuguese & \textbf{72.00\%} & 64.00\% & 70.00\% \\
Romanian & \textbf{67.00\%} & 51.00\% & 65.00\% \\
Russian & \textbf{65.00\%} & 55.00\% & 65.00\% \\
Spanish & \textbf{79.00\%} & 59.00\% & 79.00\% \\
Swedish & 65.00\% & 55.00\% & \textbf{66.00\%} \\
Turkish & \textbf{55.00\%} & 50.00\% & 54.00\% \\
Ukrainian & \textbf{69.00\%} & 56.00\% & 66.00\% \\
Vietnamese & \textbf{65.00\%} & 58.00\% & 64.00\% \\
\textbf{Avg} & \textbf{68.36\%} & 55.91\% & 67.09\% \\
\midrule
\multicolumn{4}{l}{\textit{Mid-resource (11)}} \\
\midrule
Bengali & \textbf{63.00\%} & 36.00\% & 57.00\% \\
Hebrew & 53.00\% & 38.00\% & \textbf{54.00\%} \\
Hindi & \textbf{59.00\%} & 41.00\% & 57.00\% \\
Kyrgyz & \textbf{54.00\%} & 31.00\% & 54.00\% \\
Lithuanian & \textbf{50.00\%} & 46.00\% & 47.00\% \\
Malay & \textbf{71.00\%} & 60.00\% & 71.00\% \\
Nepali & \textbf{52.00\%} & 37.00\% & 48.00\% \\
Serbian & \textbf{67.00\%} & 52.00\% & 67.00\% \\
Sinhala & \textbf{35.00\%} & 32.00\% & 33.00\% \\
Swahili & 37.00\% & 34.00\% & \textbf{38.00\%} \\
Telugu & \textbf{41.00\%} & 36.00\% & 35.00\% \\
\textbf{Avg} & \textbf{52.91\%} & 40.27\% & 51.00\% \\
\midrule
\multicolumn{4}{l}{\textit{Low-resource (9)}} \\
\midrule
Amharic & \textbf{30.00\%} & 20.00\% & 30.00\% \\
Chichewa & \textbf{36.00\%} & 31.00\% & 36.00\% \\
Filipino & \textbf{65.00\%} & 47.00\% & 64.00\% \\
Hausa & \textbf{32.00\%} & 29.00\% & 31.00\% \\
Igbo & 27.00\% & \textbf{37.00\%} & 28.00\% \\
Malagasy & 27.00\% & \textbf{34.00\%} & 28.00\% \\
Shona & \textbf{33.00\%} & 31.00\% & 31.00\% \\
Somali & 20.00\% & \textbf{27.00\%} & 18.00\% \\
Yoruba & 25.00\% & \textbf{29.00\%} & 23.00\% \\
\textbf{Avg} & \textbf{32.78\%} & 31.67\% & 32.11\% \\
\midrule
\textbf{Overall (42)} & \textbf{56.69\%} & 46.62\% & 55.38\% \\
\end{longtable}

\begin{longtable}{lccc}
\caption{MCSQA (800 samples, 8 languages): High-resource (8) on Qwen-2.5-7B-Instruct} \\
\toprule
Language & standard & end\_to\_end & context \\
\midrule
\endfirsthead
\multicolumn{4}{c}{\tablename\ \thetable{} -- continued} \\
\toprule
Language & standard & end\_to\_end & context \\
\midrule
\endhead
\midrule
\multicolumn{4}{r}{\textit{Continued on next page}} \\
\endfoot
\bottomrule
\endlastfoot
\multicolumn{4}{l}{\textit{High-resource (8)}} \\
\midrule
Chinese & \textbf{66.00\%} & 62.00\% & 66.00\% \\
Dutch & 79.00\% & \textbf{83.00\%} & 64.00\% \\
English & 77.00\% & \textbf{81.00\%} & 77.00\% \\
French & 70.00\% & \textbf{73.00\%} & 69.00\% \\
German & 70.00\% & \textbf{74.00\%} & 58.00\% \\
Japanese & 70.00\% & \textbf{78.00\%} & 67.00\% \\
Portuguese & \textbf{75.00\%} & 72.00\% & 69.00\% \\
Russian & \textbf{47.00\%} & 47.00\% & 39.00\% \\
\textbf{Avg} & 69.25\% & \textbf{71.25\%} & 63.62\% \\
\midrule
\textbf{Overall (8)} & 69.25\% & \textbf{71.25\%} & 63.62\% \\
\end{longtable}

\begin{longtable}{lccc}
\caption{Belebele (3630 samples, 121 languages): High-resource (31), Mid-resource (42) and Low-resource (48) on Qwen-2.5-7B-Instruct} \\
\toprule
Language & standard & end\_to\_end & context \\
\midrule
\endfirsthead
\multicolumn{4}{c}{\tablename\ \thetable{} -- continued} \\
\toprule
Language & standard & end\_to\_end & context \\
\midrule
\endhead
\midrule
\multicolumn{4}{r}{\textit{Continued on next page}} \\
\endfoot
\bottomrule
\endlastfoot
\multicolumn{4}{l}{\textit{High-resource (31)}} \\
\midrule
Chinese (Simplified) & 63.33\% & \textbf{83.33\%} & 70.00\% \\
Chinese (Traditional) & 70.00\% & \textbf{76.67\%} & 73.33\% \\
Czech & 76.67\% & 76.67\% & \textbf{80.00\%} \\
Danish & 76.67\% & \textbf{86.67\%} & 80.00\% \\
Dutch & 80.00\% & \textbf{90.00\%} & 80.00\% \\
Egyptian Arabic & 56.67\% & \textbf{66.67\%} & 56.67\% \\
English & 76.67\% & \textbf{90.00\%} & 76.67\% \\
French & 76.67\% & \textbf{80.00\%} & 80.00\% \\
German & 80.00\% & \textbf{93.33\%} & 86.67\% \\
Greek & \textbf{83.33\%} & 80.00\% & 83.33\% \\
Hungarian & 66.67\% & \textbf{76.67\%} & 66.67\% \\
Indonesian & 76.67\% & 76.67\% & \textbf{80.00\%} \\
Italian & \textbf{96.67\%} & 80.00\% & 96.67\% \\
Japanese & 56.67\% & \textbf{70.00\%} & 56.67\% \\
Korean & \textbf{80.00\%} & 73.33\% & 80.00\% \\
Mesopotamian Arabic & 56.67\% & \textbf{63.33\%} & 53.33\% \\
Modern Standard Arabic & 66.67\% & 66.67\% & \textbf{70.00\%} \\
Modern Standard Arabic (Romanized) & 16.67\% & \textbf{26.67\%} & 16.67\% \\
Najdi Arabic & 53.33\% & \textbf{56.67\%} & 53.33\% \\
North Levantine Arabic & 50.00\% & \textbf{56.67\%} & 53.33\% \\
Polish & 80.00\% & \textbf{83.33\%} & 80.00\% \\
Portuguese & \textbf{90.00\%} & 83.33\% & 90.00\% \\
Romanian & 66.67\% & \textbf{70.00\%} & 70.00\% \\
Russian & 60.00\% & \textbf{83.33\%} & 63.33\% \\
Slovak & \textbf{90.00\%} & 66.67\% & 90.00\% \\
Spanish & 86.67\% & \textbf{90.00\%} & 90.00\% \\
Swedish & 70.00\% & \textbf{76.67\%} & 73.33\% \\
Turkish & 66.67\% & \textbf{73.33\%} & 73.33\% \\
Ukrainian & 70.00\% & 63.33\% & \textbf{73.33\%} \\
Vietnamese & 76.67\% & \textbf{83.33\%} & 80.00\% \\
Western Persian & 73.33\% & 70.00\% & \textbf{76.67\%} \\
\textbf{Avg} & 70.65\% & \textbf{74.62\%} & 72.69\% \\
\midrule
\multicolumn{4}{l}{\textit{Mid-resource (42)}} \\
\midrule
Afrikaans & \textbf{83.33\%} & 73.33\% & 76.67\% \\
Armenian & \textbf{73.33\%} & 56.67\% & 73.33\% \\
Basque & \textbf{73.33\%} & 56.67\% & 73.33\% \\
Bengali & 50.00\% & \textbf{56.67\%} & 50.00\% \\
Bengali (Romanized) & 33.33\% & \textbf{43.33\%} & 30.00\% \\
Bulgarian & \textbf{83.33\%} & 83.33\% & 83.33\% \\
Burmese & \textbf{46.67\%} & 33.33\% & 46.67\% \\
Catalan & 76.67\% & \textbf{86.67\%} & 83.33\% \\
Croatian & 80.00\% & 80.00\% & \textbf{83.33\%} \\
Eastern Panjabi & 40.00\% & 46.67\% & \textbf{50.00\%} \\
Finnish & 80.00\% & 76.67\% & \textbf{86.67\%} \\
Georgian & 63.33\% & 60.00\% & \textbf{66.67\%} \\
Gujarati & 40.00\% & \textbf{43.33\%} & 43.33\% \\
Hebrew & 80.00\% & 70.00\% & \textbf{83.33\%} \\
Hindi & 46.67\% & \textbf{63.33\%} & 46.67\% \\
Hindi (Romanized) & 53.33\% & 46.67\% & \textbf{60.00\%} \\
Icelandic & 76.67\% & 70.00\% & \textbf{80.00\%} \\
Kannada & 53.33\% & \textbf{63.33\%} & 56.67\% \\
Kazakh & 66.67\% & 50.00\% & \textbf{70.00\%} \\
Khmer & 56.67\% & 36.67\% & \textbf{60.00\%} \\
Kyrgyz & \textbf{73.33\%} & 60.00\% & 73.33\% \\
Lithuanian & \textbf{73.33\%} & 66.67\% & 73.33\% \\
Macedonian & 70.00\% & \textbf{73.33\%} & 73.33\% \\
Malayalam & 50.00\% & \textbf{53.33\%} & 53.33\% \\
Marathi & 76.67\% & \textbf{83.33\%} & 76.67\% \\
Nepali & 46.67\% & 46.67\% & \textbf{50.00\%} \\
North Azerbaijani & 60.00\% & \textbf{63.33\%} & 63.33\% \\
Northern Uzbek & 70.00\% & \textbf{80.00\%} & 76.67\% \\
Norwegian Bokmål & 83.33\% & 80.00\% & \textbf{90.00\%} \\
Serbian & 83.33\% & 70.00\% & \textbf{86.67\%} \\
Sinhala & 43.33\% & 33.33\% & \textbf{46.67\%} \\
Sinhala (Romanized) & 36.67\% & 13.33\% & \textbf{40.00\%} \\
Slovenian & 53.33\% & \textbf{70.00\%} & 63.33\% \\
Standard Malay & 90.00\% & 80.00\% & \textbf{93.33\%} \\
Swahili & 70.00\% & 56.67\% & \textbf{73.33\%} \\
Tagalog & 60.00\% & \textbf{63.33\%} & 63.33\% \\
Tamil & 53.33\% & 53.33\% & \textbf{56.67\%} \\
Telugu & 43.33\% & \textbf{53.33\%} & 43.33\% \\
Thai & 46.67\% & \textbf{63.33\%} & 50.00\% \\
Tosk Albanian & 80.00\% & 70.00\% & \textbf{83.33\%} \\
Urdu & 76.67\% & 60.00\% & \textbf{80.00\%} \\
Urdu (Romanized) & \textbf{53.33\%} & 43.33\% & 53.33\% \\
\textbf{Avg} & 63.09\% & 60.32\% & \textbf{65.87\%} \\
\midrule
\multicolumn{4}{l}{\textit{Low-resource (48)}} \\
\midrule
Amharic & \textbf{30.00\%} & 30.00\% & 30.00\% \\
Assamese & 66.67\% & 50.00\% & \textbf{70.00\%} \\
Bambara & 16.67\% & \textbf{26.67\%} & 13.33\% \\
Cebuano & \textbf{73.33\%} & 40.00\% & 73.33\% \\
Central Kurdish & 66.67\% & 43.33\% & \textbf{70.00\%} \\
Estonian & \textbf{80.00\%} & 66.67\% & 80.00\% \\
Ganda & \textbf{23.33\%} & 16.67\% & 23.33\% \\
Guarani & 20.00\% & \textbf{36.67\%} & 20.00\% \\
Haitian Creole & \textbf{63.33\%} & 43.33\% & 63.33\% \\
Halh Mongolian & 26.67\% & \textbf{40.00\%} & 26.67\% \\
Hausa & \textbf{46.67\%} & 30.00\% & 46.67\% \\
Igbo & \textbf{43.33\%} & 30.00\% & 43.33\% \\
Ilocano & \textbf{43.33\%} & 43.33\% & 43.33\% \\
Javanese & \textbf{66.67\%} & 53.33\% & 66.67\% \\
Jingpho & \textbf{36.67\%} & 36.67\% & 36.67\% \\
Kabuverdianu & \textbf{50.00\%} & 36.67\% & 50.00\% \\
Kinyarwanda & 40.00\% & 23.33\% & \textbf{43.33\%} \\
Lao & 40.00\% & 26.67\% & \textbf{43.33\%} \\
Lingala & \textbf{36.67\%} & 33.33\% & 33.33\% \\
Luo & \textbf{26.67\%} & 16.67\% & 26.67\% \\
Maltese & \textbf{66.67\%} & 66.67\% & 66.67\% \\
Maori & 33.33\% & 33.33\% & \textbf{36.67\%} \\
Nepali (Romanized) & 33.33\% & \textbf{43.33\%} & 33.33\% \\
Nigerian Fulfulde & \textbf{26.67\%} & 13.33\% & 26.67\% \\
Northern Sotho & \textbf{40.00\%} & 20.00\% & 33.33\% \\
Nyanja & \textbf{50.00\%} & 26.67\% & 50.00\% \\
Odia & 53.33\% & 20.00\% & \textbf{60.00\%} \\
Plateau Malagasy & \textbf{43.33\%} & 43.33\% & 43.33\% \\
Shan & \textbf{30.00\%} & 26.67\% & 30.00\% \\
Shona & \textbf{30.00\%} & 23.33\% & 30.00\% \\
Sindhi & \textbf{56.67\%} & 40.00\% & 56.67\% \\
Somali & 26.67\% & \textbf{30.00\%} & 26.67\% \\
Southern Pashto & \textbf{46.67\%} & 33.33\% & 46.67\% \\
Southern Sotho & \textbf{33.33\%} & 30.00\% & 33.33\% \\
Standard Latvian & 63.33\% & \textbf{66.67\%} & 63.33\% \\
Standard Tibetan & \textbf{23.33\%} & 20.00\% & 23.33\% \\
Sundanese & \textbf{63.33\%} & 50.00\% & 63.33\% \\
Swati & 20.00\% & \textbf{40.00\%} & 20.00\% \\
Tajik & 53.33\% & \textbf{63.33\%} & 53.33\% \\
Tigrinya & 13.33\% & \textbf{20.00\%} & 13.33\% \\
Tsonga & 30.00\% & \textbf{43.33\%} & 30.00\% \\
Tswana & \textbf{23.33\%} & 20.00\% & 20.00\% \\
Waray & 53.33\% & 40.00\% & \textbf{56.67\%} \\
West Central Oromo & \textbf{30.00\%} & 30.00\% & 30.00\% \\
Wolof & 36.67\% & 23.33\% & \textbf{40.00\%} \\
Xhosa & 36.67\% & 30.00\% & \textbf{40.00\%} \\
Yoruba & \textbf{33.33\%} & 23.33\% & 33.33\% \\
Zulu & 20.00\% & \textbf{30.00\%} & 20.00\% \\
\textbf{Avg} & 40.97\% & 34.86\% & \textbf{41.32\%} \\
\midrule
\textbf{Overall (121)} & 56.25\% & 53.88\% & \textbf{57.88\%} \\
\end{longtable}

\begin{longtable}{lccc}
\caption{PIQA (3480 samples, 116 languages): High-resource (44), Mid-resource (42) and Low-resource (30) on Qwen-2.5-7B-Instruct} \\
\toprule
Language & standard & end\_to\_end & context \\
\midrule
\endfirsthead
\multicolumn{4}{c}{\tablename\ \thetable{} -- continued} \\
\toprule
Language & standard & end\_to\_end & context \\
\midrule
\endhead
\midrule
\multicolumn{4}{r}{\textit{Continued on next page}} \\
\endfoot
\bottomrule
\endlastfoot
\multicolumn{4}{l}{\textit{High-resource (44)}} \\
\midrule
Algerian Arabic & 43.33\% & \textbf{56.67\%} & 43.33\% \\
Burushaski & 43.33\% & \textbf{60.00\%} & 40.00\% \\
Cantonese & 70.00\% & \textbf{83.33\%} & 60.00\% \\
Chinese (Simplified) & 66.67\% & \textbf{70.00\%} & 56.67\% \\
Chinese (Traditional) & \textbf{60.00\%} & 60.00\% & 50.00\% \\
Czech & 53.33\% & \textbf{70.00\%} & 50.00\% \\
Dutch & 60.00\% & \textbf{70.00\%} & 43.33\% \\
Egyptian Arabic & \textbf{70.00\%} & 50.00\% & 56.67\% \\
English & 63.33\% & \textbf{83.33\%} & 70.00\% \\
French (Canada) & 83.33\% & \textbf{90.00\%} & 66.67\% \\
French (France) & 73.33\% & \textbf{76.67\%} & 56.67\% \\
German & \textbf{80.00\%} & 56.67\% & 80.00\% \\
Greek & \textbf{66.67\%} & 16.67\% & 66.67\% \\
Gulf Arabic & \textbf{60.00\%} & 40.00\% & 46.67\% \\
Hungarian & \textbf{73.33\%} & 73.33\% & 63.33\% \\
Indonesian & 86.67\% & \textbf{90.00\%} & 86.67\% \\
Italian & \textbf{83.33\%} & 80.00\% & 76.67\% \\
Japanese & \textbf{86.67\%} & 80.00\% & 76.67\% \\
Korean & \textbf{66.67\%} & 50.00\% & 50.00\% \\
Mesopotamian Arabic & \textbf{70.00\%} & 70.00\% & 56.67\% \\
Modern Standard Arabic & 46.67\% & \textbf{56.67\%} & 53.33\% \\
Moroccan Arabic & \textbf{76.67\%} & 50.00\% & 63.33\% \\
Najdi Arabic & \textbf{83.33\%} & 70.00\% & 73.33\% \\
North Levantine Arabic (Jordan) & \textbf{56.67\%} & 50.00\% & 53.33\% \\
North Levantine Arabic (Lebanon) & \textbf{83.33\%} & 76.67\% & 73.33\% \\
North Levantine Arabic (Palestine) & \textbf{66.67\%} & 60.00\% & 56.67\% \\
North Levantine Arabic (Syria) & \textbf{56.67\%} & 56.67\% & 53.33\% \\
Polish & 60.00\% & \textbf{70.00\%} & 56.67\% \\
Portuguese (Brazil) & 60.00\% & \textbf{76.67\%} & 40.00\% \\
Portuguese (Portugal) & 73.33\% & \textbf{80.00\%} & 63.33\% \\
Romanian & \textbf{100.00\%} & 93.33\% & 86.67\% \\
Russian & 50.00\% & \textbf{80.00\%} & 56.67\% \\
Slovak & 73.33\% & \textbf{76.67\%} & 56.67\% \\
Slovak (SARI) & 56.67\% & \textbf{60.00\%} & 43.33\% \\
Spanish (Mexico) & 80.00\% & \textbf{83.33\%} & 70.00\% \\
Spanish (Peru) & 90.00\% & \textbf{96.67\%} & 86.67\% \\
Spanish (Spain) & 80.00\% & \textbf{83.33\%} & 66.67\% \\
Swedish & \textbf{76.67\%} & 70.00\% & 66.67\% \\
Ta'izzi-Adeni Arabic & \textbf{76.67\%} & 63.33\% & 73.33\% \\
Tunisian Arabic & \textbf{70.00\%} & 60.00\% & 53.33\% \\
Turkish & 63.33\% & \textbf{66.67\%} & 53.33\% \\
Ukrainian & \textbf{76.67\%} & 56.67\% & 53.33\% \\
Vietnamese & 60.00\% & \textbf{73.33\%} & 63.33\% \\
Western Persian & \textbf{66.67\%} & 63.33\% & 66.67\% \\
\textbf{Avg} & \textbf{69.17\%} & 68.18\% & 60.91\% \\
\midrule
\multicolumn{4}{l}{\textit{Mid-resource (42)}} \\
\midrule
Armenian & \textbf{70.00\%} & 30.00\% & 56.67\% \\
Belarusian & \textbf{60.00\%} & 56.67\% & 56.67\% \\
Bengali & 63.33\% & \textbf{70.00\%} & 50.00\% \\
Bengali (Romanized) & \textbf{56.67\%} & 50.00\% & 33.33\% \\
Bosnian & \textbf{96.67\%} & 90.00\% & 83.33\% \\
Bulgarian & \textbf{86.67\%} & 70.00\% & 80.00\% \\
Catalan & 70.00\% & \textbf{76.67\%} & 36.67\% \\
Croatian & \textbf{73.33\%} & 70.00\% & 63.33\% \\
Eastern Panjabi & \textbf{73.33\%} & 50.00\% & 63.33\% \\
Finnish & \textbf{60.00\%} & 40.00\% & 36.67\% \\
Galician & \textbf{66.67\%} & 66.67\% & 66.67\% \\
Georgian & \textbf{60.00\%} & 53.33\% & 53.33\% \\
Gujarati & 73.33\% & 73.33\% & \textbf{80.00\%} \\
Hebrew & \textbf{56.67\%} & 33.33\% & 50.00\% \\
Hindi & \textbf{76.67\%} & 76.67\% & 60.00\% \\
Icelandic & \textbf{66.67\%} & 60.00\% & 50.00\% \\
Kannada & 56.67\% & \textbf{63.33\%} & 36.67\% \\
Kazakh & 36.67\% & \textbf{50.00\%} & 30.00\% \\
Kyrgyz & \textbf{60.00\%} & 60.00\% & 43.33\% \\
Lithuanian & 66.67\% & \textbf{76.67\%} & 73.33\% \\
Macedonian & \textbf{73.33\%} & 56.67\% & 63.33\% \\
Malayalam & \textbf{43.33\%} & 43.33\% & 26.67\% \\
Marathi & \textbf{80.00\%} & 60.00\% & 60.00\% \\
Nepali & 60.00\% & \textbf{63.33\%} & 56.67\% \\
North Azerbaijani & \textbf{50.00\%} & 46.67\% & 43.33\% \\
Northern Uzbek & 56.67\% & \textbf{70.00\%} & 43.33\% \\
Norwegian Bokmål & \textbf{66.67\%} & 63.33\% & 56.67\% \\
Norwegian Nynorsk & \textbf{73.33\%} & 73.33\% & 70.00\% \\
Serbian (Cyrillic) & \textbf{63.33\%} & 46.67\% & 46.67\% \\
Serbian (Latin) & 60.00\% & \textbf{80.00\%} & 43.33\% \\
Sinhala & 46.67\% & \textbf{60.00\%} & 33.33\% \\
Slovenian & 43.33\% & \textbf{60.00\%} & 46.67\% \\
Slovenian (CERK) & 43.33\% & \textbf{50.00\%} & 40.00\% \\
Standard Malay & 80.00\% & \textbf{83.33\%} & 56.67\% \\
Swahili & \textbf{56.67\%} & 53.33\% & 53.33\% \\
Tagalog & \textbf{66.67\%} & 53.33\% & 63.33\% \\
Tamil & \textbf{53.33\%} & 43.33\% & 43.33\% \\
Telugu & \textbf{70.00\%} & 56.67\% & 66.67\% \\
Thai & \textbf{63.33\%} & 56.67\% & 56.67\% \\
Tosk Albanian & 60.00\% & \textbf{63.33\%} & 46.67\% \\
Urdu & \textbf{73.33\%} & 63.33\% & 63.33\% \\
Urdu (Romanized) & \textbf{63.33\%} & 46.67\% & 56.67\% \\
\textbf{Avg} & \textbf{63.73\%} & 59.76\% & 53.33\% \\
\midrule
\multicolumn{4}{l}{\textit{Low-resource (30)}} \\
\midrule
Amharic & 53.33\% & \textbf{63.33\%} & 50.00\% \\
Assamese & 80.00\% & \textbf{83.33\%} & 70.00\% \\
Bambara & 40.00\% & \textbf{56.67\%} & 46.67\% \\
Bhojpuri & 63.33\% & \textbf{70.00\%} & 56.67\% \\
Central Kurdish & \textbf{46.67\%} & 46.67\% & 33.33\% \\
Dhundari & \textbf{83.33\%} & 53.33\% & 56.67\% \\
Ekpeye & 56.67\% & \textbf{66.67\%} & 40.00\% \\
Estonian & 40.00\% & \textbf{50.00\%} & 46.67\% \\
Faroese & \textbf{60.00\%} & 46.67\% & 46.67\% \\
Hausa & 43.33\% & \textbf{66.67\%} & 40.00\% \\
Hawaiian & 60.00\% & \textbf{63.33\%} & 46.67\% \\
Idoma & 43.33\% & \textbf{53.33\%} & 40.00\% \\
Igbo & 40.00\% & \textbf{46.67\%} & 30.00\% \\
Isoko & 50.00\% & \textbf{63.33\%} & 36.67\% \\
Javanese & 60.00\% & \textbf{63.33\%} & 40.00\% \\
Kinyarwanda & \textbf{70.00\%} & 46.67\% & 60.00\% \\
Kumzari & \textbf{46.67\%} & 46.67\% & 43.33\% \\
Lingala & 66.67\% & \textbf{73.33\%} & 53.33\% \\
Luo & \textbf{50.00\%} & 46.67\% & 43.33\% \\
Marwari & \textbf{70.00\%} & 70.00\% & 66.67\% \\
Meitei (Bengali script) & \textbf{73.33\%} & 53.33\% & 36.67\% \\
Meitei (Meitei script) & \textbf{56.67\%} & 36.67\% & 46.67\% \\
Nagamese & 53.33\% & \textbf{56.67\%} & 56.67\% \\
Nigerian Pidgin & 76.67\% & \textbf{80.00\%} & 53.33\% \\
Sindhi & \textbf{83.33\%} & 76.67\% & 70.00\% \\
Sindhi (Devanagari) & \textbf{66.67\%} & 63.33\% & 40.00\% \\
Urhobo & 33.33\% & \textbf{46.67\%} & 33.33\% \\
Uyghur & 30.00\% & \textbf{60.00\%} & 30.00\% \\
Yoruba & 46.67\% & \textbf{53.33\%} & 40.00\% \\
Zulu & \textbf{50.00\%} & 43.33\% & 43.33\% \\
\textbf{Avg} & 56.44\% & \textbf{58.22\%} & 46.56\% \\
\midrule
\textbf{Overall (116)} & \textbf{63.91\%} & 62.56\% & 54.45\% \\
\end{longtable}

\begin{longtable}{lccc}
\caption{MGSM (1100 samples, 11 languages): High-resource (7) and Mid-resource (4) on Qwen-2.5-7B-Instruct} \\
\toprule
Language & standard & end\_to\_end & context \\
\midrule
\endfirsthead
\multicolumn{4}{c}{\tablename\ \thetable{} -- continued} \\
\toprule
Language & standard & end\_to\_end & context \\
\midrule
\endhead
\midrule
\multicolumn{4}{r}{\textit{Continued on next page}} \\
\endfoot
\bottomrule
\endlastfoot
\multicolumn{4}{l}{\textit{High-resource (7)}} \\
\midrule
Chinese & 82.00\% & 79.00\% & \textbf{86.00\%} \\
English & 92.00\% & \textbf{95.00\%} & 92.00\% \\
French & 74.00\% & \textbf{82.00\%} & 80.00\% \\
German & 74.00\% & \textbf{80.00\%} & 78.00\% \\
Japanese & 56.00\% & \textbf{70.00\%} & 61.00\% \\
Russian & 77.00\% & \textbf{86.00\%} & 77.00\% \\
Spanish & 81.00\% & \textbf{86.00\%} & 85.00\% \\
\textbf{Avg} & 76.57\% & \textbf{82.57\%} & 79.86\% \\
\midrule
\multicolumn{4}{l}{\textit{Mid-resource (4)}} \\
\midrule
Bengali & \textbf{60.00\%} & 57.00\% & 41.00\% \\
Swahili & 19.00\% & \textbf{21.00\%} & 19.00\% \\
Telugu & 30.00\% & \textbf{39.00\%} & 28.00\% \\
Thai & 59.00\% & \textbf{78.00\%} & 64.00\% \\
\textbf{Avg} & 42.00\% & \textbf{48.75\%} & 38.00\% \\
\midrule
\textbf{Overall (11)} & 64.00\% & \textbf{70.27\%} & 64.64\% \\
\end{longtable}

\begin{longtable}{lccc}
\caption{MMath (1000 samples, 10 languages): High-resource (9) and Mid-resource (1) on Qwen-2.5-7B-Instruct} \\
\toprule
Language & standard & end\_to\_end & context \\
\midrule
\endfirsthead
\multicolumn{4}{c}{\tablename\ \thetable{} -- continued} \\
\toprule
Language & standard & end\_to\_end & context \\
\midrule
\endhead
\midrule
\multicolumn{4}{r}{\textit{Continued on next page}} \\
\endfoot
\bottomrule
\endlastfoot
\multicolumn{4}{l}{\textit{High-resource (9)}} \\
\midrule
Arabic & \textbf{37.00\%} & 28.00\% & 37.00\% \\
Chinese & 33.00\% & 32.00\% & \textbf{34.00\%} \\
English & 31.00\% & \textbf{40.00\%} & 34.00\% \\
French & \textbf{38.00\%} & 34.00\% & 37.00\% \\
Japanese & \textbf{39.00\%} & 27.00\% & 39.00\% \\
Korean & \textbf{31.00\%} & 28.00\% & 31.00\% \\
Portuguese & \textbf{37.00\%} & 27.00\% & 37.00\% \\
Spanish & \textbf{33.00\%} & 32.00\% & 33.00\% \\
Vietnamese & \textbf{38.00\%} & 34.00\% & 38.00\% \\
\textbf{Avg} & 35.22\% & 31.33\% & \textbf{35.56\%} \\
\midrule
\multicolumn{4}{l}{\textit{Mid-resource (1)}} \\
\midrule
Thai & \textbf{33.00\%} & 24.00\% & 32.00\% \\
\textbf{Avg} & \textbf{33.00\%} & 24.00\% & 32.00\% \\
\midrule
\textbf{Overall (10)} & 35.00\% & 30.60\% & \textbf{35.20\%} \\
\end{longtable}


